Identifying and Benchmarking Natural Out-of-Context Prediction Problems

Deep learning systems frequently fail at out-of-context (OOC) prediction, the problem of making reliable predictions on uncommon or unusual inputs or subgroups of the training distribution. To this end, a number of benchmarks for measuring OOC performance have recently been introduced. In this work, we introduce a framework unifying the literature on OOC performance measurement, and demonstrate how rich auxiliary information can be leveraged to identify candidate sets of OOC examples in existing datasets. We present NOOCh: a suite of naturally-occurring "challenge sets", and show how varying notions of context can be used to probe specific OOC failure modes. Experimentally, we explore the tradeoffs between various learning approaches on these challenge sets and demonstrate how the choices made in designing OOC benchmarks can yield varying conclusions.

==> figs/results/waterbirds/results_general_with_stds.tex <==
\begin{tabular}{llllllllll}
\hline
 Metric            & ERM           & CVaR          & Focal         & Reweight      & US            & Reweight (Envs)   & US (Envs)     & GDRO                   & IRM                    \\
\hline
 Worst-Group Error & 0.400 (0.050) & 0.354 (0.002) & 0.402 (0.012) & 0.361 (0.004) & 0.336 (0.014) & 0.233 (0.001)     & 0.146 (0.006) & \textbf{0.108 (0.004)} & 0.127 (0.015)          \\
 Worst-Group NLL   & 1.030 (0.035) & 0.657 (0.021) & 0.722 (0.012) & 0.884 (0.004) & 0.883 (0.024) & 0.535 (0.009)     & 0.417 (0.005) & \textbf{0.306 (0.018)} & \textbf{0.346 (0.040)} \\
 AUC-Hard          & 0.691 (0.048) & 0.703 (0.016) & 0.506 (0.080) & 0.657 (0.003) & 0.701 (0.032) & 0.744 (0.005)     & 0.778 (0.008) & \textbf{0.929 (0.005)} & 0.788 (0.015)          \\
\hline
\end{tabular}

==> sections/benchmark.tex <==
% \section{The {\rococo \ } Benchmark}
\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/kite_Hard_Positives_85911.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/sports_ball_Hard_Positives_79966.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/surfboard_Hard_Positives_342549.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}

\medskip
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/kite_Hard_Negatives_549597.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/sports_ball_Hard_Negatives_187785.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/surfboard_Hard_Negatives_173373.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{Using the co-occurrence/extractibility (CE) criterion, examples of (0.05, 0.1)-hard positives (top row) and negatives (bottom row) for the classes (L to R):  \texttt{kite, sports\_ball, surfboard}.} \label{fig:benchmark-hard-pos-neg-examples}
\end{figure}




\section{Finding Naturally-Occurring OOC Problems} \label{sec:benchmark}

% One major challenge of developing methods for OOC prediction is evaluation: many standard benchmarks rely on synthetic data or a synthetically-created shift: for instance, mixing and matching foregrounds and backgrounds with changing probabilities in the training and test sets.
% However, 

Throughout this paper, we consider the binary prediction task of determining object presence --- given an image $X$, is an object of class $Y$ present or not?
% The label is 1 if at least one instance of the object is present, and 0 otherwise.
% As described in Sec. \ref{sec:intro}, context can play a role in prediction through a number of frequently co-occurring objects and object relationships, in ways that may go beyond what is easily mimicked synthetically.
In order to study how context shifts arise naturally within an existing computer vision benchmark, we propose two methods which leverage annotations to automatically identify candidate OOC examples in the test set.
% We study how context shifts arise within 
% % To understand better how context shifts can arise in practice, we study 
% an existing computer vision benchmark, and propose two methods which leverage existing annotations to automatically identify OOC examples in the test set.
% These OOC sets can play the role of ``stress tests'' for a proposed method.
% \RZ{The paragraph above is a bit repetitive with the intro.}

\subsection{Background: COCO and COCO-Stuff}

The Microsoft Common Objects in COntext dataset (COCO) \citep{lin2014microsoft} is a computer vision dataset consisting of images of natural scenes.
Each image is annotated with instance labels and segmentations for every ``thing'' in the image, as well as several captions describing the content of the scene.
Images usually contain multiple items and as such usually have multiple labels.

However, for the purposes of investigating OOC prediction, many relevant objects are not labelled in COCO; for instance, background objects such as ``sky'' or ``grass'' are not COCO classes.
Fortunately, the COCO-Stuff dataset \citep{caesar2018coco} provides labels and segmentations for all of the ``stuff'' in the images from COCO.
The ``thing'' vs ``stuff'' distinction is a technical one: a thing is an object with a specified size and shape, whereas stuff has no ``defined spatial extent'' \citep{forsyth1996finding}.
Having both thing and stuff labels is essential for understanding model behaviour on OOC examples, since it is exactly these ``stuff'' classes which often (but not always) provide important context cues.
Taken together, the thing and stuff annotations
% provide a coarse but mostly complete, machine-readable description of each image in the COCO dataset, and 
yield a rich sandbox for queries about the role of context in prediction.
For our purposes, COCO-Stuff contains 171 binary tasks for determining object presence (81 thing classes and 90 stuff classes; we ignore the 1 ``unlabelled'' class).

\subsection{Automatically Identifying OOC Examples: Hard Positives and Negatives}

As mentioned in Sec. \ref{sec:intro}, context is hard to define.
In this work, we consider two contrasting notions of context: 1. frequently co-occurring, easily extractible objects; and 2. the ``gist'' of a scene.
Based on these, we present two criteria for identifying naturally-occurring OOC prediction problems within the existing COCO(-Stuff) dataset.
We identify both {\it hard positives}, where the class is present despite an unusual context, and {\it hard negatives}, where the class is \textit{not} present, despite a usual context.
% We now present two methods of identifying challenging but naturally-occurring OOC prediction problems, buried within the existing COCO(-Stuff) dataset.
% We explain these methods below and discuss the implicit notions of context each one relies on.
% \DM{Explain why focus on hard positives and negatives: need both labels}

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_airplane_Hard_Positive.pdf}
\caption{hard positive (CE)} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_airplane_Hard_Positive.pdf}
\caption{hard positive (Gist)} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_Bowl_Hard_Negative.pdf}
\caption{hard negative (CE)} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast_2/example_contrast_Gist_criterion_Bowl_Hard_Negative.png}
\caption{hard negative (Gist)} \label{fig:b}
\end{subfigure}
\caption{\small{
To contrast the CE and Gist criteria, we show samples from the \texttt{airplane} (L) and \texttt{bowl} (R) tasks.}
% and
% % We show the examples where GDRO most outperforms ERM among (L to R): 
% hard positive, CE criterion, \texttt{airplane} task;
% hard positive, Gist criterion, \texttt{airplane} task;
% hard negative, CE criterion, \texttt{bowl} task;
% hard negative, Gist criterion, \texttt{bowl} task.
} \label{fig:results-qual-two-criteria}
\end{figure}

\subsubsection{Defining Context Using Co-Occurrences and Extractibility}

For an object class $Y$, context cues often come in the form of another object class $C$ that has two properties (cf. \citep{lovering2021predicting}).
% We first consider an object class $C$ which is different from class $Y$, and claim that many useful context cues $C$ have two properties (cf. \citep{lovering2021predicting}).
First, $C$ and $Y$ co-occur frequently \citep{biederman1982scene}.
Second, $C$ is  more \textit{extractible} than $Y$ --- easier to detect.
If $C$ were \textit{less} extractible than $Y$ it would not be a useful cue for detecting $Y$, as a model could detect $Y$ directly.
% For instance, it is frequently observed that CNNs are prone to learning signals about object texture rather than shape \citep{geirhos2018imagenet}.
% A similar argument is made in \citet{lovering2021predicting} when assessing the effect of spurious correlations in an NLP setting.

% Contextual cues can be useful: for instance, a number of object detection models explicitly incorporate it to improve performance [cite].
% However, in deep learning systems, trouble can arise when a contextual cue is much easier to learn than the target class i.e. when it is more \textit{extractible}.
% For instance, it is frequently observed that CNNs are prone to learning signals about object texture rather than shape [cite a few].
% % One important aspect of context is extractibility: how easy it is to learn to detect a context cue's presence in an example.
% % Context cues can help humans improve their processing efficiency [cite], and are often ``shortcuts'' [cite] for model prediction.
% The more extractible a signal is, the more likely it will become a contextual signal that a model relies on [cite simplicity bias] --- and when that signal is not present, the more likely a model will struggle to perform well [cite extractibility.

We can utilize these properties to create candidate context cues $C$ for a class of interest $Y$.
Given segmentations, we can use an object's size within an image as a proxy for extractibility (larger objects tend to be more extractible).
% : the larger the object's bounding box in an image, the more extractible it is.
Let the $Area$ operator take the sum of the areas of all segmentations of instances of that object, or return 0 if the object is not present.
% Consider any feature $C \neq Y$ to be a possible contextual cue for $Y$; for example, let $Y = \texttt{surfboard}, C=\texttt{sea}$.
Then, to estimate from the training set how important of a context variable $C$ is, we can compute $A(C, Y) = \mathds{E}[Area(C) - Area(Y) | Y = 1]$.
When $A(C, Y)$ is larger, this means that when $Y$ is present, $C$ is usually also present, and on average, takes up more of the image than $Y$ does.
When $A(C, Y) > \alpha$, we say that $C$ is an $\alpha$-strong context cue for $Y$ (or just $\alpha$-context for brevity).
We find that many of the contexts identified using this method for large enough $\alpha$ are intuitive.
Some examples of (label, 0.05-context) pairs are: (\texttt{car}, \texttt{road}), (\texttt{bowl}, \texttt{dining\_table}), (\texttt{cow}, \texttt{grass}).

ul
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
%     \centering
%     \includegraphics[scale=0.4]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
%     \centering
%     \includegraphics[scale=0.4]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{Using the gist criterion, the number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, where $\tau$ thresholds the cosine similarity to the average caption embedding of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}
% \end{subfigure}
% % \caption{Using the gist-based method, we find that 0.25-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% % The diagonal line represents where they are exactly equal, on average.
% % }
% \label{fig:benchmark-descriptive-statistics}
% \end{figure}

% \begin{figure}
% \centering
% \begin{minipage}{.48\textwidth}
%   \centering
%   \includegraphics[scale=0.4]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{minipage}\hspace*{\fill}
% \begin{minipage}{.48\textwidth}
%   \centering
%     \includegraphics[scale=0.4]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{Using the gist criterion, the number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, where $\tau$ thresholds the cosine similarity to the average caption embedding of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}

% \end{minipage}
% \end{figure}




% Fig \ref{fig:benchmark-num-tasks-num-confs} shows that, under this definition, most of the 171 object classes in COCO-Stuff have context cues for $\alpha \geq 0$.
% Note that a 0-context cue is fairly strong: this means that on average, in images where $Y$ is present, $C$ takes up at least as much area as $Y$ does.
% This indicates that there may be a large number of OOC examples hidden in many of these tasks.
% % For instance, over two-thirds of tasks have at least one 0-context cue, and over 1/3 have at least one 0.05-context cue.
% We find that the contexts returned using this method for large enough $\alpha$ are intuitive.
% Some examples of (label, 0.05-context) pairs are: (\texttt{car}, \texttt{road}), (\texttt{bowl}, \texttt{dining\_table}), (\texttt{cow}, \texttt{grass}).
% Additionally, many tasks have more than one context variable: at $\alpha=0$ about 50 tasks have 3, and at $\alpha=0.05$ about 15 tasks have 3.
% Some examples of labels with multiple 0.05-context variables are: (\texttt{surfboard}, [\texttt{sea}, \texttt{sky-other}]),
% (\texttt{tennis-racket}, [\texttt{person}, \texttt{playing-field}]),
% (\texttt{traffic-light}, [\texttt{building-other}, \texttt{road}, \texttt{sky-other}, \texttt{tree}]).
% All of these groupings are intuitive, providing some evidence that this method of isolating context variables may be a usef one.




Using this notion of context, we can then define hard positive and hard negative examples.
We make the simplifying \textit{noisy-or} assumption: that each context cue provides evidence for $Y$, so that the presence of any cue supports $Y$ being present, while the absence of all provides evidence against $Y$'s presence.
% \RZ{We can motivate this particular definition of hard cases by saying something like: under the assumption that each context variable provides evidence for Y, so that the presence of any is enough to support Y being present, while if none are present provides evidence against Y. This is the noisy-or.}
% Then, a hard positive occurs when no context variable is present but $Y = 1$, and a hard negative occurs when some context variable is present, but $Y = 0$.
Given some image, we can define an ($\alpha, \beta$)-hard positive or negative.
If $Y=1$, and for all $\alpha$-context cues $C$, we have $Area(C) < \beta$ in this image (and there is at least one $\alpha$-context cue), then the example is an ($\alpha, \beta$)-hard positive.
Alternatively, if $Y=0$, and there exists some $\alpha$-context variable $C$ such that $Area(C) > \beta$, then the example is an ($\alpha, \beta$)-hard negative.
We will call this method the co-occurrence/extractibility (CE) criterion (see Fig \ref{fig:benchmark-hard-pos-neg-examples} for examples).
% In Fig \ref{fig:benchmark-hard-pos-neg-examples} we show examples of hard positive and hard negative images in COCO-Stuff.
Throughout, we use $\alpha=0.05, \beta=1$ unless otherwise noted; these parameters were chosen since they approximately equalize $P[(X, Y)\ \textrm{is}\ (\alpha, \beta)\textrm{-hard} \ | Y = y]$ across $y = 0, 1$.
See Appendix \ref{app:data} for more details.

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/proportion_hard_positives_by_area.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/proportion_hard_negatives_by_area.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Across a range of $\alpha, \beta$, the percentage of hard positive/negative examples (L/R) in the test set which are $(\alpha, \beta)$-hard.
% } \label{fig:benchmark-hard-pos-neg-examples-area}
% \end{figure}

% Fig \ref{fig:benchmark-hard-pos-neg-examples-area} shows that hard positive/negative examples are numerous in the data.
% For instance, we see that at the (0.05, 0.1) level, about 10\% of all possible (object, category) pairs are hard positives, and a similar number for hard negatives.
% % Alternatively, in Fig [fig], we can see that about 50\% of test images qualify as hard positives in some category, and about 85\% of test images qualify as hard negatives in some category.

\subsubsection{Defining Context Using Gist}

We now turn to a broader notion of context, that of the ``gist'' of a scene \citep{torralba2003contextual}, or its overall semantic content.
This is something that humans are able to recognize easily \citep{larson2014spatiotemporal}, but goes beyond object frequency and extractibility.
When an object is present in a scene whose gist is very different from the scenes the object was present in at training time, this may create a large challenge for OOC prediction.


We here describe our method for estimating gist shift, which we call the gist criterion.
We leverage caption annotation data in COCO (each image has 5 caption sentences), making the assumption that information in a caption captures the gist of a scene.
We then take an SBERT embedding \citep{reimers2019sentence} of each available image caption for an image, and average these embeddings to get a single embedding for each image.
Then, for a given image and some target label $Y$, we can look at the cosine similarity between that image's embedding and the average embedding across all training images with $Y=1$.
If this similarity is below some threshold $\tau$, and $Y = 1$ for the test image, it is a $\tau$-hard positive;
%Similarly, 
if this similarity is above $\tau$, and $Y = 0$ for the test image, it is a $\tau$-hard negative.
% Fig. \ref{fig:benchmark-hard-pos-neg-examples-caption} shows how the number of $\tau$-hard positive/negative examples in the COCO-Stuff test change change as we change $\tau$.
% \DM{[maybe show examples? car cup bowl sports-ball tie]}
Note, we do not look at distance to $Y=0$ examples; we assume that captions for $Y=0$ images may have little in common, whereas the mean caption for $Y=1$ is a prototypical description of $Y$ ``in context''.
Throughout, we set the threshold $\tau$ for each task so that the number of hard positives and negatives is the same as the CE criterion for that task, to facilitate comparisons.
See Figure \ref{fig:results-qual-two-criteria} for examples of hard positive and negatives chosen by this criterion in comparison to the CE criterion, and Appendix \ref{app:data} for more details.

% Throughout, we use $\tau = 0.25$, which was chosen since it approximately equalizes $P[(X, Y)\  \textrm{is}\ (\alpha, \beta)\textrm{-hard}\  | Y = y] $ across values of $y = 0, 1$.
% \RZ{This definition does not take into account distance to embeddings for Y=0 examples. We can justify this by saying that we are assuming the caption describes the primary content of the image, so the mean caption where the object is present is an average description of the object in its context.} 



% While extractibility is an important factor for context and OOC performance, simply understanding which objects are extractible (or large) in images does not necessarily give us a full picture of context.
% Another important factor to consider is \textit{relevance}: which co-occuring objects are most relevant to the label of interest? 
% We would like to know when are the relevant contextual objects in the image similar to the most commonly seen relevant objects in the training set.
% To estimate this, we can leverage captions provided in the COCO dataset: each image has 5 captions describing the scene content.
% We make the assumption that more relevant contextual information is more likely to be referred to (explicitly or implicitly) in a caption.


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{The number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, there $\tau$ thresholds the caption cosine similarity to the average caption of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}
% \end{figure}


\subsection{\rococo-CE and \rococo-Gist: Selecting Challenge Sets }

\begin{wraptable}{R}{0.45\linewidth}
    \centering
    \input{tables/nhard}
    \caption{Counts of hard positive, hard negative \& positive examples per \rococo\ task.}
    \label{tab:n_hard_examples}
\end{wraptable}
We train binary classifiers to minimize average NLL on each of the 171 classes in COCO-Stuff.
We find that for nearly all tasks, the hard positives and negatives defined by our methods incur higher average loss than positive and negative examples respectively (Fig. \ref{fig:benchmark-hard-pos-neg-task-scatter}), for both the CE and Gist criteria.
This provides some evidence that our criteria are, in fact, identifying examples which are more difficult to classify correctly.

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Positives_NLL.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Negatives_NLL.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Positives_NLL.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Negatives_NLL.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
We find that hard positives/negatives induce higher average loss for both criteria.
Each point is a task in COCO-Stuff: the x- and y-axis values show the average loss achieved by an ERM model on all positives (negatives) and the average loss on hard positives (negatives).
From L to R: CE criterion (positives), CE criterion (negatives), gist criterion (positives), gist criterion (negatives).
% Using the co-occurrence-based method, we find that (0.05, 1)-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
The diagonal line represents where the hard example losses match marginal losses.
} \label{fig:benchmark-hard-pos-neg-task-scatter}
\end{figure}




% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Positives_NLL.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Negatives_NLL.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Using the co-occurrence-based method, we find that (0.05, 1)-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% The diagonal line represents where they are exactly equal, on average.
% } \label{fig:benchmark-hard-pos-neg-task-scatter-area}
% \end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Positives_NLL.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Negatives_NLL.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Using the gist-based method, we find that 0.25-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% The diagonal line represents where they are exactly equal, on average.
% } \label{fig:benchmark-hard-pos-neg-task-scatter-caption}
% \end{figure}




To select candidate OOC tasks for our challenge sets, we select the 12 tasks with the largest difference between average NLL on hard examples (by the CE criterion) and average NLL on all examples, filtering out those tasks without at least 50 hard positives and hard negatives.
% and also those tasks which seem subjectively too similar to ones already chosen (e.g. removed \textrm{sheep} because \textrm{cow} was selected, removed \textrm{wine-glass} because \textrm{cup} was selected).
% To make up the {\rococo\ } benchmark, we take the 12 tasks, with at least 50 hard positives and negatives, that have the largest average difference between loss on (0.05, 0.1)-hard examples and average examples.
% We filtered out a couple of tasks which seemed subjectively too similar to ones already in the benchmark (e.g. removed sheep because cow was in, removed wine glass because cup was in).
% The final task list is: \texttt{car, bowl, boat, fire, airplane, cow, backpack, cup, surfboard, tie, sports\_ball, kite}.
We call these tasks the {\rococo \ } (Naturally-Occurring Out-of-context Challenge) suite (Table \ref{tab:n_hard_examples}). 
We then identify two groups of challenge sets: \rococo-CE, which consists of the hard positive and negative examples on each of the 12 tasks in {\rococo \ } as identified by the CE criterion; and \rococo-Gist, which is the analogous set for the gist criterion.
% Within each task in {\rococo \ }, we identify two challenge sets: \rococo-CE and \rococo-Gist, which consist of the hard positive and negative examples on that task as selected by the CE criterion and the gist criterion, respectively.
This gives us 24 total challenge sets on which to evaluate an ML model's OOC performance.
% : two for each of the 12 aforementioned tasks.

% \DM{Address how I picked these parameters}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_airplane_Hard_Positive.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_airplane_Hard_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_Bowl_Hard_Negative.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_Bowl_Hard_Negative.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{
% To contrast the CE and Gist criteria, we show (L to R):
% % We show the examples where GDRO most outperforms ERM among (L to R): 
% hard positives, CE criterion, \texttt{airplane} task;
% hard positives, Gist criterion, \texttt{airplane} task;
% hard negatives, CE criterion, \texttt{bowl} task;
% hard negatives, Gist criterion, \texttt{bowl} task;
% } \label{fig:results-qual-two-criteria}
% \end{figure}


\paragraph{Contrasting the Two Criteria (Fig. \ref{fig:results-qual-two-criteria}).}
The left two images in Fig. \ref{fig:results-qual-two-criteria} are hard positives on the \texttt{airplane} task.
On the far left, we see the inside of an airplane: this is selected as a hard positive by the CE criteria because there is no sky visible.
On the second left, the sky is visible but the overall scene is unusual; this is selected as a hard positive by the Gist criteria.
The right two images are hard negatives on the \texttt{bowl} task.
On the second right, we see a large dinner with many plates: this is selected as a hard negative by the CE criteria because there is a prominent dining table but no bowls.
On the far right, we see a paper plate on a desk (not a dining table): 
this is selected as a hard negative by the Gist criteria since there is no bowl but it is similar to images where you might expect a bowl.

==> sections/benchmark_new.tex <==
% \section{The {\rococo \ } Benchmark}
\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/kite_Hard_Positives_85911.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/sports_ball_Hard_Positives_79966.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/surfboard_Hard_Positives_342549.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}

\medskip
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/kite_Hard_Negatives_549597.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/sports_ball_Hard_Negatives_187785.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/surfboard_Hard_Negatives_173373.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{Using the co-occurrence/extractibility (CE) criterion, examples of (0.05, 0.1)-hard positives (top row) and negatives (bottom row) for the classes (L to R):  \texttt{kite, sports\_ball, surfboard}.} \label{fig:benchmark-hard-pos-neg-examples}
\end{figure}




\section{Finding Naturally-Occurring OOC Problems} \label{sec:benchmark}

% One major challenge of developing methods for OOC prediction is evaluation: many standard benchmarks rely on synthetic data or a synthetically-created shift: for instance, mixing and matching foregrounds and backgrounds with changing probabilities in the training and test sets.
% However, 

Throughout this paper, we consider the binary prediction task of determining object presence, a problem where relationships between various objects naturally provide helpful context --- given an image $X$, is an object of class $Y$ present or not?
% The label is 1 if at least one instance of the object is present, and 0 otherwise.
% As described in Sec. \ref{sec:intro}, context can play a role in prediction through a number of frequently co-occurring objects and object relationships, in ways that may go beyond what is easily mimicked synthetically.
In order to study how context shifts arise naturally within an existing computer vision benchmark, we propose two methods which leverage annotations to automatically identify candidate OOC examples in the test set.
% We study how context shifts arise within 
% % To understand better how context shifts can arise in practice, we study 
% an existing computer vision benchmark, and propose two methods which leverage existing annotations to automatically identify OOC examples in the test set.
% These OOC sets can play the role of ``stress tests'' for a proposed method.
% \RZ{The paragraph above is a bit repetitive with the intro.}

\subsection{Background: COCO and COCO-Stuff}

The Microsoft Common Objects in COntext dataset (COCO) \citep{lin2014microsoft} is a computer vision dataset consisting of images of natural scenes.
Each image is annotated with instance labels and segmentations for every ``thing'' in the image, as well as several captions describing the content of the scene.
Images usually contain multiple items and as such usually have multiple labels.

However, for the purposes of investigating OOC prediction, many relevant objects are not labelled in COCO; for instance, background objects such as ``sky'' or ``grass'' are not COCO classes.
Fortunately, the COCO-Stuff dataset \citep{caesar2018coco} provides labels and segmentations for all of the ``stuff'' in the images from COCO.
The ``thing'' vs ``stuff'' distinction is a technical one: a thing is an object with a specified size and shape, whereas stuff has no ``defined spatial extent'' \citep{forsyth1996finding}.
Having both thing and stuff labels is essential for understanding model behaviour on OOC examples, since it is exactly these ``stuff'' classes which often (but not always) provide important context cues.
Taken together, the thing and stuff annotations
% provide a coarse but mostly complete, machine-readable description of each image in the COCO dataset, and 
yield a rich sandbox for queries about the role of context in prediction.
For our purposes, COCO-Stuff contains 171 binary tasks for determining object presence (81 thing classes and 90 stuff classes; we ignore the 1 ``unlabelled'' class).

\subsection{Automatically Identifying OOC Examples: Hard Positives and Negatives}

As mentioned in Sec. \ref{sec:intro}, context is hard to define.
We note that different definitions of context correspond to different OOC example-level failure modes.
In this work, we consider two contrasting notions of context: 1. frequently co-occurring, easily extractible objects; and 2. the ``gist'' of a scene.
We operationalize these two notions of context here, presenting two criteria for identifying naturally-occurring OOC prediction problems within the existing COCO(-Stuff) dataset.
We identify both {\it hard positives}, where the class is present despite an unusual context, and {\it hard negatives}, where the class is \textit{not} present, despite a usual context.
% We now present two methods of identifying challenging but naturally-occurring OOC prediction problems, buried within the existing COCO(-Stuff) dataset.
% We explain these methods below and discuss the implicit notions of context each one relies on.
% \DM{Explain why focus on hard positives and negatives: need both labels}

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_airplane_Hard_Positive.pdf}
\caption{hard positive (CE)} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_airplane_Hard_Positive.pdf}
\caption{hard positive (Gist)} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_Bowl_Hard_Negative.pdf}
\caption{hard negative (CE)} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/example_contrast_2/example_contrast_Gist_criterion_Bowl_Hard_Negative.png}
\caption{hard negative (Gist)} \label{fig:b}
\end{subfigure}
\caption{\small{
To contrast the CE and Gist criteria, we show samples from the \texttt{airplane} (L) and \texttt{bowl} (R) tasks.}
% and
% % We show the examples where GDRO most outperforms ERM among (L to R): 
% hard positive, CE criterion, \texttt{airplane} task;
% hard positive, Gist criterion, \texttt{airplane} task;
% hard negative, CE criterion, \texttt{bowl} task;
% hard negative, Gist criterion, \texttt{bowl} task.
} \label{fig:results-qual-two-criteria}
\end{figure}

\subsubsection{Defining Context Using Co-Occurrences and Extractibility}

For an object class $Y$, context cues often come in the form of another object class $C$ that has two properties (cf. \citep{lovering2021predicting}).
% We first consider an object class $C$ which is different from class $Y$, and claim that many useful context cues $C$ have two properties (cf. \citep{lovering2021predicting}).
First, $C$ and $Y$ co-occur frequently \citep{biederman1982scene}.
Second, $C$ is  more \textit{extractible} than $Y$ --- easier to detect.
If $C$ were \textit{less} extractible than $Y$ it would not be a useful cue for detecting $Y$, as a model could detect $Y$ directly.
% For instance, it is frequently observed that CNNs are prone to learning signals about object texture rather than shape \citep{geirhos2018imagenet}.
% A similar argument is made in \citet{lovering2021predicting} when assessing the effect of spurious correlations in an NLP setting.

% Contextual cues can be useful: for instance, a number of object detection models explicitly incorporate it to improve performance [cite].
% However, in deep learning systems, trouble can arise when a contextual cue is much easier to learn than the target class i.e. when it is more \textit{extractible}.
% For instance, it is frequently observed that CNNs are prone to learning signals about object texture rather than shape [cite a few].
% % One important aspect of context is extractibility: how easy it is to learn to detect a context cue's presence in an example.
% % Context cues can help humans improve their processing efficiency [cite], and are often ``shortcuts'' [cite] for model prediction.
% The more extractible a signal is, the more likely it will become a contextual signal that a model relies on [cite simplicity bias] --- and when that signal is not present, the more likely a model will struggle to perform well [cite extractibility.

We can utilize these properties to create candidate context cues $C$ for a class of interest $Y$.
Given segmentations, we can use an object's size within an image as a proxy for extractibility (larger objects tend to be more extractible).
% : the larger the object's bounding box in an image, the more extractible it is.
Let the $Area$ operator take the sum of the areas of all segmentations of instances of that object, or return 0 if the object is not present.
% Consider any feature $C \neq Y$ to be a possible contextual cue for $Y$; for example, let $Y = \texttt{surfboard}, C=\texttt{sea}$.
Then, to estimate from the training set how important of a context variable $C$ is, we can compute $A(C, Y) = \mathds{E}[Area(C) - Area(Y) | Y = 1]$.
When $A(C, Y)$ is larger, this means that when $Y$ is present, $C$ is usually also present, and on average, takes up more of the image than $Y$ does.
When $A(C, Y) > \alpha$, we say that $C$ is an $\alpha$-strong context cue for $Y$ (or just $\alpha$-context for brevity).
We find that many of the contexts identified using this method for large enough $\alpha$ are intuitive.
Some examples of (label, 0.05-context) pairs are: (\texttt{car}, \texttt{road}), (\texttt{bowl}, \texttt{dining\_table}), (\texttt{cow}, \texttt{grass}).

ul
% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
%     \centering
%     \includegraphics[scale=0.4]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
%     \centering
%     \includegraphics[scale=0.4]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{Using the gist criterion, the number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, where $\tau$ thresholds the cosine similarity to the average caption embedding of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}
% \end{subfigure}
% % \caption{Using the gist-based method, we find that 0.25-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% % The diagonal line represents where they are exactly equal, on average.
% % }
% \label{fig:benchmark-descriptive-statistics}
% \end{figure}

% \begin{figure}
% \centering
% \begin{minipage}{.48\textwidth}
%   \centering
%   \includegraphics[scale=0.4]{figs/benchmark/num_tasks_by_num_confs.pdf}
%     \caption{The number of tasks in the COCO-Stuff dataset which have context variables identifiable at each level of $\alpha$.
%     There are 171 total tasks.
%     For instance, this figure shows that there are around 70 tasks with at least one context cue at $\alpha \geq 0.05$, and around 30 tasks with at least five context cues at $\alpha \geq 0$.
%     }
%     \label{fig:benchmark-num-tasks-num-confs}
% \end{minipage}\hspace*{\fill}
% \begin{minipage}{.48\textwidth}
%   \centering
%     \includegraphics[scale=0.4]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{Using the gist criterion, the number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, where $\tau$ thresholds the cosine similarity to the average caption embedding of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}

% \end{minipage}
% \end{figure}




% Fig \ref{fig:benchmark-num-tasks-num-confs} shows that, under this definition, most of the 171 object classes in COCO-Stuff have context cues for $\alpha \geq 0$.
% Note that a 0-context cue is fairly strong: this means that on average, in images where $Y$ is present, $C$ takes up at least as much area as $Y$ does.
% This indicates that there may be a large number of OOC examples hidden in many of these tasks.
% % For instance, over two-thirds of tasks have at least one 0-context cue, and over 1/3 have at least one 0.05-context cue.
% We find that the contexts returned using this method for large enough $\alpha$ are intuitive.
% Some examples of (label, 0.05-context) pairs are: (\texttt{car}, \texttt{road}), (\texttt{bowl}, \texttt{dining\_table}), (\texttt{cow}, \texttt{grass}).
% Additionally, many tasks have more than one context variable: at $\alpha=0$ about 50 tasks have 3, and at $\alpha=0.05$ about 15 tasks have 3.
% Some examples of labels with multiple 0.05-context variables are: (\texttt{surfboard}, [\texttt{sea}, \texttt{sky-other}]),
% (\texttt{tennis-racket}, [\texttt{person}, \texttt{playing-field}]),
% (\texttt{traffic-light}, [\texttt{building-other}, \texttt{road}, \texttt{sky-other}, \texttt{tree}]).
% All of these groupings are intuitive, providing some evidence that this method of isolating context variables may be a usef one.




Using this notion of context, we can then define hard positive and hard negative examples.
We make the simplifying \textit{noisy-or} assumption: that each context cue provides evidence for $Y$, so that the presence of any cue supports $Y$ being present, while the absence of all provides evidence against $Y$'s presence.
% \RZ{We can motivate this particular definition of hard cases by saying something like: under the assumption that each context variable provides evidence for Y, so that the presence of any is enough to support Y being present, while if none are present provides evidence against Y. This is the noisy-or.}
% Then, a hard positive occurs when no context variable is present but $Y = 1$, and a hard negative occurs when some context variable is present, but $Y = 0$.
Given some image, we can define an ($\alpha, \beta$)-hard positive or negative.
If $Y=1$, and for all $\alpha$-context cues $C$, we have $Area(C) < \beta$ in this image (and there is at least one $\alpha$-context cue), then the example is an ($\alpha, \beta$)-hard positive.
Alternatively, if $Y=0$, and there exists some $\alpha$-context variable $C$ such that $Area(C) > \beta$, then the example is an ($\alpha, \beta$)-hard negative.
We will call this method the co-occurrence/extractibility (CE) criterion (see Fig \ref{fig:benchmark-hard-pos-neg-examples} for examples).
% In Fig \ref{fig:benchmark-hard-pos-neg-examples} we show examples of hard positive and hard negative images in COCO-Stuff.
Throughout, we use $\alpha=0.05, \beta=1$ unless otherwise noted; these parameters were chosen since they approximately equalize $P[(X, Y)\ \textrm{is}\ (\alpha, \beta)\textrm{-hard} \ | Y = y]$ across $y = 0, 1$.
See Appendix \ref{app:data} for more details.

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/proportion_hard_positives_by_area.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/proportion_hard_negatives_by_area.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Across a range of $\alpha, \beta$, the percentage of hard positive/negative examples (L/R) in the test set which are $(\alpha, \beta)$-hard.
% } \label{fig:benchmark-hard-pos-neg-examples-area}
% \end{figure}

% Fig \ref{fig:benchmark-hard-pos-neg-examples-area} shows that hard positive/negative examples are numerous in the data.
% For instance, we see that at the (0.05, 0.1) level, about 10\% of all possible (object, category) pairs are hard positives, and a similar number for hard negatives.
% % Alternatively, in Fig [fig], we can see that about 50\% of test images qualify as hard positives in some category, and about 85\% of test images qualify as hard negatives in some category.

\subsubsection{Defining Context Using Gist}

We now turn to a broader notion of context, that of the ``gist'' of a scene \citep{torralba2003contextual}, or its overall semantic content.
This is something that humans are able to recognize easily \citep{larson2014spatiotemporal}, but goes beyond object frequency and extractibility.
When an object is present in a scene whose gist is very different from the scenes the object was present in at training time, this may create a large challenge for OOC prediction.


We here describe our method for estimating gist shift, which we call the gist criterion.
We leverage caption annotation data in COCO (each image has 5 caption sentences), making the assumption that information in a caption captures the gist of a scene.
We then take an SBERT embedding \citep{reimers2019sentence} of each available image caption for an image, and average these embeddings to get a single embedding for each image.
Then, for a given image and some target label $Y$, we can look at the cosine similarity between that image's embedding and the average embedding across all training images with $Y=1$.
If this similarity is below some threshold $\tau$, and $Y = 1$ for the test image, it is a $\tau$-hard positive;
%Similarly, 
if this similarity is above $\tau$, and $Y = 0$ for the test image, it is a $\tau$-hard negative.
% Fig. \ref{fig:benchmark-hard-pos-neg-examples-caption} shows how the number of $\tau$-hard positive/negative examples in the COCO-Stuff test change change as we change $\tau$.
% \DM{[maybe show examples? car cup bowl sports-ball tie]}
Note, we do not look at distance to $Y=0$ examples; we assume that captions for $Y=0$ images may have little in common, whereas the mean caption for $Y=1$ is a prototypical description of $Y$ ``in context''.
Throughout, we set the threshold $\tau$ for each task so that the number of hard positives and negatives is the same as the CE criterion for that task, to facilitate comparisons.
See Figure \ref{fig:results-qual-two-criteria} for examples of hard positive and negatives chosen by this criterion in comparison to the CE criterion, and Appendix \ref{app:data} for more details.

% Throughout, we use $\tau = 0.25$, which was chosen since it approximately equalizes $P[(X, Y)\  \textrm{is}\ (\alpha, \beta)\textrm{-hard}\  | Y = y] $ across values of $y = 0, 1$.
% \RZ{This definition does not take into account distance to embeddings for Y=0 examples. We can justify this by saying that we are assuming the caption describes the primary content of the image, so the mean caption where the object is present is an average description of the object in its context.} 



% While extractibility is an important factor for context and OOC performance, simply understanding which objects are extractible (or large) in images does not necessarily give us a full picture of context.
% Another important factor to consider is \textit{relevance}: which co-occuring objects are most relevant to the label of interest? 
% We would like to know when are the relevant contextual objects in the image similar to the most commonly seen relevant objects in the training set.
% To estimate this, we can leverage captions provided in the COCO dataset: each image has 5 captions describing the scene content.
% We make the assumption that more relevant contextual information is more likely to be referred to (explicitly or implicitly) in a caption.


% \begin{figure}
%     \centering
%     \includegraphics[scale=0.5]{figs/benchmark/proportion_hard_examples_by_caption.pdf}
%     \caption{The number of $\tau$-hard positive/negative examples in the COCO-Stuff test set as a proportion of all positive/negative examples, there $\tau$ thresholds the caption cosine similarity to the average caption of that category in the training set.
%     }
%     \label{fig:benchmark-hard-pos-neg-examples-caption}
% \end{figure}


\subsection{\rococo-CE and \rococo-Gist: Selecting Challenge Sets }

\begin{wraptable}{R}{0.45\linewidth}
    \centering
    \input{tables/nhard}
    \caption{Counts of hard positive, hard negative \& positive examples per \rococo\ task.}
    \label{tab:n_hard_examples}
\end{wraptable}
We train binary classifiers to minimize average NLL on each of the 171 classes in COCO-Stuff.
We find that for nearly all tasks, the hard positives and negatives defined by our methods incur higher average loss than positive and negative examples respectively (Fig. \ref{fig:benchmark-hard-pos-neg-task-scatter}), for both the CE and Gist criteria.
This provides some evidence that our criteria are, in fact, identifying examples which are more difficult to classify correctly.

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Positives_NLL.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Negatives_NLL.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Positives_NLL.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Negatives_NLL.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
We find that hard positives/negatives induce higher average loss for both criteria.
Each point is a task in COCO-Stuff: the x- and y-axis values show the average loss achieved by an ERM model on all positives (negatives) and the average loss on hard positives (negatives).
From L to R: CE criterion (positives), CE criterion (negatives), gist criterion (positives), gist criterion (negatives).
% Using the co-occurrence-based method, we find that (0.05, 1)-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
The diagonal line represents where the hard example losses match marginal losses.
} \label{fig:benchmark-hard-pos-neg-task-scatter}
\end{figure}




% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Positives_NLL.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_area_Hard_Negatives_NLL.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Using the co-occurrence-based method, we find that (0.05, 1)-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% The diagonal line represents where they are exactly equal, on average.
% } \label{fig:benchmark-hard-pos-neg-task-scatter-area}
% \end{figure}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Positives_NLL.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/task_loss_scatter_by_caption_Hard_Negatives_NLL.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{Using the gist-based method, we find that 0.25-hard positives/negatives are harder, on average, than positives/negatives (L/R), for nearly every task of which has at least 1 hard positive/negative.
% The diagonal line represents where they are exactly equal, on average.
% } \label{fig:benchmark-hard-pos-neg-task-scatter-caption}
% \end{figure}




To select candidate OOC tasks for our challenge sets, we select the 12 tasks with the largest difference between average NLL on hard examples (by the CE criterion) and average NLL on all examples, filtering out those tasks without at least 50 hard positives and hard negatives.
% and also those tasks which seem subjectively too similar to ones already chosen (e.g. removed \textrm{sheep} because \textrm{cow} was selected, removed \textrm{wine-glass} because \textrm{cup} was selected).
% To make up the {\rococo\ } benchmark, we take the 12 tasks, with at least 50 hard positives and negatives, that have the largest average difference between loss on (0.05, 0.1)-hard examples and average examples.
% We filtered out a couple of tasks which seemed subjectively too similar to ones already in the benchmark (e.g. removed sheep because cow was in, removed wine glass because cup was in).
% The final task list is: \texttt{car, bowl, boat, fire, airplane, cow, backpack, cup, surfboard, tie, sports\_ball, kite}.
We call these tasks the {\rococo \ } (Naturally-Occurring Out-of-context Challenge) suite (Table \ref{tab:n_hard_examples}). 
We then identify two groups of challenge sets: \rococo-CE, which consists of the hard positive and negative examples on each of the 12 tasks in {\rococo \ } as identified by the CE criterion; and \rococo-Gist, which is the analogous set for the gist criterion.
% Within each task in {\rococo \ }, we identify two challenge sets: \rococo-CE and \rococo-Gist, which consist of the hard positive and negative examples on that task as selected by the CE criterion and the gist criterion, respectively.
This gives us 24 total challenge sets on which to evaluate an ML model's OOC performance.
% : two for each of the 12 aforementioned tasks.

% \DM{Address how I picked these parameters}

% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_airplane_Hard_Positive.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_airplane_Hard_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_CE_criterion_Bowl_Hard_Negative.pdf}
% % \caption{First subfigure} \label{fig:a}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.25\textwidth}
% \includegraphics[width=\linewidth]{figs/benchmark/example_contrast/example_contrast_Gist_criterion_Bowl_Hard_Negative.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
% \caption{
% To contrast the CE and Gist criteria, we show (L to R):
% % We show the examples where GDRO most outperforms ERM among (L to R): 
% hard positives, CE criterion, \texttt{airplane} task;
% hard positives, Gist criterion, \texttt{airplane} task;
% hard negatives, CE criterion, \texttt{bowl} task;
% hard negatives, Gist criterion, \texttt{bowl} task;
% } \label{fig:results-qual-two-criteria}
% \end{figure}


\paragraph{Contrasting the Two Criteria (Fig. \ref{fig:results-qual-two-criteria}).}
The left two images in Fig. \ref{fig:results-qual-two-criteria} are hard positives on the \texttt{airplane} task.
On the far left, we see the inside of an airplane: this is selected as a hard positive by the CE criteria because there is no sky visible.
On the second left, the sky is visible but the overall scene is unusual; this is selected as a hard positive by the Gist criteria.
The right two images are hard negatives on the \texttt{bowl} task.
On the second right, we see a large dinner with many plates: this is selected as a hard negative by the CE criteria because there is a prominent dining table but no bowls.
On the far right, we see a paper plate on a desk (not a dining table): 
this is selected as a hard negative by the Gist criteria since there is no bowl but it is similar to images where you might expect a bowl.

==> sections/conclusion.tex <==
\section{Discussion} \label{sec:conclusion}

\paragraph{Limitations \& Impacts.}
The idea of computationally identifying OOC examples is necessarily limited: by their nature, OOC examples are exceptions to rules, and there will always be OOC examples which can only be discovered through qualitative examination.
Further, the task chosen for our benchmark was chosen for simplicity of analysis in a research context rather than real world significance --- outputting segmentations or many-way classification may be more applicable to most applications.
We hope that the impact of our work is to enable better evaluation of model performance on atypical or under-represented examples, both through usage of these challenge sets and ones inspired by the ideas presented here.
However, the usage of benchmarks can have downsides where standardized performance metrics are prioritized over fundamental advances in modelling which are not captured in those metrics.
In various applications of interest, results may need to be reported across a number of different metrics since this gives a clearer picture of model performance --- AUC may not always be a (or the most) relevant metric.


\paragraph{Conclusion \& Looking Forward.}
Here, we hope to accent several aspects of this work.
% There are several aspects of this work we would like to bring to the fore here.
Firstly, we think that the notion of gist shift is an important direction for OOC research --- we found it to be a very challenging problem with no one method standing out above the others.
Fundamentally, a model which maintains performance even when the gist of the scene is unusual will be solving one of the hardest aspects of the OOC problem.
% --- for instance, explicating and testing different notions of context.
Another is the relationship between calibration and robustness: both are properties that we generally desire of ``trustworthy'' models, but 
%we see in Sec. \ref{sec:experiments} the 
our results show that these two goals are not always practically aligned.
% models which are more robust in OOC situations sometimes suffer from a calibration perspective, whereas ERM displays superior calibration even on OOC examples.

Finally, we would like to highlight the idea systematizing OOC evaluation, whether this is through automatic discovery of OOC example through annotations or some other means.
This not only enables the scalable creation of challenge sets, but allows for faster generation and exploration of new hypotheses about the type of context shifts that models struggle on.
We hope that methods of this type can be applied elsewhere to better understand the challenges of OOC prediction.

% One noteworthy aspect of this work is the idea of automatic discovery of OOC examples.
% This is useful tool for probing 

% We present the {\rococo} challenge sets, groups of examples found in the COCO-Stuff test set which are OOC with respect to its training set.

% After running a number of methods 


% \DM{Write this}

% \begin{itemize}
%     \item Compare to WILDS results
%     \item Unfortunate there are tradeoffs
%     \item Calibration
%     \item Interpretability
%     \item Other methods
% \end{itemize}



==> sections/intro.tex <==
\section{Introduction} \label{sec:intro}

People often find context %can be
useful for prediction, %in humans, 
both for improving accuracy and processing efficiency \citep{chun2000contextual}.
However, deep learning systems frequently over-rely on context cues \citep{geirhos2020shortcut,geirhos2018imagenet,lovering2021predicting}, which can lead to poor performance on out-of-context (OOC) examples, when contextual information is misleading.
% about the correct prediction.
% Fields such as robust learning \citep{hu2018does,duchi2016variance,srivastava2020robustness} and domain generalization \citep{creager2020environment,arjovsky2019invariant} have tackled the OOC problem, and 
% a growing number of practical anecdotes indicate the problem may be ubiquitous \citep{oakden2020hidden,winkler2019association}.
Indeed, the OOC prediction problem is a challenging one to solve and define: in a natural image, ``context'' can be complex and high-dimensional, including aspects of object relationships \citep{torralba2003contextual}, image backgrounds \citep{xiao2020noise}, experimental settings \citep{peters2016causal}, or world models \citep{bobick1995using}.
%\RZ{Do we mean challenging to predict in OOC conditions, or challenging to define the context?}
% Many methods for OOC prediction have been proposed, in particular from fields such as robust learning \citep{hu2018does,duchi2016variance,srivastava2020robustness} and domain generalization \citep{creager2020environment,arjovsky2019invariant}.

% A number of practical stories demonstrate that in the standard course of 

However, machine learning researchers rarely evaluate OOC prediction methods in ways that capture the full complexity of practical context shifts.
Many standard benchmarks rely on sharp, synthetically-created shifts in one salient feature, e.g., image background or color \citep{kim2019learning,xiao2020noise,sagawa2019distributionally}.
% , or synthetic image corruptions \citep{michaelis2019benchmarking,hendrycks2019benchmarking}.
% Other datasets represent more natural OOC settings but
% are highly curated/
Meanwhile, other datasets represent more natural OOC settings but are
small \citep{choi2011tree}, do not contain a training set \citep{barbu2019objectnet}, or entail significant domain knowledge \citep{koh2020wilds}.
While these are significant and valuable works, a closer analogue to the OOC problems that arise in the standard research model development cycle might more scalably provide insights into the challenges faced by current approaches.

% one might suppose that a dataset 
% one can imagine the need for a closer analogue to the OOC problems that arise in the standard model development cycle
% While these are significant and valuable works, they do not necessarily provide insight into 
% they do not provide the clearest window for interpretation at scale of the OOC problems faced by current models.
% While each of these are useful datasets, each involves a departure
% While understanding these types of synthetic shifts is important, it is unclear whether they faithfully represent practically-arising OOC problems.

% However, due to the complexity of context shifts, evaluating the OOC performance of a method is challenging --- many standard benchmarks rely on sharp, synthetically-created shift in one salient feature, e.g. image background or color \citep{kim2019learning,xiao2020noise,sagawa2019distributionally}, or synthetic image corruptions \citep{michaelis2019benchmarking,hendrycks2019benchmarking}.
% While understanding these types of synthetic shifts is important, it is unclear whether they faithfully represent practically-arising OOC problems.
% Other datasets represent more natural OOC settings but are highly curated \citep{barbu2019objectnet}, small \citep{choi2011tree}, or entail significant domain knowledge \citep{koh2020wilds}.
% Other datasets aim to represent more natural shifts but may be challenging to use in standard model development cycles due to focus on non-standard domains \citep{koh2020wilds}, a lack of a training set \citep{barbu2019objectnet}, or small size \citep{choi2011tree}.

In this work, we introduce methods for identifying sets of OOC problems which naturally arise in existing computer vision datasets, and use these methods to expose OOC ``challenge sets'' \citep{isabelle2017challenge} within an existing benchmark.
% In this work, we uncover a set of OOC problems which naturally arise in an existing computer vision benchmark, exposing OOC ``challenge sets'' \citep{isabelle2017challenge} within an existing dataset.
We focus on the task of determining object presence in an image, a problem where relationships between various objects naturally provide helpful context.
By identifying candidate OOC examples at scale, we enable quantitative and qualitative analysis of the OOC problems that are \textit{already present}, gaining a clearer window into both the performance of current approaches, as well as opportunities for further improvement.
% Through quantitative and qualitative analysis of the difficult OOC examples that are \textit{already present} in a vision dataset, we get a clearer window into both the performance of current approaches, as well as opportunities for further improvement.
% we can gain insight into the challenges faced by current approaches in the OOC setting.
% \RZ{Could motivate why consider detection task - considering the problem of determining object presence, in the presence or absence of context cues specific to that object class}.
% We leverage existing annotations to define the notion of ``hard positives'' and ``hard negatives'', and automatically identify difficult groups of OOC examples as challenge sets on a number of tasks.
% Furthermore, we compare the performance of various methods on these tasks and explore the tradeoffs that occur when using different types of apporaches to OOC prediction.
Our contributions are as follows:
\begin{itemize}
    \item We present {\rococo} (Naturally-Occurring Out-of-context Challenge sets), a suite of ``challenge sets'' for evaluating performance on naturally-arising OOC problems;
    \item  We introduce novel methods for automatically identifying OOC challenge sets from existing annotated data, and define concepts of ``hard positives'' and ``hard negatives'' in the OOC setting; and
    % Using two contrasting notions of context, we introduce novel methods of automatically uncovering challenge sets from existing annotated data, defining concepts of ``hard positives'' and ``hard negatives'' in the OOC setting; and
    % Based on two notions of context, we define two general methods which use annotations to automatically create challenge sets from an image dataset; and
    \item We analyze the performance of several methods from the robust learning literature on these challenge sets, and explore the tradeoffs inherent in different approaches.
\end{itemize}

% There is growing evidence to show that deep learning systems rely heavily on context cues for maximizing predictive performance \citep{oakden2020hidden,winkler2019association,geirhos2020shortcut,geirhos2018imagenet,lovering2021predicting}.
% % This is not inherently a bad thing: for instance, context cues are important for human prediction and improve processing efficiency \citep{chun2000contextual}.
% % In fact, outside of deep learning, a number of approaches have explicitly incorporated contextual information to improve performance \citep{choi2011tree,murphy2003using,torralba2003contextual}.
% However, deep models frequently exhibit over-reliance on these cues, which can lead to poor performance on out-of-context (OOC) examples, when some object of interest is present but the context cues are not.

% The OOC prediction problem is as difficult as the definition of context itself.
% In a natural image, ``context'' can be defined in a myriad of ways, including using object relationships \citep{xiao2020noise}, image backgrounds \citep{xiao2020noise}, experimental settings \citep{peters2016causal}, or world models \citep{bobick1995using}.
% Since context cues can be multi-faceted and high-dimensional, 
% % they are almost certain to be under-sampled in a training set.
% % As such,
% we expect OOC problems to arise frequently in practice.
% To this end, many methods for OOC prediction have been proposed, in particular from fields such as robust learning \citep{hu2018does,duchi2016variance,srivastava2020robustness} and domain generalization \citep{creager2020environment,arjovsky2019invariant}.
% However, many of these methods are evaluated on synthetic or semi-synthetic data: for instance, datasets where a sharp, synthetically-created shift in one salient feature, e.g. image background or color, defines the OOC set \citep{kim2019learning,xiao2020noise,sagawa2019distributionally}.
% While understanding these types of synthetic shifts is important,
% it is unclear whether they faithfully represent
% practically-arising OOC problems, which may involve shifts as widely-varying and complex as the contexts themselves.
% %  is important to understand how these OOC problems may arise in practice, and how methods may perform on them.

% In this work, we explore the question of what ``naturally-occurring'' OOC problems look like, by identifying the existence of OOC ``challenge sets'' \citep{isabelle2017challenge} within an existing computer vision benchmark.
% We focus on the task of determining object presence in an image, a problem where the relationships between various objects naturally provides helpful context.
% % \RZ{Could motivate why consider detection task - considering the problem of determining object presence, in the presence or absence of context cues specific to that object class}.
% We leverage existing annotations to define the notion of ``hard positives'' and ``hard negatives'', and automatically identify difficult groups of OOC examples as challenge sets on a number of object detection tasks.
% Furthermore, we compare the performance of various methods on these tasks and explore the tradeoffs that occur when using different types of models from the robust learning literature.
% Our contributions are as follows:
% \DM{Is NOOCH a better name than ROCOCO?}
% \begin{itemize}
%     \item We present {\rococo}, a suite of ``challenge sets'' for evaluating a vision model's performance on naturally-arising OOC problems;
%     \item We introduce notions of ``hard positives'' and ``hard negatives'' in the OOC context, and give two methods for automatically identifying these examples using annotated data; and
%     % Based on two notions of context, we define two general methods which use annotations to automatically create challenge sets from an image dataset; and
%     \item We analyze the performance of several methods from across the robust learning literature on these challenge sets, and explore the tradeoffs inherent in different approaches.
% \end{itemize}

% However, these approaches often assume that the context is represented by an \textit{environment} variable (essentially a one-hot encoding of context), which can underspecify context shift in practice, due to the potential complexity of context cues.


% Contextual information is an important aspect of prediction, both in humans and machines [cite several].
% In human visual perception, context cues are often used to improve efficiency of processing; as such they can be helpful for efficiency, or harmful if not present [cite].
% This is the same in machines: in particular, the challenge of making good predictions out-of-context (OOC) is essential to the project of machine learning, and one which has received attention under a number of names, including domain generalization [cite], OOD prediction [cite], and 0-shot/meta learning [cite].

% In practice, OOC prediction problems are difficult and numerous because context can be complex.
% For instance, while we can think of the ``background'' of an image as being the context, the number of degrees of freedom that make up the background are enormous --- images can be under a wide range of lighting conditions, with many different types of objects present in various arrangements.
% Viewed this way, the context variable is complex and high-dimensional, which essentially guarantees that in practice, some contexts will be under-sampled at training time, and test-time shifts in context can be quite complex.
% In this regard, several previous approaches to the OOC problem fall short.
% A range of domain generalization algorithms represent context as a one-hot \textit{environment} variable [cite], which for most cases under-specifies the type of context shift we care about.
% Additionally, a number of proposed benchmarks for the OOC task are built around synthetic or semi-synthetic biases/shifts, which can be much larger or more jarring than realistic context shifts.

% In this work, we present a benchmark for OOC prediction which, rather than relying on synthetic shifts, is centred around naturally occurring context shifts that arise in an existing object recognition dataset.
% Our benchmark leverages existing annotations to present a methodology for identifying expected difficult context shifts, and probing which examples may suffer from OOC problems, in order to better evaluate algorithmic performance.
% We benchmark a range of methods in different categories on this dataset and contrast their behaviour on difficult OOC test examples, exploring test performance, calibration, and probing the pros and cons of adaptivity and invariance as different approaches to OOC prediction problems.

% Our contributions are as follows:
% \begin{itemize}
%     \item We introduce the \rococo benchmark for OOC prediction, consisting of naturally occurring contextual shifts in a binary object detection task
%     \item We evaluate a number of methods on this benchmark, finding that current robust environment-based approaches fall short in a number of ways, including calibration, excessive invariance, and under-performance on ``hard'' examples (GDRO/IRM/upsampling??)
%     \item We propose a number of common approaches in the ML literature for mitigating these issues, including dynamic re-weighting of hard examples, auxiliary tasks, and adapting parameters to side information
% \end{itemize}

% In particular, we consider the (hard) problem of ``out-of-context'' (OOC) prediction.
% Contextual elements can be complex, high-dimensional and/or structured.
% As such, it is almost assured that certain contextual configurations may be undersampled in any observed dataset, or may not be observed at all - whether through sampling variance or bias.
% In these cases, there are many examples of models being misled by OOC examples at test time [cite].
% In particular, this tends to occur when the contextual cue is more \textit{extractible} than the signal we care about [cite].
% Due to the simplicity bias of many DNNs (and possibly other ML systems), the model may learn to predict the context rather than the label, leading to poor OOC prediction.

% Recently, a number of works have tried to approach the OOC prediction problem from a specific angle - by using contextual information in the form of \textit{environments} (or groups) [cite].
% These environments were originally proposed with a causal interpretation - each represents a different intervention on the data-generating causal graph - however, in practice they are often simply thought of as meaningful partitions of the data.
% Experimentally, these environments are represented as a one-hot variable, often referring to a single feature of the data, such as the color [cite] or the background [cite].
% However, context is a complicated, high-dimensional thing which cannot necessarily be fully captured through such partitioning.
% Additionally, many works explore this phenomenon using a large, synthetically created shift [cite].
% This is reasonable, as it is easier to detect differences in, say, robustness to spurious correlation in this setting, but often contextual shifts can be more subtle and occur throughout many properties of the input.

% In this work, we investigate the notion of OOC prediction in a more realistic setting; exploring an existing dataset, identifying naturally occurring context shifts, and using these to evaluate the performance of various learning approaches.

==> sections/intro_new.tex <==
\section{Introduction} \label{sec:intro}

People often find context %can be
useful for prediction, %in humans, 
both for improving accuracy and processing efficiency \citep{chun2000contextual}.
However, deep learning systems frequently over-rely on context cues \citep{geirhos2020shortcut,geirhos2018imagenet,lovering2021predicting}, which can lead to poor performance on out-of-context (OOC) examples, when contextual information is misleading.
% about the correct prediction.
% Fields such as robust learning \citep{hu2018does,duchi2016variance,srivastava2020robustness} and domain generalization \citep{creager2020environment,arjovsky2019invariant} have tackled the OOC problem, and 
% a growing number of practical anecdotes indicate the problem may be ubiquitous \citep{oakden2020hidden,winkler2019association}.
Indeed, the OOC prediction problem is a challenging one to solve and define: in a natural image, ``context'' can be varied, complex and high-dimensional \citep{torralba2003contextual,xiao2020noise,peters2016causal,bobick1995using}.
% , including aspects of object relationships \citep{torralba2003contextual}, image backgrounds \citep{xiao2020noise}, experimental settings \citep{peters2016causal}, or world models \citep{bobick1995using}.
%\RZ{Do we mean challenging to predict in OOC conditions, or challenging to define the context?}
% Many methods for OOC prediction have been proposed, in particular from fields such as robust learning \citep{hu2018does,duchi2016variance,srivastava2020robustness} and domain generalization \citep{creager2020environment,arjovsky2019invariant}.

% A number of practical stories demonstrate that in the standard course of 
As such, realistic evaluation of a prediction method's OOC performance is challenging.
Manual evaluation of ``corner cases'' by domain experts may (always) be the gold standard, but given the rise of larger models and datasets \citep{kaplan2020scaling}, there is a need for approaches to OOC evaluation which are realistic, interpretable, and scalable.
To this end, a number of benchmarks have been created which rely on some type of simple auxiliary information to determine what is OOC.
For instance, many standard benchmarks use a sharp, synthetically-created shifts in one salient feature, e.g., image background or color \citep{kim2019learning,xiao2020noise,sagawa2019distributionally}.
% Many standard benchmarks do not capture the full complexity of practical context shifts, instead relying on sharp, synthetically-created shifts in one salient feature, e.g., image background or color \citep{kim2019learning,xiao2020noise,sagawa2019distributionally}.
Other datasets leverage different types of simple annotations;
\citet{koh2020wilds} uses (among others) timestamps or geographic information, and \citet{hendrycks2021natural} uses the loss obtained by an ensemble of models.
In each of these datasets, there is structure \textit{a priori} over the auxiliary information which yields some notion of which examples are OOC --- for instance, unusual values of the auxiliary information are considered OOC.

When viewed in this way, it seems that it is the nature of the annotated auxiliary information in question which bottlenecks the usefulness of an OOC dataset.
For instance, using synthetic auxiliary information (such as a synthetic background) yields a dataset which does not capture the full complexity of practical context shifts.
Having a distributional shift which is defined by a real, but low dimensional auxiliary variable (e.g. timestamps) does not yield rich information about the type of failure which occurred on a specific test example, and additionally limits the complexity of shifts which can be tested for.


In this work, we generalize the method used in prior OOC benchmarks to much richer classes of annotations. 
We introduce methods for automatically identifying sets of OOC problems which naturally arise in existing computer vision datasets, and use these methods to expose OOC ``challenge sets'' \citep{isabelle2017challenge} within an existing benchmark.
We show how such methods can be adapted to correspond to different classes of example-level failure modes through differing notions of context.
% In this work, we uncover a set of OOC problems which naturally arise in an existing computer vision benchmark, exposing OOC ``challenge sets'' \citep{isabelle2017challenge} within an existing dataset.
% We focus on the task of determining object presence in an image, a problem where relationships between various objects naturally provide helpful context.
By identifying candidate OOC examples at scale, we enable more realistic and targeted  analysis of models' OOC performance, gaining a clearer window into both current approaches, as well as opportunities for further improvement.
% Through quantitative and qualitative analysis of the difficult OOC examples that are \textit{already present} in a vision dataset, we get a clearer window into both the performance of current approaches, as well as opportunities for further improvement.
% we can gain insight into the challenges faced by current approaches in the OOC setting.
% \RZ{Could motivate why consider detection task - considering the problem of determining object presence, in the presence or absence of context cues specific to that object class}.
% We leverage existing annotations to define the notion of ``hard positives'' and ``hard negatives'', and automatically identify difficult groups of OOC examples as challenge sets on a number of tasks.
% Furthermore, we compare the performance of various methods on these tasks and explore the tradeoffs that occur when using different types of apporaches to OOC prediction.
Our contributions are as follows:
\begin{itemize}
    \item We present {\rococo} (Naturally-Occurring Out-of-context Challenge sets), a suite of ``challenge sets'' for evaluating performance on naturally-arising OOC problems;
    \item  We introduce novel methods for automatically identifying OOC challenge sets from existing annotated data which operationalize and contrast two notions of ``context'', and define concepts of ``hard positives'' and ``hard negatives'' in the OOC setting; and
    % Using two contrasting notions of context, we introduce novel methods of automatically uncovering challenge sets from existing annotated data, defining concepts of ``hard positives'' and ``hard negatives'' in the OOC setting; and
    % Based on two notions of context, we define two general methods which use annotations to automatically create challenge sets from an image dataset; and
    \item We analyze the performance of several methods from the robust learning literature on these challenge sets, and explore the tradeoffs inherent in different approaches.
\end{itemize}


==> sections/methods.tex <==

\section{Methods} \label{sec:methods}

% In Sec. \ref{sec:experiments}, we test a number of methods on the {\rococo \ } challenge sets, and provide analysis of their performance.
% We focus on five methods:
% , which represent a range of different philosophies on OOC prediction:
% expected risk minimization (ERM), group DRO (GDRO) \citep{sagawa2019distributionally}, invariant risk minimization (IRM) \citep{arjovsky2019invariant} , conditional value at risk minimization (CVaR) \citep{rockafellar2002conditional}, and focal loss \citep{lin2017focal}.
We choose to focus on five methods which provide a useful contrast between different approaches to OOC prediction. 
Expected risk minimization (\textbf{ERM}) is the standard loss function in ML systems; as shown by \citet{gulrajani2020search}, it can be difficult to beat on domain generalization problems.
Group DRO (\textbf{GDRO}) \citep{sagawa2019distributionally} and invariant risk minimization (\textbf{IRM}) \citep{arjovsky2019invariant} are popular examples of environment-based learning methods.
In contrast to these, we also look at two \textit{adaptive} methods, which do not require auxiliary information at training time and instead attempt to adaptively determine the most difficult examples at each step.
Conditional value at risk minimization (\textbf{CVaR}) \citep{rockafellar2002conditional}, like GDRO, can be thought of as an example of distributionally robust optimization, a common approach in the robustness literature \citep{duchi2021statistics} --- however, in CVaR we minimize the loss for a worst case distribution over examples at each step, and in GDRO we minimize the worst-case loss among pre-defined groups.
\textbf{Focal} loss \citep{lin2017focal} is not necessarily commonly used in the OOC setting; however, it is a widely used reweighting technique in computer vision; a class of approaches common in OOC prediction \citep{shimodaira2000improving}.
See App. \ref{app:other-methods} for information on other methods we experimented with but did not include here, including methods that adapt parameters to context and methods which aim to predict context.
We found the methods we included here had the best results overall, on the standard and hard examples. %\RZ{Could justify the selection of these -- we found the methods here to have the best results overall, on the standard and hard examples. And what do you mean by adapt parameters to context?}


Throughout, we use the following notation.
We are given a dataset $\{x_i, y_i\}_{i=1}^n$ with inputs and target labels respectively, and possibly some side information $\{ c_i \}_{i=1}^n$ as well (e.g. environment variables).
If side information is available, we assume it is available at training time but not necessarily test time.
We are aiming to learn a function $f: \mathds{X} \longrightarrow \mathds{Y}$.
We assume $\ell$ to be the the example-wise cross-entropy loss function, and that 
% For all methods, we our function $f$ is a Resnet-50, trained with SGD (learning rate = 1e-4 and momentum = 0.9, which we found to work the best for ERM).

\subsection{Expected Risk Minimization}
Expected risk minimization (ERM) is the standard paradigm for training ML models.
In ERM, we minimize the mean loss $\ell$ on the training set, plus potentially some data-independent regularizer $\mathcal{R}$:
\begin{equation}
    \mathcal{L}_{ERM}(f) = \frac{1}{n} \sum_{i=1}^n \ell(f(x_i), y_i) + \mathcal{R}(f)
\end{equation}

% We can examine three types of ERM models: 1) trained from scratch, 2) finetuned from Imagenet pre-trained weights, and 3) logistic regression on top of pre-trained Imagenet features.
% \RZ{Small rewording}: 1) logistic regression on top of pre-trained Imagenet features; 2) logistic regression on top of pre-trained Imagenet features; 3) logistic regression on top of Imagenet features, finetuned.
% Since we found the finetuning from Imagenet pre-training worked the best across nearly all metrics, we used that initialization procedure for all other methods as well.

% \begin{itemize}
%     \item ERM, trained from scratch
%     \item ERM, image net pre-trained
%     \item ERM, logistic regression on pretrained representations
%     \item Footnote: ERM, learning rate tuning
% \end{itemize}

\subsection{Environment-Based Methods}
One common setting is where the side information $c_i$ for each example is a one-hot variable, representing an \textit{environment}.
The notion of environments for robust learning was originally given with causal motivation \citep{peters2016causal}, where each value of $c$ represents a different intervention on the underlying causal graph.
However, this type of grouping procedure can be used completely separately from the causal context, and so we just consider it to represent some informative partition of our data, which is defined as an input at training time.
Here, $c \in \{ 1 \dots C \}$ is an integer or a one-hot encoded variable.
We will use the following shorthand to describe the average loss for a group:
\begin{equation}
    \ell_c (f) = \frac{1}{n_c} \sum_{i=1}^{n} \ell(f(x_i), y_i) \one \{ c_i = c \}
\end{equation}
% We consider two popular environment-based learning algorithms.

\paragraph{Group DRO.}
The first environment-based method we consider is Group Distributionally Robust Optimization (GDRO) \citep{sagawa2019distributionally}, which aims to minimize the loss on the worst of $C$ partitions, with partition $c$ of size $n_c$, and group adjustment hyperparameter $K$:
\begin{equation}
    \mathcal{L}_{GDRO}(f) = \underset{c \in \{ 1 \dots C \}}{\max} \Big\{  \ell_c (f) + \frac{K}{\sqrt{n_c}}  \Big\} + \mathcal{R}(f)
\end{equation}
This loss aims to ensure that no group's loss is that bad, and the group adjustment term ensures greater focus on smaller groups, which may otherwise be ignored.

\paragraph{IRM.}
The second environment-based method we consider is invariant risk minimization (IRM) \citep{arjovsky2019invariant}:
% , which uses the following loss function
\begin{equation}
    \mathcal{L}_{IRM}(f) = \sum_{c=1}^C  \ell_c (f) + \lambda \| \nabla_{w | w=1} \ell_c (w \cdot f) \| + \mathcal{R}(f)
\end{equation}
The second term here is a gradient penalty on the output of $f$, $w$ is a constant multiplier on the output of $f$, and $\lambda$ is a hyperparameter.
The intuition for this is somewhat involved \citep{arjovsky2019invariant}; the overarching motivation is that each environment should learn a representation such that the same predictive classifier is optimal across environments.


% \subsection{Uses Side Information More Flexibly}
% We can also explore methods that take advantage of side information beyond just data partitioning.
% One of these is auxiliary task prediction --- here we decompose our function as $f_y \circ f_r$, where $f_r$ is a learned representation and $f_y$ is a predictive classifier/regressor for $y$ on top of that learned representation.
% \RZ{Is there a reference for this method - one of the papers from Liang's group predicted the context, no?}
% We can add a function $f_c$ which aims to predict $c$ on top of $f_r$ as well, yielding the function $f = [f_y, f_c] \circ f_r$, where we concatenate the outputs of the two predictive functions both feeding from the same representation.
% Then the loss is
% \begin{equation}
%     \mathcal{L}(f) = \frac{1}{n} \sum_{i=1}^n \ell((f_y \circ f_r)(x_i), y_i) + \lambda \ell((f_c \circ f_r)(x_i), y_i) + \mathcal{R}(f)
% \end{equation}
% where we can use $\lambda \in (0, 1)$ to signal that the auxiliary task $c$ is important, influencing the representation, but less important than the main task $y$.
% Our hope is that the information in the auxiliary task can add extra information to the representation in a way that improves robustness; this may be true in particular if the auxiliary task contains some data relevant to the task.

% We can additionally consider the option of adapting our function $f$ depending on the input.
% We consider there are some parameters $\theta$ in $f$ which we will vary as a function of the input $x$, in particular, as a function of our prediction of $c$ for an input $x$.
% We use FiLM as an inspiration for this [cite], learning a single channel-wise parameter after each Resnet block.


\subsection{Adaptive Methods}

Finally, we consider a class of loss functions which, rather than using an injection of side information to specify which examples are OOC, focuses dynamically on the hardest examples at each step.
The first is conditional variance-at-risk optimization (CVaR).
This can be cast as a type of distributionally robust optimization (DRO) \citep{duchi2021statistics}, where we aim to maximize the loss over, rather than the whole training set, a worst-case distribution over training examples.
For some $p \in (0, 1)$, CVaR($p$) is defined as the average loss of the $p$-percent worst-loss examples.

We also consider focal loss \citep{lin2017focal}, which dynamically upweights high loss examples using a parameter $\gamma \geq 0$.
With binary $y$, $q(x, y) = f(x)$ if $y = 1$ and $q(x) = 1 - f(x)$ if $y = 0$, with $f(x) \in [0, 1]$ as the continuous-scored output of $f$, not the binary prediction.
Then, we have focal loss as a modification of the cross-entropy loss --- at $\gamma=0$ this reduces to cross-entropy; as $\gamma$ increases, it focuses more loss on the examples which have higher loss already:
\begin{equation}
    \mathcal{L}_{Focal}(f) = \frac{1}{n} \sum_{i=1}^n -(1 - q(x_i, y))^\gamma \log(q(x_i, y)) + \mathcal{R}(f)
\end{equation}

%\RZ{Did you get a chance to look at how worst-loss or focal examples change during training? Could put a pointer to Appendix and do this over next few days.}





% variance regularization? rex?

==> sections/methods_new.tex <==

\section{Methods} \label{sec:methods}

% In Sec. \ref{sec:experiments}, we test a number of methods on the {\rococo \ } challenge sets, and provide analysis of their performance.
% We focus on five methods:
% , which represent a range of different philosophies on OOC prediction:
% expected risk minimization (ERM), group DRO (GDRO) \citep{sagawa2019distributionally}, invariant risk minimization (IRM) \citep{arjovsky2019invariant} , conditional value at risk minimization (CVaR) \citep{rockafellar2002conditional}, and focal loss \citep{lin2017focal}.
We choose to focus on five methods which provide a useful contrast between different approaches to OOC prediction. 
Expected risk minimization (\textbf{ERM}) is the standard loss function in ML systems; as shown by \citet{gulrajani2020search}, it can be difficult to beat on domain generalization problems.
Group DRO (\textbf{GDRO}) \citep{sagawa2019distributionally} and invariant risk minimization (\textbf{IRM}) \citep{arjovsky2019invariant} are popular examples of environment-based learning methods.
In contrast to these, we also look at two \textit{adaptive} methods, which do not require auxiliary information at training time and instead attempt to adaptively determine the most difficult examples at each step.
Conditional value at risk minimization (\textbf{CVaR}) \citep{rockafellar2002conditional}, like GDRO, can be thought of as an example of distributionally robust optimization, a common approach in the robustness literature \citep{duchi2021statistics} --- however, in CVaR we minimize the loss for a worst case distribution over examples at each step, and in GDRO we minimize the worst-case loss among pre-defined groups.
\textbf{Focal} loss \citep{lin2017focal} is not necessarily commonly used in the OOC setting; however, it is a widely used reweighting technique in computer vision; a class of approaches common in OOC prediction \citep{shimodaira2000improving}.
Finally, we explore reweighting and undersampling, two common techniques for handling various forms of data imbalance.
See App. \ref{app:other-methods} for information on other methods we experimented with but did not include here, including methods that adapt parameters to context and methods which aim to predict context.
We found the methods we included here had the best results overall, on the standard and hard examples. %\RZ{Could justify the selection of these -- we found the methods here to have the best results overall, on the standard and hard examples. And what do you mean by adapt parameters to context?}


Throughout, we use the following notation.
We are given a dataset $\{x_i, y_i\}_{i=1}^n$ with inputs and target labels respectively, and possibly some side information $\{ c_i \}_{i=1}^n$ as well (e.g. environment variables).
If side information is available, we assume it is available at training time but not necessarily test time.
We are aiming to learn a function $f: \mathds{X} \longrightarrow \mathds{Y}$.
We assume $\ell$ to be the the example-wise cross-entropy loss function, and that 
% For all methods, we our function $f$ is a Resnet-50, trained with SGD (learning rate = 1e-4 and momentum = 0.9, which we found to work the best for ERM).

\subsection{Expected Risk Minimization}
Expected risk minimization (ERM) is the standard paradigm for training ML models.
In ERM, we minimize the mean loss $\ell$ on the training set, plus potentially some data-independent regularizer $\mathcal{R}$:
\begin{equation}
    \mathcal{L}_{ERM}(f) = \frac{1}{n} \sum_{i=1}^n \ell(f(x_i), y_i) + \mathcal{R}(f)
\end{equation}

% We can examine three types of ERM models: 1) trained from scratch, 2) finetuned from Imagenet pre-trained weights, and 3) logistic regression on top of pre-trained Imagenet features.
% \RZ{Small rewording}: 1) logistic regression on top of pre-trained Imagenet features; 2) logistic regression on top of pre-trained Imagenet features; 3) logistic regression on top of Imagenet features, finetuned.
% Since we found the finetuning from Imagenet pre-training worked the best across nearly all metrics, we used that initialization procedure for all other methods as well.

% \begin{itemize}
%     \item ERM, trained from scratch
%     \item ERM, image net pre-trained
%     \item ERM, logistic regression on pretrained representations
%     \item Footnote: ERM, learning rate tuning
% \end{itemize}

\subsection{Label-Based Adjustments}

Since COCO-Stuff contains significant label imbalance, we consider methods intended to correct for label imbalance.
We let $w_i = P(Y = y_i)$ in the training set.
To make a fairer comparison with the environment-based methods (below), we add a tuning parameter $\alpha$ to control the degree of adjustment.
$\alpha = 1$ represents the standard versions of these loss functions, but we frequently found other values $\alpha \in [0, 2]$ to be useful.

\paragraph{Label Reweighting.}
We reweight the loss of each training example in the ERM loss function, inversely proportional (when $\alpha = 1$) to the likelihood of observing that label:
\begin{equation}
    \mathcal{L}_{Reweight}(f) = \frac{1}{n} \sum_{i=1}^n (\frac{1}{w_i})^\alpha \ell(f(x_i), y_i) + \mathcal{R}(f)
\end{equation}

\paragraph{Label Undersampling.}
Rather than sampling training examples uniformly, we sample them with probability inversely proportional (when $\alpha = 1$) to the likelihood of observing that label.
We let $\mathcal{I}$ be a list of indices of size $n$, sampled independently from $[1 \dots n]$, such that for each $j \in \mathcal{I}$, $P(j = i)$ is proportional to $(\frac{1}{w_i})^\alpha$.
We redraw this for the training set every epoch and weight their losses equally as follows:
\begin{equation}
    \mathcal{L}_{Undersampling}(f) = \frac{1}{n} \sum_{i \in \mathcal{I}} \ell(f(x_i), y_i) + \mathcal{R}(f)
\end{equation}

\subsection{Environment-Based Methods}
One common setting is where the side information $c_i$ for each example is a one-hot variable, representing an \textit{environment}.
The notion of environments for robust learning was originally given with causal motivation \citep{peters2016causal}, where each value of $c$ represents a different intervention on the underlying causal graph.
However, this type of grouping procedure can be used completely separately from the causal context, and so we just consider it to represent some informative partition of our data, which is defined as an input at training time.
Here, $c \in \{ 1 \dots C \}$ is an integer or a one-hot encoded variable.
We will use the following shorthand to describe the average loss for a group:
\begin{equation}
    \ell_c (f) = \frac{1}{n_c} \sum_{i=1}^{n} \ell(f(x_i), y_i) \one \{ c_i = c \}
\end{equation}
% We consider two popular environment-based learning algorithms.

\paragraph{Group DRO.}
The first environment-based method we consider is Group Distributionally Robust Optimization (GDRO) \citep{sagawa2019distributionally}, which aims to minimize the loss on the worst of $C$ partitions, with partition $c$ of size $n_c$, and group adjustment hyperparameter $K$:
\begin{equation}
    \mathcal{L}_{GDRO}(f) = \underset{c \in \{ 1 \dots C \}}{\max} \Big\{  \ell_c (f) + \frac{K}{\sqrt{n_c}}  \Big\} + \mathcal{R}(f)
\end{equation}
This loss aims to ensure that no group's loss is that bad, and the group adjustment term ensures greater focus on smaller groups, which may otherwise be ignored.

\paragraph{IRM.}
The second environment-based method we consider is invariant risk minimization (IRM) \citep{arjovsky2019invariant}:
% , which uses the following loss function
\begin{equation}
    \mathcal{L}_{IRM}(f) = \sum_{c=1}^C  \ell_c (f) + \lambda \| \nabla_{w | w=1} \ell_c (w \cdot f) \| + \mathcal{R}(f)
\end{equation}
The second term here is a gradient penalty on the output of $f$, $w$ is a constant multiplier on the output of $f$, and $\lambda$ is a hyperparameter.
The intuition for this is somewhat involved \citep{arjovsky2019invariant}; the overarching motivation is that each environment should learn a representation such that the same predictive classifier is optimal across environments.

\paragraph{Environment Reweighting and Undersampling.}
These are equivalent to label reweighting/undersampling above, but with $w_i = P(c = c_i)$.

% \subsection{Uses Side Information More Flexibly}
% We can also explore methods that take advantage of side information beyond just data partitioning.
% One of these is auxiliary task prediction --- here we decompose our function as $f_y \circ f_r$, where $f_r$ is a learned representation and $f_y$ is a predictive classifier/regressor for $y$ on top of that learned representation.
% \RZ{Is there a reference for this method - one of the papers from Liang's group predicted the context, no?}
% We can add a function $f_c$ which aims to predict $c$ on top of $f_r$ as well, yielding the function $f = [f_y, f_c] \circ f_r$, where we concatenate the outputs of the two predictive functions both feeding from the same representation.
% Then the loss is
% \begin{equation}
%     \mathcal{L}(f) = \frac{1}{n} \sum_{i=1}^n \ell((f_y \circ f_r)(x_i), y_i) + \lambda \ell((f_c \circ f_r)(x_i), y_i) + \mathcal{R}(f)
% \end{equation}
% where we can use $\lambda \in (0, 1)$ to signal that the auxiliary task $c$ is important, influencing the representation, but less important than the main task $y$.
% Our hope is that the information in the auxiliary task can add extra information to the representation in a way that improves robustness; this may be true in particular if the auxiliary task contains some data relevant to the task.

% We can additionally consider the option of adapting our function $f$ depending on the input.
% We consider there are some parameters $\theta$ in $f$ which we will vary as a function of the input $x$, in particular, as a function of our prediction of $c$ for an input $x$.
% We use FiLM as an inspiration for this [cite], learning a single channel-wise parameter after each Resnet block.




\subsection{Adaptive Methods}

Finally, we consider a class of loss functions which, rather than using an injection of side information to specify which examples are OOC, focuses dynamically on the hardest examples at each step.
The first is conditional variance-at-risk optimization (CVaR).
This can be cast as a type of distributionally robust optimization (DRO) \citep{duchi2021statistics}, where we aim to maximize the loss over, rather than the whole training set, a worst-case distribution over training examples.
For some $p \in (0, 1)$, CVaR($p$) is defined as the average loss of the $p$-percent worst-loss examples.

We also consider focal loss \citep{lin2017focal}, which dynamically upweights high loss examples using a parameter $\gamma \geq 0$.
With binary $y$, $q(x, y) = f(x)$ if $y = 1$ and $q(x) = 1 - f(x)$ if $y = 0$, with $f(x) \in [0, 1]$ as the continuous-scored output of $f$, not the binary prediction.
Then, we have focal loss as a modification of the cross-entropy loss --- at $\gamma=0$ this reduces to cross-entropy; as $\gamma$ increases, it focuses more loss on the examples which have higher loss already:
\begin{equation}
    \mathcal{L}_{Focal}(f) = \frac{1}{n} \sum_{i=1}^n -(1 - q(x_i, y))^\gamma \log(q(x_i, y)) + \mathcal{R}(f)
\end{equation}

%\RZ{Did you get a chance to look at how worst-loss or focal examples change during training? Could put a pointer to Appendix and do this over next few days.}





% variance regularization? rex?

==> sections/results.tex <==



\section{Experiments} \label{sec:experiments}

% We now present experimental results.
% We use the COCO-Stuff dataset.
For all experiments we use a ResNet-50 \citep{he2016deep}, finetuned from ImageNet-pretrained features \citep{russakovsky2015imagenet}.
See App. \ref{app:data} and \ref{app:experiments} for further experimental details.
For the environment-based methods, we follow \citet{sagawa2019distributionally} and create 4 environments: 1 for each element of the cross-product of the label and its highest-$\alpha$ context class.
Many of the robust baselines from Sec. \ref{sec:methods} come with a hyperparameter which aims to trade off between average performance and OOC performance; we choose the hyperparameter which minimizes the maximum loss of hard positives and hard negatives on the validation set.

\subsection{Quantitative Analysis}

% We display results in the following formats.
In Table \ref{tab:auc-by-task}, we show AUC (area under the ROC curve) on hard examples for each of the five methods we focus on, for each of the 12 {\rococo\ } tasks individually --- AUC is a particularly informative metric since it is sensitive to label imbalance, and tasks in {\rococo \ } contain 1-10\% positive examples.
In Figures \ref{fig:results-auc-hard-easy}, \ref{fig:results-err-hard-posneg-easy}, \ref{fig:results-nll-hard-posneg-easy}, and \ref{fig:results-ece-hard-easy}, we show AUC, classification error, mean negative log-likelihood (NLL), and expected calibration error (ECE) \citep{guo2017calibration} respectively, averaged across the 12 tasks.
For AUC and ECE, we display results for hard and easy examples separately (where an ``easy'' example is defined as one which is not ``hard'', i.e. not a hard positive or hard negative).
For error and NLL, we further break out the results on hard examples into hard positives and hard negatives.
For all, we show \rococo-CE and \rococo-Gist separately.
% In the rest of this subsection, we organize our analysis by learning method.

\begin{table}
\resizebox{0.5\columnwidth}{!}{%
\centering
\input{tables/area_aucs_hard}
% \caption{Foo}
}
\hfill
\resizebox{0.5\columnwidth}{!}{%
\centering
\input{tables/caption_aucs_hard}
% \caption{Bar}
}
\caption{AUC on hard test examples for all 12 \rococo \ stress tests, after hyperparameter selection. 
Bold numbers have overlapping standard deviations.
L: \rococo-CE.
R: \rococo-Gist.
}
\label{tab:auc-by-task}
\end{table}

\paragraph{Gist Shift is Difficult.}
We note that performance on \rococo-Gist is worse than \rococo-CE.
This suggests that the more complex notion of context embodied by the gist yields a more difficult OOC task.
In some ways, would expect models to find these more holistic shifts harder, as these gist shifts go well beyond ``shortcuts'' \citep{geirhos2020shortcut}.
We also note that the gap between the environment-based methods and ERM is much smaller on \rococo-Gist, indicating that ERM is a strong baseline on this task, making gist shift a useful direction for OOC prediction research.
% This suggests that \rococo-Gist is a more difficult and potentially useful set for probing the limits of OOC performance among deep models, and that gist shift represents a useful goal for OOC prediction research.

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_area_he_auc.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_caption_he_auc.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
AUC (area under the ROC curve) achieved on hard and easy examples. Higher is better.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-auc-hard-easy}
\end{figure} 

\paragraph{Tradeoffs Exist Between Harder and Easier Examples.}
We note two tradeoffs across AUC, error, and NLL results: models that are better on hard examples tend to be worse on easy examples (and vice versa), and models that are better on hard positives tend to be worse on hard negatives.
ERM is better on easy examples and hard negatives: since the dataset is imbalanced, the hard negatives are the easier ``hard'' examples, and we expect ERM to perform better here since negatives are the majority class.
We also note that environment-based methods beat ERM on hard positives (the harder ``hard'' examples) suggesting that the extra information from environments helps.


\paragraph{Environments Matter.}
GDRO's performance falls the most between \rococo-CE and \rococo-Gist.
We interpret GDRO's performance on \rococo-CE as unusually high, as it optimizes over a set of groups similar to the ones that calculate this metric.
However, this seems to overstate its ability to handle more complex OOC problems, such as \rococo-Gist.
The choice of environment variables is crucial in general; IRM might improve with the addition of environment variables which vary more independently from the context variables of concern.
% ; this would more closely mimic the examples in \citet{arjovsky2019invariant}.
The effect of environments and how to choose or create them is an open question,
and an active area of research.
%\cite{}}


\paragraph{ERM Makes Confident OOC Errors.}
We find that the AUC and NLL/Error plots tell different stories.
When looking at AUC, we see that the environment-based methods perform the best on \rococo-CE, and things are more even on \rococo-Gist, with GDRO falling off quite a bit and IRM recording the worst AUC on hard examples.
However, when looking at NLL (or error), we see that on both challenge sets, GDRO and IRM have much lower NLL than ERM on hard positives (and higher on hard negatives/easy examples).
This suggests that while the relative ordering of predictions on hard examples from ERM models may be fairly good (as suggested by the AUC), when it is wrong, it is sometimes extremely wrong, incurring high NLL on its worst mistakes.


\paragraph{Adaptive Methods Find Different Tradeoffs.}
We find that CVaR and focal loss find interesting tradeoffs between ERM and environment-based methods.
CVaR performs slightly worse than ERM on both hard and easy examples by AUC and error measures; and by ECE it is by far the worst of any method.
However, CVaR's NLL on hard positives is between ERM and the environment-based methods.
Focal loss, on the other hand, performs similarly to ERM by AUC on both hard and easy examples, but it performs similarly to the environment-based methods on hard positives and negatives by error and NLL, providing a strong tradeoff between overall and OOC performance.
% See App. \ref{app:experiments} for more observations about adaptive methods results.

\paragraph{Two Surprising Calibration Results.}
% We note two surprising calibration results.
First, we found that there was \textit{not} the same tradeoff with calibration as there was with the other metrics.
In particular, ERM had the best calibration on both hard and easy examples, suggesting there may be a path forward to avoid some of the tradeoffs between OOC and average performance by thinking more about calibration.
Second, we found that focal loss had much better calibration on easy examples than any other method (except ERM).
The well-calibrated nature of focal loss is known \citep{mukhoti2020calibrating}; interestingly, it was the only method with low NLL/Error on hard positives \textit{and} good calibration on easy examples.






% \paragraph{ERM.}
% We find that ERM achieves lower AUC, error and NLL on hard examples than environment-based methods do, with the opposite result among easy examples.
% However, ERM performs better on hard negatives 
% % than the environment-based methods
% : we note that since the dataset is imbalanced (1-10\% positive), the hard negatives are in some sense the easier ``hard'' examples, and we might expect ERM to perform well here since negatives are the majority class.
% % This presents an open question going forward: how do we best evaluate performance on hard negative examples in the presence of label imbalance?
% % Note that this is not an issue for a metric like AUC, which is robust to label imbalance.
% % We further note that compared to the environment-based methods, ERM's improvement on hard negatives is much smaller than its decrease in performance on hard positives. 
% Finally, we find that ERM is the best-calibrated model on both hard and easy examples.
% This is somewhat surprising, and it suggests that there may not be a tradeoff between OOC performance and overall performance when it comes to calibration.
% % way we usually think about tradeoffs in OOC settings do not necessarily apply to calibration.



\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_area_hphne_err.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_caption_hphne_err.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Classification error achieved on hard positive, hard negative, and easy examples.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-err-hard-posneg-easy}
\end{figure}


% \paragraph{GDRO and IRM.}
% We find that the two environment-based methods perform similarly across the board.
% % , with some interesting contrasts.
% On both challenge set groups, these methods achieve the good NLL on the hard positives, indicating that the extra environment information is helfpul.
% We note that this NLL is still not particularly low (0.4-0.5) indicating there is room for improvement on both challenge sets.
% % GDRO clearly performs the best on hard AUC, and IRM has nearly as good NLL on hard examples.
% These two methods also have the best hard AUC on most \rococo-CE tasks, but are much more similar to the other methods on \rococo-Gist, with IRM performing somewhat poorly.
% In particular, we note that GDRO's performance falls off the most drastically between \rococo-CE and \rococo-Gist.
% % They clearly perform the best on hard examples, with the best hard AUC on 11 of the 12 tasks on \rococo-CE, and on 9 of the 12 on \rococo-Gist, showing that the auxiliary information provided by environments is helpful for OOC performance.
% % However, we note that like all the other methods, the performance is worse on \rococo-Gist, indicating that perhaps the information contained in the chosen environment variables does not adequately capture the type of context present in the gist. 
% % which the caption shift changes.
% % This seems especially true of GDRO, which has a higher hard AUC than IRM on 11 of 12 tasks on \rococo-CE, but only 6 of 12 on \rococo-Gist.
% Our interpretation of this result is that GDRO's performance on the co-occurrence sets is unusually high --- it performs minimax optimization over a very similar set of groups that go into calculating this metric, its loss function seems like nearly a perfect match for solving \rococo-CE.
% However, this performance seems to overstate its ability to handle more complex OOC problems, such as those presented in the caption-based setting.
% In general, the choice of environment variables is paramount for both approaches --- in particular, IRM might improve with the addition of some environment variables which vary more independently from the context variables of concern.
% % ; this would more closely mimic the examples in \citet{arjovsky2019invariant}.
% The effect of environments, how to choose environments from auxiliary data, and the viability of self-determined environments are all open questions.



\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_area_hphne_nll.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_caption_hphne_nll.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Negative log-likelihood (NLL) achieved on hard positive, hard negative, and easy examples.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-nll-hard-posneg-easy}
\end{figure}


% \paragraph{CVaR.}
% By both AUC and error measures, CVaR performs slightly worse than ERM on both hard and easy examples; and by ECE it performs by far the worst of any method.
% However, when evaluating by NLL, CVaR profiles as a tradeoff between ERM and the environment-based methods.
% This is intuitive, since it is doing something similar to GDRO, but it is finding the highest-loss examples in each minibatch rather than the environment with the highest loss examples.
% % We find in Table \ref{tab:calib-failure} that CVaR tends to be mostly \textit{underconfident}.
% Digging deeper, we find that CVaR tends to be mostly \textit{underconfident}.
% This may explain why its NLL on hard positives may be better than its error rate; where ERM is confidently wrong OOC, CVaR outputs a less-wrong probability (although potentially still making the wrong prediction).


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_area_he_ece.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars_old/algo_comp_barplot_caption_he_ece.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Expected Calibration Error (ECE) achieved on hard and easy examples. Lower is better.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-ece-hard-easy}
\end{figure}

% \paragraph{Focal Loss.}
% We find that focal loss combines some features from both ERM and environment-based methods: it performs similarly to ERM by AUC on both hard and easy examples, but it performs similarly to the environment-based methods on hard positives and negatives by error and NLL.
% Additionally, its calibration is very strong, particularly on easy examples.
% % it is the second-best performing method (after ERM) by calibration, performing very well on easy examples and moderately well on hard examples.
% The well-calibrated nature of focal loss has been noted previously \citep{mukhoti2020calibrating}, but its performance on OOC prediction is a new observation.
% While focal loss does not perform quite as well OOC as the environment-based methods, it provides a strong tradeoff between overall and OOC performance.
\begin{wrapfigure}{L}{0.5\linewidth} % "[t!]" placement specifier just for this example
% \hspace*{-0.5cm}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Hard_Positive.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Hard_Negative.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Easy_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
\caption{Test set examples where GDRO most improves over ERM (L) hard positives and (R) hard negatives
from the \rococo-CE \texttt{car} category.
Titles show NLL for each method on that image.
% From L to R: .
} \label{fig:results-qual-examples-car}
\end{wrapfigure}





\subsection{Qualitative Analysis}



% We now examine some images from the test set to understand better the differences in performance between the various methods.
% In this section, we focus on the \texttt{car} class, and 
\paragraph{Where Environment-based Learning Improves Over ERM.}
In Fig. \ref{fig:results-qual-examples-car}, we show the images with the largest gaps in NLL on the \texttt{car} task among two groups: hard positives and hard negatives (in \rococo-CE).
% These examples give us some insight into the strengths and weaknesses of the GDRO method.
The hard positive and hard negative where GDRO most overperformed (top row) are both images we might expect, where the object label and context do not match: a living room with a tiny toy car on the shelf, and a normal street scene that happens to not have any cars.
See App. \ref{app:qual} for analysis on where GDRO underperforms ERM.



\paragraph{Contrasting \rococo-CE and \rococo-Gist.}
In Fig. \ref{fig:results-qual-examples-critdiff}, we use examples of hard positives from the \texttt{cow} task to contrast the CE and gist criteria.
On the left, we show a hard positive from \rococo-CE, with cows standing on pavement: this is a hard positive in \rococo-CE since there is no grass; GDRO and IRM outperform ERM on this image.
However, it is \textit{not} a hard positive in \rococo-Gist, since cows are the central focus of the image.
On the right, we show a hard positive from \rococo-Gist, where the image focuses on a giraffe, but there are several white cows in the background standing on a grassy field.
This is \textit{not} a hard positive in \rococo-CE, due to the large field, but it \textit{is} a hard positive in \rococo-Gist, since the giraffe is the focus of the image.
ERM outperforms GDRO and IRM on this image --- the environment-based objectives do not encourage as strong performance where the context (grass) and object (cow) align.




\begin{wrapfigure}{L}{0.6\linewidth} % "[t!]" placement specifier just for this example
% \hspace*{-0.5cm}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_critdiff/example_critdiff_CE_criterion_cow.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
\begin{subfigure}{0.35\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_critdiff/example_critdiff_Gist_criterion_cow.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Easy_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
\caption{Examples of hard positives from \rococo-CE (L) and \rococo-Gist (R) for the \texttt{cow} task.
% est set examples where GDRO most improves over ERM (L) hard positives and (R) hard negatives
% from the \rococo-CE \texttt{car} category.
Titles show NLL for several methods on that image.
% From L to R: .
} \label{fig:results-qual-examples-critdiff}
\end{wrapfigure}



% the sky is visible but the overall scene is unusual; this is selected as a hard positive by the Gist criteria.









% In Table \ref{tab:auc-by-task}, we show the AUC on hard examples for each method across each of the 12 {\rococo \ } tasks.
% We use AUC as our metric of choice since each class is imbalanced (mostly ~2-3\% positive labels), and this imbalance can vary between classes when we restrict only to hard examples.
% We first note that the two methods that use auxiliary information (GDRO and IRM), outperform the others on nearly every task.
% We also note that each method performs worse on the hard examples selected by captions than by area.
% This suggests that the more holistic notion of context captured by the caption method is more relevant to natural prediction problems than the area-based notion.
% We further note that the environment-based methods are less dominant on the caption-based tests, achieving the high AUC on only 9 of the 12 tasks instead of 11.
% This suggests that the auxiliary input provided to these methods is less sufficient for learning invariances that generalize to caption-OOC prediction than for area-OOC prediction; an intuitive result, since the environment labels explicitly contain information about the most important context variables.




% % In Fig \ref{fig:results-auc-hard-easy}, we show the data from Table \ref{tab:auc-by-task} averaged across tasks, alongside the AUCs for easy examples.
% % We see that on both groups of stress tests, there is a tradeoff between performance on hard and easy examples -- the environment-based methods perform better on the hard examples and worse on the easy examples.

% % We next dive deeper into these numbers by splitting out the hard examples into hard positives and hard negatives.
% % In Fig. \ref{fig:results-err-hard-posneg-easy}, we show the error rate on hard positives, hard negatives, and easy examples.
% % We see again there is a tradeoff here --- this time, between hard positives and hard negatives.
% % Note that in general, error will be higher on positive examples due to label imbalance.
% % The methods that tend to be worse on hard positives (the hardest of the ``hard'' examples) tend to be better on the ``easy'' examples, and the hard negatives (the easier ``hard'' examples).
% % The exception to this is focal loss, which is able to achieve relatively low error on both easy examples and hard positives.
% % This suggests that the more adaptive approach may be better able to negotiate the tradeoffs between OOC prediction and average performance than an environment-based approach.


% In Fig \ref{fig:results-ece-hard-easy} we explore another angle, the calibration of these methods, by looking at the expected calibration error (ECE) averaged across the 12 tasks.
% Interestingly, we find a totally different story here.
% Firstly, the calibration on hard examples seems to be \textit{better} than the calibration on easy examples.
% Secondly, the methods that have better calibration on hard examples are also the ones that have better calibration on easy examples: there does not seem to be a tradeoff.
% Again focal loss stands out as a method, as the only one with low error on hard positives and also low ECE on easy examples.


% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/results/calib_failure/calib_failure_boat.pdf}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/results/calib_failure/calib_failure_car.pdf}
% \end{subfigure}
% \caption{
% Calibration plots showing two failure modes of GDRO on easy example calibration: L: class \texttt{boat}, slightly underconfident, and R: class \texttt{car}, very overconfident.
% } \label{fig:results-gdro-calibration-failure-modes}
% \end{figure}

% We dig further, and observe two failure modes, shown in Fig. \ref{fig:results-gdro-calibration-failure-modes}.
% Firstly, a model may be somewhat underconfident, returning slightly higher accuracy scores than expected across each calibration bin.
% Secondly, a model may be extremely overconfident: returning very low accuracy scores across each calibration bin (particularly the high confidence ones).
% We can define these using the signed error (accuracy - confidence), averaged across 5 bins.
% If this is very negative (positive), the model if very over(under)confident; if it is slightly negative (positive) the model is slightly over(under)confident.

% \begin{table}[]
%     \centering
%     \input{tables/calib_failure_modes}
%     \caption{Number of tasks (summing to at most 12) for which each method is over/under-confident.
%     Calculated as $\epsilon =$ average(acc(bin) - conf(bin));
%     if $\epsilon < -0.2$: very overconfident;
%     if $-0.1 > \epsilon >= -0.2$: slightly overconfident;
%     if $\epsilon > 0.2$: very underconfident;
%     if $0.1 < \epsilon <= 0.2$: slightly underconfident.
%     }
%     \label{tab:calib-failure}
% \end{table}


% In Table \ref{tab:calib-failure}, we show that these are the two most common failure modes, explaining the mis-calibration of some methods on easy examples.
% In fact, GDRO is the only method to be very overconfident, which it is on 4 tasks (one third of 12!), meaning that catastrophic failure on easy examples is a potential tradeoff of this method.
% Also, these results suggest that methods intended to improve OOC prediction may become slightly underconfident on easy examples as a side effect.

% % We find that on easy examples, the two environment-based methods exhibit these failure modes, GDRO is somewhat underconfident on 3 out of 12 tasks, and extremely overconfident on 4 tasks; IRM is somewhat underconfident on 4 tasks.
% % Neither is ever extremely underconfident or somewhat overconfident.
% % Neither of the well-calibrated models (ERM/Focal loss), which do not use auxiliary information, exhibit these failure modes on any task.
% % This suggests a way of thinking about the weaknesses of environment-based methods: in order to improve on hard OOC examples, they may compensate by failing catastrophically on \textit{easy} examples; or by outputting lower confidence on these examples.
% % (excessive invariance angle??)



% % \begin{figure}[t!] % "[t!]" placement specifier just for this example
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_car_Y1.pdf}
% % % \caption{First subfigure} \label{fig:a}
% % \end{subfigure}\hspace*{\fill}
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_car_Y0.pdf}
% % % \caption{Second subfigure} \label{fig:b}
% % \end{subfigure}
% % \caption{
% % Car loss difference ERM - GDRO by object cooccurrence frequency.
% % } \label{fig:results-coocc-car}
% % \end{figure}

% % \begin{figure}[t!] % "[t!]" placement specifier just for this example
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_backpack_Y1.pdf}
% % % \caption{First subfigure} \label{fig:a}
% % \end{subfigure}\hspace*{\fill}
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_backpack_Y0.pdf}
% % % \caption{Second subfigure} \label{fig:b}
% % \end{subfigure}
% % \caption{
% % Backpack loss difference ERM - GDRO by object cooccurrence frequency.
% % } \label{fig:results-coocc-car}
% % \end{figure}




% % \begin{itemize}
% %     \item Overall results: Error/NLL
% %     \begin{itemize}
% %         \item split into pos/neg
% %         \item hard/easy
% %         \item hard pos/hard neg
% %     \end{itemize}
% %     \item Results: calibration
% %     \begin{itemize}
% %         \item Split into hard/easy
% %     \end{itemize}
% %     \item Results: comparison of worst images in each condition
% %     \begin{itemize}
% %         \item Qualitative analysis - show samples
% %         \item discuss excessive invariance
% %         \item talk about which images co-occur most frequently with over/under-performance
% %     \end{itemize}
% % \end{itemize}

% % \begin{figure}
% %     \centering
% %     \includegraphics[scale=0.6]{figs/calib_new.png}
% %     \caption{Caption}
% %     \label{fig:my_label}
% % \end{figure}

==> sections/results_new.tex <==



\section{Experiments} \label{sec:experiments}

% We now present experimental results.
% We use the COCO-Stuff dataset.
For all experiments we use a ResNet-50 \citep{he2016deep}, finetuned from ImageNet-pretrained features \citep{russakovsky2015imagenet}.
See App. \ref{app:data} and \ref{app:experiments} for further experimental details.
For the environment-based methods, we follow \citet{sagawa2019distributionally} and create 4 environments: 1 for each element of the cross-product of the label and its highest-$\alpha$ context class.
Many of the robust baselines from Sec. \ref{sec:methods} come with a hyperparameter which aims to trade off between average performance and OOC performance; we choose the hyperparameter which minimizes the maximum loss of hard positives and hard negatives on the validation set.



% TODO change tables
\begin{table}
\resizebox{\columnwidth}{!}{%
\centering
\input{tables/area_aucs_hard}
% \caption{Foo}
}
\caption{AUC on hard test examples for all 12 \rococo-CE \ stress tests, after hyperparameter selection. 
Bold numbers have overlapping standard deviations with the highest observed mean's.
}
\label{tab:auc-by-task-ce}
\end{table}
\begin{table}
\resizebox{\columnwidth}{!}{%
\centering
\input{tables/caption_aucs_hard}
% \caption{Bar}
}
\caption{AUC on hard test examples for all 12 \rococo-Gist \ stress tests, after hyperparameter selection. 
Bold numbers have overlapping standard deviations with the highest observed mean's.
}
\label{tab:auc-by-task-gist}
\end{table}



\subsection{Quantitative Analysis}





% We display results in the following formats.
In Tables \ref{tab:auc-by-task-ce} and \ref{tab:auc-by-task-gist}, we show AUC (area under the ROC curve) on hard examples for each of the five methods we focus on, for each of the 12 {\rococo\ } tasks individually --- AUC is a particularly informative metric since it is sensitive to label imbalance, and tasks in {\rococo \ } contain 1-10\% positive examples.
In Figures \ref{fig:results-auc-hard-easy}, \ref{fig:results-err-hard-posneg-easy}, \ref{fig:results-nll-hard-posneg-easy}, and \ref{fig:results-ece-hard-easy}, we show AUC, classification error, mean negative log-likelihood (NLL), and expected calibration error (ECE) \citep{guo2017calibration} respectively, averaged across the 12 tasks.
For AUC and ECE, we display results for hard and easy examples separately (where an ``easy'' example is defined as one which is not ``hard'', i.e. not a hard positive or hard negative).
For error and NLL, we further break out the results on hard examples into hard positives and hard negatives.
For all, we show \rococo-CE and \rococo-Gist separately.
% In the rest of this subsection, we organize our analysis by learning method.


% TODO this probably won't change much
\paragraph{Gist Shift is Difficult.}
We note that performance on \rococo-Gist is worse than \rococo-CE.
This suggests that the more complex notion of context embodied by the gist yields a more difficult OOC task.
In some ways, would expect models to find these more holistic shifts harder, as these gist shifts go well beyond ``shortcuts'' \citep{geirhos2020shortcut}.
We also note that the gap between the environment-based methods and ERM is much smaller on \rococo-Gist, indicating that ERM is a strong baseline on this task, making gist shift a useful direction for OOC prediction research.
% This suggests that \rococo-Gist is a more difficult and potentially useful set for probing the limits of OOC performance among deep models, and that gist shift represents a useful goal for OOC prediction research.



% TODO this probably won't change much
\paragraph{Tradeoffs Exist Between Harder and Easier Examples.}
We note two tradeoffs across AUC, error, and NLL results: models that are better on hard examples tend to be worse on easy examples (and vice versa), and models that are better on hard positives tend to be worse on hard negatives.
ERM is better on easy examples and hard negatives: since the dataset is imbalanced, the hard negatives are the easier ``hard'' examples, and we expect ERM to perform better here since negatives are the majority class.
% We also note that environment-based methods beat ERM on hard positives (the harder ``hard'' examples) suggesting that the extra information from environments helps.


% TODO this probably won't change much
\paragraph{Environments Matter.}
Overall, environment-based methods perform the best.
This is mostly clearly indicated in the improvement between reweighting/undersampling methods when using environments rather than labels.
However, the environment-based methods are also the ones whose performance falls off the most between \rococo-CE and \rococo-Gist.
% In particular, we interpret GDRO's performance on \rococo-CE as unusually high, as it optimizes over a set of groups similar to the ones that calculate this metric.
This could be because \rococo-CE is a simpler benchmark, more well specified by the given environments
--- we give more evidence towards this intution in Table \ref{tab:waterbirds}.
% The choice of environment variables is crucial in general; IRM might improve with the addition of environment variables which vary more independently from the context variables of concern; more closely mimicking the examples in \citet{arjovsky2019invariant}.
The effect of environments and how to choose or create them is an open question,
and an active area of research.
%\cite{}}

% TODO add section about reweighting/undersampling
\paragraph{Reweighting Is a Strong Baseline.}
We find that reweighting examples, given an equivalent amount of hyperparameter tuning to GDRO/IRM, performs similarly on this type of task.
In Table \ref{tab:waterbirds}, we replicate this result on the Waterbirds dataset.

% % TODO this probably won't change much
% \paragraph{ERM Makes Confident OOC Errors.}
% We find that the AUC and NLL/Error plots tell different stories.
% When looking at AUC, we see that the environment-based methods perform the best on \rococo-CE, and things are more even on \rococo-Gist, with GDRO falling off quite a bit and IRM recording the worst AUC on hard examples.
% However, when looking at NLL (or error), we see that on both challenge sets, GDRO and IRM have much lower NLL than ERM on hard positives (and higher on hard negatives/easy examples).
% This suggests that while the relative ordering of predictions on hard examples from ERM models may be fairly good (as suggested by the AUC), when it is wrong, it is sometimes extremely wrong, incurring high NLL on its worst mistakes.


% TODO check this

\paragraph{Adaptive Methods Find Different Tradeoffs.}
We find that CVaR and focal loss find interesting tradeoffs between ERM and environment-based methods.
CVaR performs comparable ERM on both hard and easy examples by AUC and error measures; and by ECE it is by far the worst of any method.
However, CVaR's NLL on hard positives is between ERM and the environment-based methods'.
Focal loss, on the other hand, performs similarly to ERM by AUC on both hard and easy examples, but it performs similarly to the environment-based methods on hard positives and negatives by error and NLL, providing a strong tradeoff between overall and OOC performance.
% See App. \ref{app:experiments} for more observations about adaptive methods results.


% TODO check this
\paragraph{Two Surprising Calibration Results.}
% We note two surprising calibration results.
We found that there was \textit{not} the same tradeoff with calibration as there was with the other metrics.
In particular, ERM and undersampling had the best calibration on \textit{both} hard and easy examples, suggesting there may be a path forward to avoid some of the tradeoffs between OOC and average performance by thinking more about calibration.
Secondly, we found the environment-based methods were not better calibrated, even on hard examples.
% Second, we found that undersampling had much better calibration on easy examples than any other method (comparable to ERM).
% The well-calibrated nature of focal loss is known \citep{mukhoti2020calibrating}; interestingly, it was the only method with low NLL/Error on hard positives \textit{and} good calibration on easy examples.




% TODO write this
\input{sections/results_waterbirds}



% \paragraph{ERM.}
% We find that ERM achieves lower AUC, error and NLL on hard examples than environment-based methods do, with the opposite result among easy examples.
% However, ERM performs better on hard negatives 
% % than the environment-based methods
% : we note that since the dataset is imbalanced (1-10\% positive), the hard negatives are in some sense the easier ``hard'' examples, and we might expect ERM to perform well here since negatives are the majority class.
% % This presents an open question going forward: how do we best evaluate performance on hard negative examples in the presence of label imbalance?
% % Note that this is not an issue for a metric like AUC, which is robust to label imbalance.
% % We further note that compared to the environment-based methods, ERM's improvement on hard negatives is much smaller than its decrease in performance on hard positives. 
% Finally, we find that ERM is the best-calibrated model on both hard and easy examples.
% This is somewhat surprising, and it suggests that there may not be a tradeoff between OOC performance and overall performance when it comes to calibration.
% % way we usually think about tradeoffs in OOC settings do not necessarily apply to calibration.




\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_area_he_auc.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_caption_he_auc.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
AUC (area under the ROC curve) achieved on hard and easy examples. Higher is better.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-auc-hard-easy}
\end{figure}



\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_area_hphne_err.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_caption_hphne_err.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Classification error achieved on hard positive, hard negative, and easy examples.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-err-hard-posneg-easy}
\end{figure}


% \paragraph{GDRO and IRM.}
% We find that the two environment-based methods perform similarly across the board.
% % , with some interesting contrasts.
% On both challenge set groups, these methods achieve the good NLL on the hard positives, indicating that the extra environment information is helfpul.
% We note that this NLL is still not particularly low (0.4-0.5) indicating there is room for improvement on both challenge sets.
% % GDRO clearly performs the best on hard AUC, and IRM has nearly as good NLL on hard examples.
% These two methods also have the best hard AUC on most \rococo-CE tasks, but are much more similar to the other methods on \rococo-Gist, with IRM performing somewhat poorly.
% In particular, we note that GDRO's performance falls off the most drastically between \rococo-CE and \rococo-Gist.
% % They clearly perform the best on hard examples, with the best hard AUC on 11 of the 12 tasks on \rococo-CE, and on 9 of the 12 on \rococo-Gist, showing that the auxiliary information provided by environments is helpful for OOC performance.
% % However, we note that like all the other methods, the performance is worse on \rococo-Gist, indicating that perhaps the information contained in the chosen environment variables does not adequately capture the type of context present in the gist. 
% % which the caption shift changes.
% % This seems especially true of GDRO, which has a higher hard AUC than IRM on 11 of 12 tasks on \rococo-CE, but only 6 of 12 on \rococo-Gist.
% Our interpretation of this result is that GDRO's performance on the co-occurrence sets is unusually high --- it performs minimax optimization over a very similar set of groups that go into calculating this metric, its loss function seems like nearly a perfect match for solving \rococo-CE.
% However, this performance seems to overstate its ability to handle more complex OOC problems, such as those presented in the caption-based setting.
% In general, the choice of environment variables is paramount for both approaches --- in particular, IRM might improve with the addition of some environment variables which vary more independently from the context variables of concern.
% % ; this would more closely mimic the examples in \citet{arjovsky2019invariant}.
% The effect of environments, how to choose environments from auxiliary data, and the viability of self-determined environments are all open questions.



\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_area_hphne_nll.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_caption_hphne_nll.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Negative log-likelihood (NLL) achieved on hard positive, hard negative, and easy examples.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-nll-hard-posneg-easy}
\end{figure}


% \paragraph{CVaR.}
% By both AUC and error measures, CVaR performs slightly worse than ERM on both hard and easy examples; and by ECE it performs by far the worst of any method.
% However, when evaluating by NLL, CVaR profiles as a tradeoff between ERM and the environment-based methods.
% This is intuitive, since it is doing something similar to GDRO, but it is finding the highest-loss examples in each minibatch rather than the environment with the highest loss examples.
% % We find in Table \ref{tab:calib-failure} that CVaR tends to be mostly \textit{underconfident}.
% Digging deeper, we find that CVaR tends to be mostly \textit{underconfident}.
% This may explain why its NLL on hard positives may be better than its error rate; where ERM is confidently wrong OOC, CVaR outputs a less-wrong probability (although potentially still making the wrong prediction).


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_area_he_ece.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\centering
\includegraphics[width=0.9\linewidth]{figs/results/algo_comp_bars/algo_comp_barplot_caption_he_ece.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
Expected Calibration Error (ECE) achieved on hard and easy examples. Lower is better.
% L: \rococo-CE.
% R: \rococo-Gist.
} \label{fig:results-ece-hard-easy}
\end{figure}

% \paragraph{Focal Loss.}
% We find that focal loss combines some features from both ERM and environment-based methods: it performs similarly to ERM by AUC on both hard and easy examples, but it performs similarly to the environment-based methods on hard positives and negatives by error and NLL.
% Additionally, its calibration is very strong, particularly on easy examples.
% % it is the second-best performing method (after ERM) by calibration, performing very well on easy examples and moderately well on hard examples.
% The well-calibrated nature of focal loss has been noted previously \citep{mukhoti2020calibrating}, but its performance on OOC prediction is a new observation.
% While focal loss does not perform quite as well OOC as the environment-based methods, it provides a strong tradeoff between overall and OOC performance.
\begin{wrapfigure}{L}{0.5\linewidth} % "[t!]" placement specifier just for this example
% \hspace*{-0.5cm}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Hard_Positive.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
\begin{subfigure}{0.25\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Hard_Negative.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Easy_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
\caption{Test set examples where GDRO most improves over ERM (L) hard positives and (R) hard negatives
from the \rococo-CE \texttt{car} category.
Titles show NLL for each method on that image.
% From L to R: .
} \label{fig:results-qual-examples-car}
\end{wrapfigure}





\subsection{Qualitative Analysis}



% We now examine some images from the test set to understand better the differences in performance between the various methods.
% In this section, we focus on the \texttt{car} class, and 
\paragraph{Where Environment-based Learning Improves Over ERM.}
In Fig. \ref{fig:results-qual-examples-car}, we show the images with the largest gaps in NLL on the \texttt{car} task among two groups: hard positives and hard negatives (in \rococo-CE).
% These examples give us some insight into the strengths and weaknesses of the GDRO method.
The hard positive and hard negative where GDRO most overperformed (top row) are both images we might expect, where the object label and context do not match: a living room with a tiny toy car on the shelf, and a normal street scene that happens to not have any cars.
See App. \ref{app:qual} for analysis on where GDRO underperforms ERM.



\paragraph{Contrasting \rococo-CE and \rococo-Gist.}
In Fig. \ref{fig:results-qual-examples-critdiff}, we use examples of hard positives from the \texttt{cow} task to contrast the CE and gist criteria.
On the left, we show a hard positive from \rococo-CE, with cows standing on pavement: this is a hard positive in \rococo-CE since there is no grass; GDRO and IRM outperform ERM on this image.
However, it is \textit{not} a hard positive in \rococo-Gist, since cows are the central focus of the image.
On the right, we show a hard positive from \rococo-Gist, where the image focuses on a giraffe, but there are several white cows in the background standing on a grassy field.
This is \textit{not} a hard positive in \rococo-CE, due to the large field, but it \textit{is} a hard positive in \rococo-Gist, since the giraffe is the focus of the image.
ERM outperforms GDRO and IRM on this image --- the environment-based objectives do not encourage as strong performance where the context (grass) and object (cow) align.




\begin{wrapfigure}{L}{0.6\linewidth} % "[t!]" placement specifier just for this example
% \hspace*{-0.5cm}
\begin{subfigure}{0.32\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_critdiff/example_critdiff_CE_criterion_cow.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
\begin{subfigure}{0.35\textwidth}
\includegraphics[width=\linewidth]{figs/results/qual_critdiff/example_critdiff_Gist_criterion_cow.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}%\hspace*{\fill}
% \hspace*{-2cm}
% \begin{subfigure}{0.33\textwidth}
% \includegraphics[width=\linewidth]{figs/results/qual_examples/example_loss_diff_GDRO_over_ERM_car_Easy_Positive.pdf}
% % \caption{Second subfigure} \label{fig:b}
% \end{subfigure}
\caption{Examples of hard positives from \rococo-CE (L) and \rococo-Gist (R) for the \texttt{cow} task.
% est set examples where GDRO most improves over ERM (L) hard positives and (R) hard negatives
% from the \rococo-CE \texttt{car} category.
Titles show NLL for several methods on that image.
% From L to R: .
} \label{fig:results-qual-examples-critdiff}
\end{wrapfigure}



% the sky is visible but the overall scene is unusual; this is selected as a hard positive by the Gist criteria.









% In Table \ref{tab:auc-by-task}, we show the AUC on hard examples for each method across each of the 12 {\rococo \ } tasks.
% We use AUC as our metric of choice since each class is imbalanced (mostly ~2-3\% positive labels), and this imbalance can vary between classes when we restrict only to hard examples.
% We first note that the two methods that use auxiliary information (GDRO and IRM), outperform the others on nearly every task.
% We also note that each method performs worse on the hard examples selected by captions than by area.
% This suggests that the more holistic notion of context captured by the caption method is more relevant to natural prediction problems than the area-based notion.
% We further note that the environment-based methods are less dominant on the caption-based tests, achieving the high AUC on only 9 of the 12 tasks instead of 11.
% This suggests that the auxiliary input provided to these methods is less sufficient for learning invariances that generalize to caption-OOC prediction than for area-OOC prediction; an intuitive result, since the environment labels explicitly contain information about the most important context variables.




% % In Fig \ref{fig:results-auc-hard-easy}, we show the data from Table \ref{tab:auc-by-task} averaged across tasks, alongside the AUCs for easy examples.
% % We see that on both groups of stress tests, there is a tradeoff between performance on hard and easy examples -- the environment-based methods perform better on the hard examples and worse on the easy examples.

% % We next dive deeper into these numbers by splitting out the hard examples into hard positives and hard negatives.
% % In Fig. \ref{fig:results-err-hard-posneg-easy}, we show the error rate on hard positives, hard negatives, and easy examples.
% % We see again there is a tradeoff here --- this time, between hard positives and hard negatives.
% % Note that in general, error will be higher on positive examples due to label imbalance.
% % The methods that tend to be worse on hard positives (the hardest of the ``hard'' examples) tend to be better on the ``easy'' examples, and the hard negatives (the easier ``hard'' examples).
% % The exception to this is focal loss, which is able to achieve relatively low error on both easy examples and hard positives.
% % This suggests that the more adaptive approach may be better able to negotiate the tradeoffs between OOC prediction and average performance than an environment-based approach.


% In Fig \ref{fig:results-ece-hard-easy} we explore another angle, the calibration of these methods, by looking at the expected calibration error (ECE) averaged across the 12 tasks.
% Interestingly, we find a totally different story here.
% Firstly, the calibration on hard examples seems to be \textit{better} than the calibration on easy examples.
% Secondly, the methods that have better calibration on hard examples are also the ones that have better calibration on easy examples: there does not seem to be a tradeoff.
% Again focal loss stands out as a method, as the only one with low error on hard positives and also low ECE on easy examples.


% \begin{figure}[t!] % "[t!]" placement specifier just for this example
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/results/calib_failure/calib_failure_boat.pdf}
% \end{subfigure}\hspace*{\fill}
% \begin{subfigure}{0.48\textwidth}
% \includegraphics[width=\linewidth]{figs/results/calib_failure/calib_failure_car.pdf}
% \end{subfigure}
% \caption{
% Calibration plots showing two failure modes of GDRO on easy example calibration: L: class \texttt{boat}, slightly underconfident, and R: class \texttt{car}, very overconfident.
% } \label{fig:results-gdro-calibration-failure-modes}
% \end{figure}

% We dig further, and observe two failure modes, shown in Fig. \ref{fig:results-gdro-calibration-failure-modes}.
% Firstly, a model may be somewhat underconfident, returning slightly higher accuracy scores than expected across each calibration bin.
% Secondly, a model may be extremely overconfident: returning very low accuracy scores across each calibration bin (particularly the high confidence ones).
% We can define these using the signed error (accuracy - confidence), averaged across 5 bins.
% If this is very negative (positive), the model if very over(under)confident; if it is slightly negative (positive) the model is slightly over(under)confident.

% \begin{table}[]
%     \centering
%     \input{tables/calib_failure_modes}
%     \caption{Number of tasks (summing to at most 12) for which each method is over/under-confident.
%     Calculated as $\epsilon =$ average(acc(bin) - conf(bin));
%     if $\epsilon < -0.2$: very overconfident;
%     if $-0.1 > \epsilon >= -0.2$: slightly overconfident;
%     if $\epsilon > 0.2$: very underconfident;
%     if $0.1 < \epsilon <= 0.2$: slightly underconfident.
%     }
%     \label{tab:calib-failure}
% \end{table}


% In Table \ref{tab:calib-failure}, we show that these are the two most common failure modes, explaining the mis-calibration of some methods on easy examples.
% In fact, GDRO is the only method to be very overconfident, which it is on 4 tasks (one third of 12!), meaning that catastrophic failure on easy examples is a potential tradeoff of this method.
% Also, these results suggest that methods intended to improve OOC prediction may become slightly underconfident on easy examples as a side effect.

% % We find that on easy examples, the two environment-based methods exhibit these failure modes, GDRO is somewhat underconfident on 3 out of 12 tasks, and extremely overconfident on 4 tasks; IRM is somewhat underconfident on 4 tasks.
% % Neither is ever extremely underconfident or somewhat overconfident.
% % Neither of the well-calibrated models (ERM/Focal loss), which do not use auxiliary information, exhibit these failure modes on any task.
% % This suggests a way of thinking about the weaknesses of environment-based methods: in order to improve on hard OOC examples, they may compensate by failing catastrophically on \textit{easy} examples; or by outputting lower confidence on these examples.
% % (excessive invariance angle??)



% % \begin{figure}[t!] % "[t!]" placement specifier just for this example
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_car_Y1.pdf}
% % % \caption{First subfigure} \label{fig:a}
% % \end{subfigure}\hspace*{\fill}
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_car_Y0.pdf}
% % % \caption{Second subfigure} \label{fig:b}
% % \end{subfigure}
% % \caption{
% % Car loss difference ERM - GDRO by object cooccurrence frequency.
% % } \label{fig:results-coocc-car}
% % \end{figure}

% % \begin{figure}[t!] % "[t!]" placement specifier just for this example
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_backpack_Y1.pdf}
% % % \caption{First subfigure} \label{fig:a}
% % \end{subfigure}\hspace*{\fill}
% % \begin{subfigure}{0.48\textwidth}
% % \includegraphics[width=\linewidth]{figs/results/cooccurrence/cooccurrence_GDRO_backpack_Y0.pdf}
% % % \caption{Second subfigure} \label{fig:b}
% % \end{subfigure}
% % \caption{
% % Backpack loss difference ERM - GDRO by object cooccurrence frequency.
% % } \label{fig:results-coocc-car}
% % \end{figure}




% % \begin{itemize}
% %     \item Overall results: Error/NLL
% %     \begin{itemize}
% %         \item split into pos/neg
% %         \item hard/easy
% %         \item hard pos/hard neg
% %     \end{itemize}
% %     \item Results: calibration
% %     \begin{itemize}
% %         \item Split into hard/easy
% %     \end{itemize}
% %     \item Results: comparison of worst images in each condition
% %     \begin{itemize}
% %         \item Qualitative analysis - show samples
% %         \item discuss excessive invariance
% %         \item talk about which images co-occur most frequently with over/under-performance
% %     \end{itemize}
% % \end{itemize}

% % \begin{figure}
% %     \centering
% %     \includegraphics[scale=0.6]{figs/calib_new.png}
% %     \caption{Caption}
% %     \label{fig:my_label}
% % \end{figure}

==> sections/results_waterbirds.tex <==
\subsubsection{Comparison to Waterbirds}

\begin{table}[]
    \centering
    \resizebox{\columnwidth}{!}{%
    \input{figs/results/waterbirds/results_general}
    }
    \caption{AUC on ``hard'' test examples on the Waterbirds dataset.
    Hard examples are the union of two groups: land birds on water backgrounds and water birds on land backgrounds.
    Worst-group error or NLL takes the worse of the two; AUC-Hard calculates the AUC across the union.
    }
    \label{tab:waterbirds}
\end{table}

For comparison's sake, we show in Table \ref{tab:waterbirds} an analogous table of results for Waterbirds \citep{sagawa2019distributionally}, a semi-synthetic dataset which is generated by pasting images of birds on top of either either land or water backgrounds; the goal is to classify land birds from water birds.
At training time, land birds are mostly shown on land (and water birds on water), but at test time we hope to perform well, regardless of background.
The information regarding place is made available through environments: the four environments are land/land, land/water, etc.

In Table \ref{tab:waterbirds}, we see that there is a particularly large gap in performance between the best environment-based methods (particularly Group DRO) and the methods that do not use environments.
For instance, Group DRO and IRM improve over ERM by about 0.3 in worst-group error (the metric of choice in \citet{sagawa2019distributionally}); and Group DRO improves over \textit{all} other methods by about 0.14 in AUC on hard examples.
This difference is an order of magnitude greater than observed on \rococo, suggesting that semi-synthetic datasets where the environments fully specify the shift of interest (such as Waterbirds), may over-estimate the performance of current environment-based methods, and possibly Group DRO in particular.
The contrast between Tables \ref{tab:auc-by-task-ce}, \ref{tab:auc-by-task-gist} and Table \ref{tab:waterbirds} documents the usefulness of having benchmarks for robustness across a range of complexity, and motivates the creation of benchmarks such as \rococo.



==> sections/sections_rewrite_Sep6/nooch_methods_camera_ready.tex <==

\section{Evaluating Robustness Approaches on {\rococo }} \label{sec:methods}
We now turn to evaluating various ML methods on the {\rococo \ } benchmarks.
We choose to focus on four categories of methods which provide a useful contrast between different approaches to OOC prediction. 
Expected risk minimization (\textbf{ERM}) is the standard loss function in ML systems; as shown by \citet{gulrajani2020search}, it can be difficult to beat on domain generalization problems.
Label-based adjustments (\textbf{Reweight} and \textbf{US}) use information about label imbalance at training time to adjust the loss function towards performing better on unusual labels.
Environment-based methods (\textbf{GDRO} \citep{sagawa2019distributionally}, \textbf{IRM} \citep{arjovsky2019invariant}, \textbf{Reweight-Envs}, \textbf{US-Envs}) use categorical auxiliary information (i.e. \textit{environments}) at training time to adjust the loss function towards performing better on unusual subgroups.
Finally, adaptive methods (\textbf{CVaR} (\citep{rockafellar2002conditional}) and \textbf{Focal} \citep{lin2017focal}) do not use auxiliary information at all, but instead try to infer adaptively from the input during training what the worst-performing subgroups should be.
See App. \ref{app:other-methods} for information on other methods we experimented with but did not include here.
We found the methods we included here had the best results overall, on the standard and hard examples. 


Throughout, we use the following notation.
We are given a dataset $\{x_i, y_i\}_{i=1}^n$ with inputs and target labels respectively, and possibly some side information $\{ c_i \}_{i=1}^n$ as well (e.g. environment variables).
If side information is available, we assume it is available at training time but not necessarily test time.
We are aiming to learn a function $f: \mathds{X} \longrightarrow \mathds{Y}$.
We assume $\ell$ to be the the example-wise cross-entropy loss function.


\paragraph{Expected Risk Minimization.}
Expected risk minimization (ERM) is the standard paradigm for training ML models.
In ERM, we minimize the mean loss $\ell$ on the training set, plus potentially some data-independent regularizer $\mathcal{R}$:
\begin{equation}
    \mathcal{L}_{ERM}(f) = \frac{1}{n} \sum_{i=1}^n \ell(f(x_i), y_i) + \mathcal{R}(f)
\end{equation}


\paragraph{Label-Based Adjustments.}
Since COCO-Stuff contains significant label imbalance, we consider methods intended to correct for label imbalance.
We let $w_i = P(Y = y_i)$ in the training set.
To make a fairer comparison with the environment-based methods (below), we add a tuning parameter $\alpha$ to control the degree of adjustment.
$\alpha = 1$ represents the standard versions of these loss functions, but we frequently found other values $\alpha \in [0, 2]$ to be useful.
We can then weight the loss for each example proportionally to $(\frac{1}{w_i})^\alpha$ (label reweighting), or sample each point with probability proportional to $(\frac{1}{w_i})^\alpha$ (label undersampling).

% \paragraph{Label Reweighting.}
% We reweight the loss of each training example in the ERM loss function, inversely proportional (when $\alpha = 1$) to the likelihood of observing that label:
% \begin{equation}
%     \mathcal{L}_{Reweight}(f) = \frac{1}{n} \sum_{i=1}^n (\frac{1}{w_i})^\alpha \ell(f(x_i), y_i) + \mathcal{R}(f)
% \end{equation}

% \paragraph{Label Undersampling.}
% Rather than sampling training examples uniformly, we sample them with probability inversely proportional (when $\alpha = 1$) to the likelihood of observing that label.
% We let $\mathcal{I}$ be a list of indices of size $n$, sampled independently from $[1 \dots n]$, such that for each $j \in \mathcal{I}$, $P(j = i)$ is proportional to $(\frac{1}{w_i})^\alpha$.
% We redraw this for the training set every epoch and weight their losses equally as follows:
% \begin{equation}
%     \mathcal{L}_{Undersampling}(f) = \frac{1}{n} \sum_{i \in \mathcal{I}} \ell(f(x_i), y_i) + \mathcal{R}(f)
% \end{equation}

\subsection{Environment-Based Methods}
One common setting is where the auxiliary information $c_i$ for each example is a categorical variable, representing an \textit{environment}.
The notion of environments for robust learning was originally given with causal motivation \citep{peters2016causal}, where each value of $c$ represents a different intervention on the underlying causal graph.
However, this type of grouping procedure can be used completely separately from the causal context, and so we just consider it to represent some informative partition of our data, which is defined as an input at training time.
Here, $c \in \{ 1 \dots C \}$ is an integer or a one-hot encoded variable.
We will use the following shorthand to describe the average loss for an environment, with $n_c$ referring to the number of examples in that environment: 
\begin{equation}
    \ell_c (f) = \frac{1}{n_c} \sum_{i=1}^{n} \ell(f(x_i), y_i) \one \{ c_i = c \}
\end{equation}
% We consider two popular environment-based learning algorithms.

\paragraph{Group DRO.}
The first environment-based method we consider is Group Distributionally Robust Optimization (GDRO) \citep{sagawa2019distributionally}, which aims to minimize the loss on the worst of $C$ partitions, with partition $c$ of size $n_c$, and group adjustment hyperparameter $K$:
\begin{equation}
    \mathcal{L}_{GDRO}(f) = \underset{c \in \{ 1 \dots C \}}{\max} \Big\{  \ell_c (f) + \frac{K}{\sqrt{n_c}}  \Big\} + \mathcal{R}(f)
\end{equation}
This loss aims to ensure that no group's loss is that bad, and the group adjustment term ensures greater focus on smaller groups, which may otherwise be ignored.

\paragraph{IRM.}
The second environment-based method we consider is invariant risk minimization (IRM) \citep{arjovsky2019invariant}:
% , which uses the following loss function
\begin{equation}
    \mathcal{L}_{IRM}(f) = \sum_{c=1}^C  \ell_c (f) + \lambda \| \nabla_{w | w=1} \ell_c (w \cdot f) \| + \mathcal{R}(f)
\end{equation}
The second term here is a gradient penalty on the output of $f$, $w$ is a constant multiplier on the output of $f$, and $\lambda$ is a hyperparameter.
The intuition for this is somewhat involved \citep{arjovsky2019invariant}; the overarching motivation is that each environment should learn a representation such that the same predictive classifier is optimal across environments.

\paragraph{Environment Reweighting and Undersampling.}
These are equivalent to label reweighting/undersampling above, but with $w_i = P(C = c_i)$.





\subsection{Adaptive Methods}

Finally, we consider a class of loss functions which, rather than using an injection of side information to specify which examples are OOC, focuses dynamically on the hardest examples at each step.
The first is conditional variance-at-risk optimization (CVaR).
This can be cast as a type of distributionally robust optimization (DRO) \citep{duchi2021statistics}, where we aim to maximize the loss over, rather than the whole training set, a worst-case distribution over training examples.
For some $p \in (0, 1)$, CVaR($p$) is defined as the average loss of the $p$-percent worst-loss examples.

We also consider focal loss \citep{lin2017focal}, which dynamically upweights high loss examples using a parameter $\gamma \geq 0$.
With binary $y$, $q(x, y) = f(x)$ if $y = 1$ and $q(x) = 1 - f(x)$ if $y = 0$, with $f(x) \in [0, 1]$ as the continuous-scored output of $f$, not the binary prediction.
Then, we have focal loss as a modification of the cross-entropy loss --- at $\gamma=0$ this reduces to cross-entropy; as $\gamma$ increases, it focuses more loss on the examples which have higher loss already:
\begin{equation}
    \mathcal{L}_{Focal}(f) = \frac{1}{n} \sum_{i=1}^n -(1 - q(x_i, y))^\gamma \log(q(x_i, y)) + \mathcal{R}(f)
\end{equation}



==> tables/app_stds_old/results_area_auc_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & \textbf{0.988 (0.000)} & 0.765 (0.044) & 0.959 (0.003)          & \textbf{0.987 (0.002)} & \textbf{0.988 (0.000)} \\
 bowl         & 0.983 (0.000)          & 0.927 (0.017) & 0.943 (0.007)          & 0.975 (0.003)          & \textbf{0.983 (0.000)} \\
 boat         & 0.995 (0.000)          & 0.961 (0.011) & 0.945 (0.022)          & \textbf{0.996 (0.001)} & \textbf{0.996 (0.000)} \\
 fire-hydrant & 0.979 (0.001)          & 0.962 (0.003) & 0.972 (0.005)          & 0.982 (0.003)          & \textbf{0.986 (0.001)} \\
 airplane     & 0.997 (0.001)          & 0.989 (0.003) & \textbf{0.998 (0.002)} & \textbf{0.999 (0.001)} & \textbf{0.998 (0.000)} \\
 cow          & 0.995 (0.001)          & 0.981 (0.007) & 0.995 (0.001)          & 0.995 (0.001)          & \textbf{0.997 (0.000)} \\
 backpack     & 0.932 (0.001)          & 0.898 (0.014) & 0.903 (0.011)          & 0.850 (0.018)          & \textbf{0.937 (0.001)} \\
 cup          & \textbf{0.966 (0.001)} & 0.922 (0.007) & 0.921 (0.007)          & 0.941 (0.006)          & \textbf{0.966 (0.000)} \\
 surfboard    & 0.998 (0.000)          & 0.980 (0.004) & 0.989 (0.003)          & \textbf{0.998 (0.000)} & \textbf{0.998 (0.000)} \\
 tie          & 0.987 (0.001)          & 0.983 (0.003) & 0.876 (0.024)          & \textbf{0.983 (0.006)} & \textbf{0.989 (0.000)} \\
 sports-ball  & \textbf{0.993 (0.000)} & 0.962 (0.004) & 0.951 (0.014)          & \textbf{0.994 (0.000)} & \textbf{0.994 (0.000)} \\
 kite         & 0.999 (0.000)          & 0.996 (0.000) & 0.997 (0.000)          & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
\hline
 Average      & 0.984 (0.000)          & 0.944 (0.004) & 0.954 (0.003)          & 0.975 (0.002)          & \textbf{0.986 (0.000)} \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_auc_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & 0.769 (0.002)          & \textbf{0.923 (0.001)} & 0.868 (0.004)          & 0.780 (0.010)          & 0.773 (0.001)          \\
 bowl         & 0.749 (0.003)          & \textbf{0.846 (0.013)} & \textbf{0.828 (0.023)} & 0.701 (0.009)          & 0.751 (0.005)          \\
 boat         & 0.869 (0.002)          & \textbf{0.945 (0.012)} & 0.909 (0.014)          & 0.894 (0.021)          & 0.854 (0.007)          \\
 fire-hydrant & 0.913 (0.004)          & \textbf{0.942 (0.004)} & 0.902 (0.008)          & 0.933 (0.003)          & 0.925 (0.001)          \\
 airplane     & 0.986 (0.002)          & \textbf{0.995 (0.001)} & 0.986 (0.003)          & 0.984 (0.002)          & 0.983 (0.001)          \\
 cow          & 0.935 (0.003)          & \textbf{0.963 (0.004)} & 0.943 (0.001)          & 0.922 (0.007)          & 0.939 (0.002)          \\
 backpack     & 0.812 (0.004)          & \textbf{0.849 (0.012)} & \textbf{0.811 (0.032)} & 0.755 (0.034)          & 0.816 (0.003)          \\
 cup          & \textbf{0.870 (0.004)} & 0.825 (0.019)          & 0.820 (0.025)          & 0.794 (0.020)          & \textbf{0.868 (0.002)} \\
 surfboard    & 0.939 (0.002)          & \textbf{0.960 (0.004)} & \textbf{0.957 (0.008)} & 0.937 (0.003)          & 0.935 (0.000)          \\
 tie          & 0.742 (0.002)          & \textbf{0.781 (0.036)} & 0.640 (0.029)          & \textbf{0.696 (0.075)} & \textbf{0.743 (0.006)} \\
 sports-ball  & 0.867 (0.002)          & \textbf{0.909 (0.001)} & \textbf{0.859 (0.050)} & 0.856 (0.008)          & 0.865 (0.001)          \\
 kite         & 0.932 (0.001)          & \textbf{0.960 (0.005)} & \textbf{0.953 (0.004)} & 0.931 (0.004)          & 0.940 (0.001)          \\
\hline
 Average      & 0.865 (0.001)          & \textbf{0.908 (0.004)} & 0.873 (0.006)          & 0.849 (0.007)          & 0.866 (0.001)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_ece_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR          & Focal                  \\
\hline
 car          & \textbf{0.008 (0.001)} & 0.116 (0.082) & 0.054 (0.013) & 0.198 (0.039) & 0.016 (0.002)          \\
 bowl         & \textbf{0.007 (0.001)} & 0.125 (0.029) & 0.057 (0.016) & 0.395 (0.001) & 0.012 (0.001)          \\
 boat         & \textbf{0.002 (0.000)} & 0.093 (0.028) & 0.119 (0.007) & 0.022 (0.003) & 0.014 (0.002)          \\
 fire-hydrant & \textbf{0.001 (0.000)} & 0.069 (0.015) & 0.069 (0.009) & 0.016 (0.005) & 0.010 (0.001)          \\
 airplane     & \textbf{0.000 (0.000)} & 0.020 (0.004) & 0.004 (0.001) & 0.002 (0.000) & 0.015 (0.002)          \\
 cow          & \textbf{0.000 (0.000)} & 0.044 (0.016) & 0.013 (0.001) & 0.013 (0.005) & 0.007 (0.000)          \\
 backpack     & \textbf{0.003 (0.000)} & 0.065 (0.009) & 0.042 (0.026) & 0.308 (0.001) & 0.010 (0.002)          \\
 cup          & \textbf{0.003 (0.001)} & 0.080 (0.015) & 0.068 (0.002) & 0.295 (0.005) & \textbf{0.004 (0.001)} \\
 surfboard    & \textbf{0.001 (0.000)} & 0.023 (0.003) & 0.018 (0.002) & 0.004 (0.001) & 0.009 (0.001)          \\
 tie          & \textbf{0.002 (0.000)} & 0.077 (0.023) & 0.131 (0.036) & 0.097 (0.018) & 0.033 (0.003)          \\
 sports-ball  & \textbf{0.002 (0.000)} & 0.053 (0.019) & 0.071 (0.007) & 0.042 (0.013) & 0.018 (0.001)          \\
 kite         & \textbf{0.000 (0.000)} & 0.013 (0.004) & 0.015 (0.005) & 0.001 (0.000) & 0.008 (0.001)          \\
\hline
 Average      & \textbf{0.003 (0.000)} & 0.065 (0.008) & 0.055 (0.004) & 0.116 (0.004) & 0.013 (0.000)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_ece_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & 0.017 (0.001)          & 0.008 (0.001)          & \textbf{0.004 (0.001)} & \textbf{0.005 (0.002)} & 0.012 (0.000)          \\
 bowl         & 0.013 (0.001)          & 0.008 (0.002)          & \textbf{0.005 (0.001)} & 0.011 (0.000)          & 0.009 (0.000)          \\
 boat         & 0.004 (0.000)          & \textbf{0.002 (0.000)} & 0.005 (0.001)          & \textbf{0.002 (0.000)} & 0.004 (0.000)          \\
 fire-hydrant & 0.002 (0.000)          & 0.004 (0.001)          & 0.007 (0.002)          & \textbf{0.001 (0.000)} & \textbf{0.001 (0.000)} \\
 airplane     & 0.001 (0.000)          & 0.001 (0.001)          & 0.001 (0.000)          & \textbf{0.000 (0.000)} & 0.005 (0.001)          \\
 cow          & 0.002 (0.000)          & \textbf{0.001 (0.001)} & \textbf{0.001 (0.000)} & \textbf{0.002 (0.001)} & \textbf{0.001 (0.000)} \\
 backpack     & \textbf{0.006 (0.001)} & \textbf{0.007 (0.003)} & 0.011 (0.003)          & 0.108 (0.003)          & 0.022 (0.001)          \\
 cup          & \textbf{0.009 (0.001)} & \textbf{0.021 (0.011)} & 0.034 (0.016)          & 0.113 (0.002)          & 0.018 (0.001)          \\
 surfboard    & 0.002 (0.000)          & 0.004 (0.001)          & 0.005 (0.001)          & \textbf{0.001 (0.000)} & 0.004 (0.000)          \\
 tie          & \textbf{0.002 (0.000)} & 0.009 (0.002)          & 0.023 (0.007)          & 0.039 (0.004)          & 0.010 (0.001)          \\
 sports-ball  & \textbf{0.002 (0.000)} & 0.021 (0.004)          & 0.035 (0.005)          & 0.023 (0.006)          & 0.017 (0.001)          \\
 kite         & \textbf{0.001 (0.000)} & 0.002 (0.001)          & 0.005 (0.002)          & \textbf{0.001 (0.000)} & 0.002 (0.000)          \\
\hline
 Average      & \textbf{0.005 (0.000)} & 0.007 (0.001)          & 0.011 (0.002)          & 0.025 (0.001)          & 0.009 (0.000)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_err_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & 0.020 (0.001)          & 0.465 (0.104) & 0.068 (0.013) & \textbf{0.019 (0.001)} & 0.031 (0.001) \\
 bowl         & \textbf{0.018 (0.001)} & 0.107 (0.020) & 0.077 (0.005) & \textbf{0.019 (0.001)} & 0.034 (0.001) \\
 boat         & 0.004 (0.000)          & 0.089 (0.012) & 0.092 (0.059) & \textbf{0.004 (0.000)} & 0.016 (0.001) \\
 fire-hydrant & 0.003 (0.000)          & 0.027 (0.001) & 0.040 (0.029) & \textbf{0.002 (0.000)} & 0.020 (0.001) \\
 airplane     & \textbf{0.001 (0.000)} & 0.031 (0.009) & 0.003 (0.001) & \textbf{0.001 (0.000)} & 0.007 (0.001) \\
 cow          & 0.003 (0.000)          & 0.026 (0.003) & 0.009 (0.001) & \textbf{0.003 (0.000)} & 0.009 (0.000) \\
 backpack     & \textbf{0.028 (0.000)} & 0.135 (0.013) & 0.146 (0.024) & 0.038 (0.005)          & 0.109 (0.002) \\
 cup          & \textbf{0.039 (0.000)} & 0.145 (0.015) & 0.125 (0.010) & 0.052 (0.004)          & 0.094 (0.002) \\
 surfboard    & \textbf{0.004 (0.000)} & 0.041 (0.017) & 0.016 (0.005) & \textbf{0.005 (0.001)} & 0.011 (0.000) \\
 tie          & \textbf{0.011 (0.000)} & 0.080 (0.016) & 0.260 (0.035) & \textbf{0.013 (0.002)} & 0.032 (0.002) \\
 sports-ball  & \textbf{0.013 (0.000)} & 0.079 (0.017) & 0.093 (0.024) & \textbf{0.014 (0.001)} & 0.021 (0.002) \\
 kite         & \textbf{0.002 (0.000)} & 0.024 (0.008) & 0.021 (0.002) & \textbf{0.002 (0.000)} & 0.010 (0.001) \\
\hline
 Average      & \textbf{0.012 (0.000)} & 0.104 (0.009) & 0.079 (0.007) & 0.014 (0.001)          & 0.033 (0.000) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_err_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal         \\
\hline
 car          & 0.314 (0.005)          & \textbf{0.151 (0.004)} & 0.217 (0.007)          & 0.327 (0.011)          & 0.289 (0.000) \\
 bowl         & 0.317 (0.007)          & \textbf{0.228 (0.013)} & \textbf{0.235 (0.015)} & 0.353 (0.003)          & 0.303 (0.003) \\
 boat         & \textbf{0.149 (0.002)} & \textbf{0.135 (0.024)} & \textbf{0.149 (0.046)} & \textbf{0.142 (0.011)} & 0.239 (0.020) \\
 fire-hydrant & 0.053 (0.001)          & 0.066 (0.003)          & 0.133 (0.062)          & \textbf{0.046 (0.000)} & 0.130 (0.006) \\
 airplane     & 0.011 (0.000)          & 0.015 (0.001)          & 0.016 (0.002)          & \textbf{0.011 (0.000)} & 0.039 (0.004) \\
 cow          & \textbf{0.037 (0.001)} & 0.061 (0.010)          & 0.061 (0.006)          & 0.043 (0.003)          & 0.078 (0.002) \\
 backpack     & \textbf{0.087 (0.002)} & 0.226 (0.010)          & 0.266 (0.029)          & \textbf{0.097 (0.014)} & 0.271 (0.001) \\
 cup          & \textbf{0.100 (0.001)} & 0.296 (0.046)          & 0.234 (0.054)          & 0.123 (0.010)          & 0.214 (0.007) \\
 surfboard    & 0.025 (0.001)          & 0.055 (0.021)          & 0.030 (0.005)          & \textbf{0.022 (0.001)} & 0.084 (0.001) \\
 tie          & 0.032 (0.001)          & 0.248 (0.037)          & 0.466 (0.059)          & \textbf{0.028 (0.003)} & 0.185 (0.011) \\
 sports-ball  & 0.031 (0.001)          & 0.143 (0.039)          & 0.175 (0.041)          & \textbf{0.025 (0.003)} & 0.144 (0.003) \\
 kite         & \textbf{0.007 (0.001)} & 0.033 (0.011)          & 0.063 (0.005)          & \textbf{0.006 (0.001)} & 0.062 (0.008) \\
 Average      & \textbf{0.097 (0.001)} & 0.138 (0.007)          & 0.170 (0.010)          & 0.102 (0.002)          & 0.170 (0.002) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_err_loss_neg_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM                    & CVAR                   & Focal         \\
\hline
 car          & 0.118 (0.009)          & 0.176 (0.029) & 0.158 (0.053)          & \textbf{0.084 (0.019)} & 0.269 (0.006) \\
 bowl         & \textbf{0.087 (0.016)} & 0.220 (0.030) & 0.191 (0.027)          & \textbf{0.113 (0.043)} & 0.274 (0.017) \\
 boat         & \textbf{0.052 (0.004)} & 0.130 (0.044) & \textbf{0.113 (0.090)} & \textbf{0.037 (0.022)} & 0.266 (0.028) \\
 fire-hydrant & \textbf{0.004 (0.001)} & 0.041 (0.003) & 0.117 (0.078)          & \textbf{0.003 (0.001)} & 0.119 (0.007) \\
 airplane     & \textbf{0.002 (0.000)} & 0.012 (0.002) & 0.010 (0.002)          & \textbf{0.002 (0.001)} & 0.038 (0.004) \\
 cow          & \textbf{0.011 (0.001)} & 0.051 (0.012) & 0.045 (0.007)          & \textbf{0.010 (0.001)} & 0.068 (0.002) \\
 backpack     & \textbf{0.018 (0.002)} & 0.225 (0.009) & 0.266 (0.035)          & \textbf{0.022 (0.019)} & 0.274 (0.002) \\
 cup          & \textbf{0.037 (0.001)} & 0.303 (0.051) & 0.226 (0.061)          & 0.060 (0.011)          & 0.217 (0.008) \\
 surfboard    & \textbf{0.013 (0.001)} & 0.051 (0.022) & 0.023 (0.006)          & \textbf{0.008 (0.003)} & 0.080 (0.002) \\
 tie          & 0.014 (0.000)          & 0.245 (0.038) & 0.468 (0.061)          & \textbf{0.010 (0.003)} & 0.178 (0.012) \\
 sports-ball  & 0.020 (0.001)          & 0.142 (0.041) & 0.173 (0.041)          & \textbf{0.013 (0.004)} & 0.141 (0.003) \\
 kite         & \textbf{0.004 (0.001)} & 0.031 (0.012) & 0.063 (0.004)          & \textbf{0.003 (0.001)} & 0.061 (0.008) \\
\hline
 Average      & \textbf{0.032 (0.002)} & 0.136 (0.008) & 0.154 (0.014)          & \textbf{0.030 (0.005)} & 0.165 (0.003) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_err_loss_pos_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM           & GDRO                   & IRM                    & CVAR          & Focal                  \\
\hline
 car          & 0.435 (0.012) & \textbf{0.136 (0.011)} & 0.253 (0.041)          & 0.476 (0.030) & 0.301 (0.003)          \\
 bowl         & 0.581 (0.032) & \textbf{0.239 (0.007)} & 0.286 (0.023)          & 0.627 (0.054) & 0.336 (0.014)          \\
 boat         & 0.353 (0.009) & \textbf{0.145 (0.020)} & 0.225 (0.055)          & 0.362 (0.028) & 0.183 (0.002)          \\
 fire-hydrant & 0.460 (0.011) & 0.268 (0.026)          & \textbf{0.268 (0.070)} & 0.406 (0.010) & \textbf{0.217 (0.004)} \\
 airplane     & 0.137 (0.008) & \textbf{0.056 (0.007)} & 0.090 (0.013)          & 0.125 (0.013) & \textbf{0.054 (0.003)} \\
 cow          & 0.357 (0.009) & \textbf{0.187 (0.016)} & 0.249 (0.015)          & 0.445 (0.027) & \textbf{0.192 (0.002)} \\
 backpack     & 0.822 (0.003) & \textbf{0.238 (0.014)} & \textbf{0.271 (0.082)} & 0.883 (0.039) & \textbf{0.237 (0.007)} \\
 cup          & 0.678 (0.011) & 0.223 (0.018)          & 0.310 (0.022)          & 0.704 (0.013) & \textbf{0.186 (0.006)} \\
 surfboard    & 0.372 (0.014) & \textbf{0.161 (0.018)} & 0.220 (0.037)          & 0.388 (0.061) & \textbf{0.175 (0.012)} \\
 tie          & 0.831 (0.006) & \textbf{0.380 (0.028)} & \textbf{0.348 (0.018)} & 0.863 (0.043) & 0.512 (0.009)          \\
 sports-ball  & 0.521 (0.022) & \textbf{0.205 (0.053)} & \textbf{0.243 (0.040)} & 0.563 (0.081) & \textbf{0.258 (0.009)} \\
 kite         & 0.388 (0.034) & \textbf{0.176 (0.043)} & \textbf{0.152 (0.017)} & 0.370 (0.031) & 0.206 (0.009)          \\
\hline
 Average      & 0.495 (0.005) & \textbf{0.201 (0.007)} & 0.243 (0.012)          & 0.518 (0.012) & 0.238 (0.002)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_nll_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & \textbf{0.059 (0.002)} & 0.782 (0.084) & 0.222 (0.028) & 0.286 (0.057)          & 0.095 (0.001) \\
 bowl         & \textbf{0.051 (0.002)} & 0.352 (0.067) & 0.223 (0.011) & 0.600 (0.003)          & 0.096 (0.004) \\
 boat         & \textbf{0.015 (0.000)} & 0.295 (0.009) & 0.306 (0.098) & 0.033 (0.003)          & 0.057 (0.004) \\
 fire-hydrant & \textbf{0.012 (0.000)} & 0.140 (0.021) & 0.161 (0.062) & 0.023 (0.006)          & 0.059 (0.001) \\
 airplane     & \textbf{0.006 (0.000)} & 0.101 (0.025) & 0.013 (0.003) & \textbf{0.007 (0.001)} & 0.035 (0.003) \\
 cow          & \textbf{0.011 (0.000)} & 0.118 (0.020) & 0.038 (0.002) & 0.022 (0.005)          & 0.035 (0.000) \\
 backpack     & \textbf{0.086 (0.001)} & 0.363 (0.032) & 0.359 (0.026) & 0.636 (0.007)          & 0.281 (0.003) \\
 cup          & \textbf{0.103 (0.002)} & 0.398 (0.037) & 0.329 (0.021) & 0.651 (0.006)          & 0.229 (0.007) \\
 surfboard    & \textbf{0.014 (0.001)} & 0.133 (0.043) & 0.060 (0.013) & 0.016 (0.001)          & 0.041 (0.001) \\
 tie          & \textbf{0.035 (0.001)} & 0.275 (0.049) & 0.609 (0.015) & 0.167 (0.029)          & 0.121 (0.006) \\
 sports-ball  & \textbf{0.033 (0.000)} & 0.264 (0.040) & 0.305 (0.043) & 0.086 (0.019)          & 0.081 (0.006) \\
 kite         & \textbf{0.008 (0.000)} & 0.082 (0.024) & 0.075 (0.007) & \textbf{0.008 (0.001)} & 0.041 (0.005) \\
\hline
 Average      & \textbf{0.036 (0.000)} & 0.275 (0.012) & 0.225 (0.011) & 0.211 (0.006)          & 0.098 (0.001) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_nll_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal         \\
\hline
 car          & 0.789 (0.018)          & \textbf{0.377 (0.012)} & 0.465 (0.002)          & 0.583 (0.018)          & 0.662 (0.008) \\
 bowl         & 0.774 (0.023)          & \textbf{0.517 (0.025)} & \textbf{0.519 (0.022)} & 0.682 (0.000)          & 0.671 (0.002) \\
 boat         & 0.490 (0.006)          & \textbf{0.322 (0.054)} & \textbf{0.410 (0.065)} & \textbf{0.371 (0.031)} & 0.609 (0.026) \\
 fire-hydrant & 0.196 (0.004)          & 0.210 (0.020)          & 0.353 (0.088)          & \textbf{0.151 (0.004)} & 0.305 (0.008) \\
 airplane     & \textbf{0.041 (0.001)} & 0.054 (0.009)          & 0.053 (0.006)          & \textbf{0.040 (0.002)} & 0.138 (0.011) \\
 cow          & \textbf{0.128 (0.004)} & 0.175 (0.028)          & 0.166 (0.010)          & \textbf{0.134 (0.009)} & 0.224 (0.004) \\
 backpack     & \textbf{0.246 (0.003)} & 0.462 (0.006)          & 0.542 (0.035)          & 0.650 (0.006)          & 0.606 (0.007) \\
 cup          & \textbf{0.246 (0.005)} & 0.586 (0.036)          & 0.523 (0.035)          & 0.673 (0.004)          & 0.527 (0.015) \\
 surfboard    & 0.083 (0.001)          & 0.164 (0.045)          & 0.104 (0.016)          & \textbf{0.072 (0.005)} & 0.247 (0.004) \\
 tie          & \textbf{0.120 (0.002)} & 0.552 (0.064)          & 0.673 (0.004)          & 0.227 (0.012)          & 0.479 (0.023) \\
 sports-ball  & \textbf{0.100 (0.002)} & 0.402 (0.065)          & 0.481 (0.077)          & 0.151 (0.017)          & 0.457 (0.016) \\
 kite         & \textbf{0.030 (0.001)} & 0.101 (0.030)          & 0.192 (0.017)          & \textbf{0.027 (0.002)} & 0.182 (0.019) \\
 Average      & \textbf{0.270 (0.003)} & 0.327 (0.011)          & 0.373 (0.012)          & 0.313 (0.004)          & 0.426 (0.004) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_nll_loss_neg_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & \textbf{0.330 (0.019)} & 0.487 (0.038) & 0.471 (0.106) & 0.444 (0.061)          & 0.643 (0.014) \\
 bowl         & \textbf{0.241 (0.033)} & 0.550 (0.039) & 0.510 (0.033) & 0.665 (0.005)          & 0.629 (0.031) \\
 boat         & \textbf{0.165 (0.007)} & 0.340 (0.089) & 0.409 (0.117) & \textbf{0.158 (0.056)} & 0.682 (0.044) \\
 fire-hydrant & \textbf{0.023 (0.003)} & 0.178 (0.023) & 0.343 (0.108) & 0.050 (0.013)          & 0.290 (0.010) \\
 airplane     & \textbf{0.009 (0.001)} & 0.047 (0.012) & 0.038 (0.008) & \textbf{0.013 (0.003)} & 0.138 (0.012) \\
 cow          & \textbf{0.034 (0.001)} & 0.156 (0.033) & 0.131 (0.013) & 0.054 (0.011)          & 0.201 (0.005) \\
 backpack     & \textbf{0.077 (0.005)} & 0.457 (0.005) & 0.544 (0.045) & 0.644 (0.007)          & 0.617 (0.008) \\
 cup          & \textbf{0.106 (0.004)} & 0.597 (0.039) & 0.518 (0.042) & 0.670 (0.005)          & 0.538 (0.018) \\
 surfboard    & \textbf{0.031 (0.003)} & 0.156 (0.050) & 0.088 (0.018) & \textbf{0.032 (0.009)} & 0.237 (0.004) \\
 tie          & \textbf{0.051 (0.002)} & 0.551 (0.066) & 0.673 (0.004) & 0.201 (0.014)          & 0.466 (0.025) \\
 sports-ball  & \textbf{0.057 (0.002)} & 0.402 (0.068) & 0.481 (0.079) & 0.128 (0.018)          & 0.452 (0.017) \\
 kite         & \textbf{0.014 (0.002)} & 0.098 (0.032) & 0.190 (0.017) & \textbf{0.013 (0.003)} & 0.180 (0.019) \\
\hline
 Average      & \textbf{0.095 (0.003)} & 0.335 (0.014) & 0.366 (0.018) & 0.256 (0.007)          & 0.423 (0.006) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_area_nll_loss_pos_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM           & GDRO                   & IRM                    & CVAR          & Focal                  \\
\hline
 car          & 1.072 (0.041) & \textbf{0.309 (0.012)} & 0.461 (0.068)          & 0.669 (0.064) & 0.673 (0.009)          \\
 bowl         & 1.385 (0.088) & \textbf{0.480 (0.011)} & 0.529 (0.030)          & 0.702 (0.005) & 0.720 (0.032)          \\
 boat         & 1.171 (0.033) & \textbf{0.285 (0.021)} & 0.413 (0.060)          & 0.817 (0.049) & 0.454 (0.012)          \\
 fire-hydrant & 1.639 (0.040) & 0.472 (0.020)          & \textbf{0.437 (0.076)} & 0.996 (0.069) & \textbf{0.429 (0.005)} \\
 airplane     & 0.485 (0.025) & \textbf{0.150 (0.032)} & 0.272 (0.050)          & 0.420 (0.069) & \textbf{0.144 (0.002)} \\
 cow          & 1.272 (0.037) & \textbf{0.410 (0.036)} & 0.584 (0.027)          & 1.102 (0.064) & 0.497 (0.008)          \\
 backpack     & 2.035 (0.049) & \textbf{0.511 (0.021)} & \textbf{0.523 (0.094)} & 0.719 (0.003) & \textbf{0.492 (0.010)} \\
 cup          & 1.538 (0.073) & 0.479 (0.009)          & 0.573 (0.028)          & 0.698 (0.001) & \textbf{0.427 (0.015)} \\
 surfboard    & 1.496 (0.076) & \textbf{0.371 (0.083)} & 0.525 (0.066)          & 1.163 (0.115) & 0.530 (0.006)          \\
 tie          & 3.357 (0.034) & \textbf{0.631 (0.049)} & \textbf{0.672 (0.001)} & 1.447 (0.148) & 1.054 (0.035)          \\
 sports-ball  & 1.991 (0.031) & \textbf{0.374 (0.062)} & \textbf{0.469 (0.065)} & 1.127 (0.062) & 0.663 (0.030)          \\
 kite         & 1.925 (0.014) & \textbf{0.561 (0.163)} & \textbf{0.396 (0.019)} & 1.753 (0.113) & 0.516 (0.048)          \\
\hline
 Average      & 1.614 (0.014) & \textbf{0.419 (0.017)} & 0.488 (0.016)          & 0.968 (0.022) & 0.550 (0.007)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_auc_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal                  \\
\hline
 car          & \textbf{0.990 (0.000)} & 0.930 (0.013) & 0.948 (0.014) & 0.989 (0.001)          & 0.990 (0.000)          \\
 bowl         & \textbf{0.991 (0.000)} & 0.959 (0.009) & 0.856 (0.035) & 0.984 (0.002)          & \textbf{0.990 (0.000)} \\
 boat         & \textbf{0.999 (0.000)} & 0.996 (0.001) & 0.956 (0.015) & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
 fire-hydrant & 0.999 (0.000)          & 0.998 (0.000) & 0.996 (0.002) & \textbf{0.998 (0.001)} & \textbf{0.999 (0.000)} \\
 airplane     & \textbf{1.000 (0.000)} & 1.000 (0.000) & 1.000 (0.000) & \textbf{1.000 (0.000)} & \textbf{1.000 (0.000)} \\
 cow          & 1.000 (0.000)          & 0.995 (0.003) & 0.997 (0.001) & 0.999 (0.000)          & \textbf{1.000 (0.000)} \\
 backpack     & \textbf{0.972 (0.001)} & 0.958 (0.002) & 0.942 (0.004) & 0.919 (0.021)          & \textbf{0.972 (0.000)} \\
 cup          & \textbf{0.995 (0.001)} & 0.950 (0.010) & 0.959 (0.014) & 0.975 (0.003)          & \textbf{0.995 (0.000)} \\
 surfboard    & 0.999 (0.000)          & 0.991 (0.003) & 0.983 (0.010) & 0.999 (0.000)          & \textbf{1.000 (0.000)} \\
 tie          & 0.978 (0.001)          & 0.978 (0.001) & 0.863 (0.028) & 0.972 (0.004)          & \textbf{0.981 (0.001)} \\
 sports-ball  & 0.999 (0.000)          & 0.968 (0.004) & 0.956 (0.018) & 0.998 (0.001)          & \textbf{0.999 (0.000)} \\
 kite         & 0.998 (0.000)          & 0.997 (0.000) & 0.997 (0.001) & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
\hline
 Average      & 0.993 (0.000)          & 0.977 (0.002) & 0.954 (0.005) & 0.986 (0.002)          & \textbf{0.994 (0.000)} \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_auc_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & 0.766 (0.002)          & \textbf{0.850 (0.014)} & \textbf{0.817 (0.026)} & 0.780 (0.010)          & 0.770 (0.003)          \\
 bowl         & 0.642 (0.004)          & \textbf{0.674 (0.019)} & 0.631 (0.014)          & 0.620 (0.021)          & \textbf{0.655 (0.009)} \\
 boat         & 0.826 (0.002)          & \textbf{0.880 (0.010)} & 0.818 (0.036)          & \textbf{0.855 (0.019)} & 0.806 (0.007)          \\
 fire-hydrant & 0.840 (0.007)          & 0.798 (0.011)          & 0.788 (0.018)          & \textbf{0.865 (0.008)} & 0.847 (0.002)          \\
 airplane     & 0.977 (0.001)          & \textbf{0.981 (0.002)} & 0.961 (0.001)          & 0.979 (0.000)          & 0.975 (0.002)          \\
 cow          & \textbf{0.901 (0.004)} & \textbf{0.906 (0.004)} & 0.845 (0.037)          & \textbf{0.900 (0.003)} & 0.895 (0.003)          \\
 backpack     & \textbf{0.716 (0.004)} & \textbf{0.732 (0.012)} & \textbf{0.729 (0.024)} & 0.604 (0.014)          & \textbf{0.731 (0.003)} \\
 cup          & \textbf{0.733 (0.006)} & \textbf{0.742 (0.015)} & \textbf{0.705 (0.041)} & 0.664 (0.008)          & \textbf{0.729 (0.007)} \\
 surfboard    & \textbf{0.913 (0.002)} & 0.875 (0.005)          & 0.836 (0.030)          & \textbf{0.918 (0.003)} & 0.903 (0.001)          \\
 tie          & \textbf{0.822 (0.003)} & \textbf{0.820 (0.018)} & 0.696 (0.014)          & 0.783 (0.028)          & \textbf{0.821 (0.004)} \\
 sports-ball  & 0.830 (0.003)          & \textbf{0.880 (0.001)} & 0.848 (0.029)          & 0.826 (0.011)          & 0.824 (0.002)          \\
 kite         & \textbf{0.942 (0.001)} & \textbf{0.947 (0.007)} & \textbf{0.943 (0.010)} & \textbf{0.940 (0.004)} & \textbf{0.947 (0.001)} \\
\hline
 Average      & 0.826 (0.001)          & \textbf{0.841 (0.003)} & 0.801 (0.008)          & 0.811 (0.004)          & 0.825 (0.001)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_ece_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & \textbf{0.010 (0.001)} & 0.125 (0.053) & 0.076 (0.026) & 0.199 (0.039)          & 0.017 (0.002) \\
 bowl         & \textbf{0.009 (0.001)} & 0.137 (0.030) & 0.113 (0.086) & 0.398 (0.001)          & 0.017 (0.001) \\
 boat         & \textbf{0.003 (0.000)} & 0.095 (0.028) & 0.079 (0.054) & 0.023 (0.003)          & 0.017 (0.002) \\
 fire-hydrant & \textbf{0.002 (0.000)} & 0.069 (0.015) & 0.072 (0.010) & 0.016 (0.006)          & 0.014 (0.001) \\
 airplane     & \textbf{0.001 (0.000)} & 0.028 (0.005) & 0.032 (0.014) & 0.002 (0.000)          & 0.016 (0.002) \\
 cow          & \textbf{0.001 (0.000)} & 0.046 (0.015) & 0.037 (0.018) & 0.013 (0.005)          & 0.009 (0.000) \\
 backpack     & \textbf{0.007 (0.000)} & 0.079 (0.013) & 0.059 (0.022) & 0.310 (0.002)          & 0.026 (0.001) \\
 cup          & \textbf{0.007 (0.001)} & 0.110 (0.022) & 0.091 (0.018) & 0.303 (0.002)          & 0.027 (0.002) \\
 surfboard    & \textbf{0.001 (0.000)} & 0.025 (0.002) & 0.057 (0.017) & 0.004 (0.001)          & 0.010 (0.001) \\
 tie          & \textbf{0.001 (0.000)} & 0.068 (0.022) & 0.120 (0.040) & 0.098 (0.016)          & 0.028 (0.002) \\
 sports-ball  & \textbf{0.003 (0.000)} & 0.062 (0.021) & 0.080 (0.007) & 0.044 (0.013)          & 0.025 (0.002) \\
 kite         & \textbf{0.000 (0.000)} & 0.013 (0.004) & 0.014 (0.005) & \textbf{0.001 (0.000)} & 0.010 (0.001) \\
\hline
 Average      & \textbf{0.004 (0.000)} & 0.071 (0.007) & 0.069 (0.010) & 0.118 (0.004)          & 0.018 (0.000) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_ece_loss_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal         \\
\hline
 car          & 0.019 (0.001)          & \textbf{0.006 (0.003)} & \textbf{0.003 (0.001)} & \textbf{0.006 (0.002)} & 0.013 (0.001) \\
 bowl         & 0.015 (0.001)          & \textbf{0.005 (0.001)} & \textbf{0.004 (0.001)} & 0.008 (0.001)          & 0.014 (0.000) \\
 boat         & 0.005 (0.000)          & \textbf{0.002 (0.001)} & \textbf{0.002 (0.000)} & \textbf{0.003 (0.000)} & 0.006 (0.000) \\
 fire-hydrant & 0.003 (0.000)          & 0.005 (0.002)          & 0.006 (0.002)          & \textbf{0.001 (0.000)} & 0.004 (0.001) \\
 airplane     & 0.001 (0.000)          & 0.003 (0.001)          & 0.008 (0.004)          & \textbf{0.001 (0.000)} & 0.004 (0.001) \\
 cow          & 0.002 (0.000)          & \textbf{0.003 (0.002)} & 0.003 (0.001)          & \textbf{0.002 (0.000)} & 0.004 (0.000) \\
 backpack     & \textbf{0.008 (0.000)} & \textbf{0.011 (0.003)} & \textbf{0.012 (0.009)} & 0.106 (0.003)          & 0.038 (0.001) \\
 cup          & \textbf{0.008 (0.002)} & 0.012 (0.002)          & 0.016 (0.006)          & 0.105 (0.003)          & 0.046 (0.002) \\
 surfboard    & 0.002 (0.000)          & 0.003 (0.000)          & 0.017 (0.003)          & \textbf{0.001 (0.000)} & 0.005 (0.000) \\
 tie          & \textbf{0.002 (0.000)} & 0.013 (0.003)          & 0.022 (0.007)          & 0.037 (0.005)          & 0.006 (0.001) \\
 sports-ball  & \textbf{0.004 (0.001)} & 0.014 (0.003)          & 0.025 (0.005)          & 0.023 (0.007)          & 0.023 (0.000) \\
 kite         & \textbf{0.001 (0.000)} & 0.002 (0.001)          & 0.005 (0.002)          & \textbf{0.001 (0.000)} & 0.002 (0.000) \\
\hline
 Average      & \textbf{0.006 (0.000)} & 0.007 (0.001)          & 0.010 (0.001)          & 0.024 (0.001)          & 0.014 (0.000) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_err_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal                  \\
\hline
 car          & \textbf{0.019 (0.001)} & 0.131 (0.025) & 0.109 (0.034) & \textbf{0.017 (0.001)} & 0.030 (0.000)          \\
 bowl         & \textbf{0.014 (0.000)} & 0.092 (0.019) & 0.238 (0.040) & 0.016 (0.001)          & 0.026 (0.002)          \\
 boat         & 0.003 (0.000)          & 0.085 (0.012) & 0.194 (0.109) & \textbf{0.002 (0.000)} & 0.013 (0.001)          \\
 fire-hydrant & \textbf{0.001 (0.000)} & 0.020 (0.002) & 0.033 (0.027) & \textbf{0.001 (0.000)} & 0.014 (0.001)          \\
 airplane     & 0.001 (0.000)          & 0.008 (0.001) & 0.013 (0.004) & \textbf{0.000 (0.000)} & 0.005 (0.001)          \\
 cow          & \textbf{0.002 (0.000)} & 0.020 (0.003) & 0.014 (0.003) & 0.002 (0.000)          & 0.004 (0.000)          \\
 backpack     & \textbf{0.023 (0.000)} & 0.095 (0.004) & 0.120 (0.021) & 0.034 (0.005)          & 0.083 (0.001)          \\
 cup          & 0.028 (0.000)          & 0.103 (0.024) & 0.076 (0.028) & 0.039 (0.001)          & \textbf{0.026 (0.002)} \\
 surfboard    & \textbf{0.003 (0.000)} & 0.031 (0.015) & 0.043 (0.021) & \textbf{0.003 (0.001)} & 0.005 (0.000)          \\
 tie          & \textbf{0.011 (0.000)} & 0.091 (0.015) & 0.279 (0.042) & \textbf{0.013 (0.001)} & 0.046 (0.003)          \\
 sports-ball  & 0.011 (0.000)          & 0.069 (0.015) & 0.085 (0.030) & 0.013 (0.002)          & \textbf{0.009 (0.001)} \\
 kite         & \textbf{0.002 (0.000)} & 0.020 (0.007) & 0.019 (0.001) & \textbf{0.002 (0.000)} & 0.009 (0.001)          \\
\hline
 Average      & \textbf{0.010 (0.000)} & 0.064 (0.004) & 0.102 (0.012) & 0.012 (0.000)          & 0.022 (0.000)          \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_err_loss_neg_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & 0.115 (0.008)          & 0.188 (0.078) & 0.218 (0.031) & \textbf{0.086 (0.019)} & 0.262 (0.009) \\
 bowl         & \textbf{0.141 (0.024)} & 0.471 (0.039) & 0.561 (0.039) & \textbf{0.147 (0.046)} & 0.403 (0.014) \\
 boat         & \textbf{0.067 (0.007)} & 0.210 (0.045) & 0.186 (0.087) & \textbf{0.045 (0.021)} & 0.343 (0.026) \\
 fire-hydrant & 0.013 (0.002)          & 0.127 (0.026) & 0.212 (0.116) & \textbf{0.004 (0.001)} & 0.193 (0.008) \\
 airplane     & \textbf{0.002 (0.000)} & 0.029 (0.002) & 0.078 (0.025) & \textbf{0.003 (0.001)} & 0.047 (0.004) \\
 cow          & 0.019 (0.000)          & 0.105 (0.018) & 0.146 (0.037) & \textbf{0.014 (0.001)} & 0.118 (0.003) \\
 backpack     & \textbf{0.027 (0.003)} & 0.323 (0.015) & 0.332 (0.032) & \textbf{0.032 (0.019)} & 0.338 (0.004) \\
 cup          & \textbf{0.055 (0.001)} & 0.405 (0.032) & 0.340 (0.051) & 0.085 (0.009)          & 0.376 (0.012) \\
 surfboard    & \textbf{0.015 (0.001)} & 0.094 (0.034) & 0.102 (0.026) & \textbf{0.010 (0.004)} & 0.110 (0.003) \\
 tie          & 0.013 (0.000)          & 0.216 (0.025) & 0.413 (0.044) & \textbf{0.009 (0.003)} & 0.142 (0.008) \\
 sports-ball  & 0.023 (0.002)          & 0.168 (0.049) & 0.194 (0.014) & \textbf{0.014 (0.005)} & 0.172 (0.005) \\
 kite         & 0.004 (0.001)          & 0.041 (0.015) & 0.069 (0.005) & \textbf{0.003 (0.001)} & 0.065 (0.007) \\
\hline
 Average      & \textbf{0.041 (0.002)} & 0.198 (0.011) & 0.238 (0.015) & \textbf{0.038 (0.005)} & 0.214 (0.003) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_err_loss_pos_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM           & GDRO                   & IRM                    & CVAR          & Focal                  \\
\hline
 car          & 0.459 (0.013) & \textbf{0.251 (0.044)} & \textbf{0.278 (0.057)} & 0.495 (0.029) & 0.323 (0.006)          \\
 bowl         & 0.616 (0.031) & \textbf{0.300 (0.006)} & \textbf{0.276 (0.027)} & 0.670 (0.059) & 0.370 (0.017)          \\
 boat         & 0.419 (0.015) & \textbf{0.211 (0.040)} & \textbf{0.361 (0.135)} & 0.458 (0.040) & \textbf{0.211 (0.000)} \\
 fire-hydrant & 0.612 (0.015) & 0.399 (0.024)          & \textbf{0.376 (0.083)} & 0.543 (0.002) & \textbf{0.307 (0.011)} \\
 airplane     & 0.200 (0.013) & 0.098 (0.002)          & 0.116 (0.011)          & 0.186 (0.021) & \textbf{0.087 (0.002)} \\
 cow          & 0.459 (0.011) & \textbf{0.268 (0.022)} & 0.320 (0.033)          & 0.526 (0.043) & \textbf{0.249 (0.006)} \\
 backpack     & 0.881 (0.008) & 0.340 (0.006)          & \textbf{0.337 (0.073)} & 0.919 (0.044) & \textbf{0.316 (0.006)} \\
 cup          & 0.758 (0.008) & \textbf{0.247 (0.030)} & 0.369 (0.048)          & 0.779 (0.016) & \textbf{0.281 (0.011)} \\
 surfboard    & 0.517 (0.017) & 0.329 (0.031)          & 0.420 (0.067)          & 0.542 (0.081) & \textbf{0.206 (0.012)} \\
 tie          & 0.848 (0.009) & \textbf{0.299 (0.018)} & \textbf{0.321 (0.054)} & 0.870 (0.054) & 0.395 (0.009)          \\
 sports-ball  & 0.554 (0.017) & \textbf{0.243 (0.047)} & \textbf{0.243 (0.027)} & 0.614 (0.070) & 0.344 (0.005)          \\
 kite         & 0.382 (0.030) & \textbf{0.188 (0.052)} & \textbf{0.164 (0.030)} & 0.400 (0.015) & \textbf{0.176 (0.017)} \\
\hline
 Average      & 0.559 (0.005) & \textbf{0.264 (0.009)} & 0.298 (0.018)          & 0.583 (0.013) & \textbf{0.272 (0.003)} \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_nll_loss_easy_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & \textbf{0.056 (0.002)} & 0.408 (0.074) & 0.313 (0.074) & 0.285 (0.057)          & 0.093 (0.001) \\
 bowl         & \textbf{0.041 (0.001)} & 0.338 (0.068) & 0.495 (0.108) & 0.599 (0.003)          & 0.083 (0.004) \\
 boat         & \textbf{0.010 (0.000)} & 0.288 (0.009) & 0.453 (0.143) & 0.029 (0.003)          & 0.051 (0.004) \\
 fire-hydrant & \textbf{0.005 (0.000)} & 0.125 (0.021) & 0.151 (0.062) & 0.019 (0.006)          & 0.047 (0.001) \\
 airplane     & \textbf{0.002 (0.000)} & 0.053 (0.008) & 0.067 (0.017) & 0.004 (0.001)          & 0.032 (0.003) \\
 cow          & \textbf{0.005 (0.000)} & 0.101 (0.022) & 0.073 (0.026) & 0.019 (0.005)          & 0.020 (0.001) \\
 backpack     & \textbf{0.065 (0.001)} & 0.306 (0.024) & 0.326 (0.020) & 0.632 (0.008)          & 0.226 (0.003) \\
 cup          & \textbf{0.063 (0.001)} & 0.358 (0.045) & 0.280 (0.022) & 0.647 (0.007)          & 0.095 (0.006) \\
 surfboard    & \textbf{0.009 (0.000)} & 0.108 (0.038) & 0.159 (0.062) & 0.012 (0.001)          & 0.026 (0.001) \\
 tie          & \textbf{0.040 (0.001)} & 0.287 (0.050) & 0.617 (0.012) & 0.170 (0.027)          & 0.147 (0.008) \\
 sports-ball  & \textbf{0.026 (0.000)} & 0.249 (0.037) & 0.303 (0.053) & 0.084 (0.019)          & 0.056 (0.004) \\
 kite         & \textbf{0.009 (0.000)} & 0.071 (0.020) & 0.067 (0.006) & \textbf{0.008 (0.001)} & 0.036 (0.004) \\
\hline
 Average      & \textbf{0.028 (0.000)} & 0.224 (0.012) & 0.275 (0.019) & 0.209 (0.006)          & 0.076 (0.001) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_nll_loss_neg_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal         \\
\hline
 car          & \textbf{0.321 (0.016)} & 0.539 (0.075) & 0.575 (0.049) & 0.439 (0.060)          & 0.619 (0.021) \\
 bowl         & \textbf{0.361 (0.050)} & 0.786 (0.016) & 0.701 (0.005) & 0.671 (0.004)          & 0.876 (0.033) \\
 boat         & \textbf{0.200 (0.010)} & 0.499 (0.107) & 0.468 (0.097) & \textbf{0.182 (0.056)} & 0.838 (0.051) \\
 fire-hydrant & \textbf{0.044 (0.004)} & 0.369 (0.038) & 0.465 (0.121) & 0.064 (0.011)          & 0.438 (0.012) \\
 airplane     & \textbf{0.011 (0.001)} & 0.098 (0.011) & 0.230 (0.039) & \textbf{0.016 (0.004)} & 0.153 (0.013) \\
 cow          & \textbf{0.056 (0.001)} & 0.309 (0.046) & 0.349 (0.082) & \textbf{0.064 (0.009)} & 0.331 (0.005) \\
 backpack     & \textbf{0.103 (0.005)} & 0.602 (0.019) & 0.628 (0.048) & 0.655 (0.004)          & 0.754 (0.007) \\
 cup          & \textbf{0.166 (0.008)} & 0.693 (0.010) & 0.632 (0.043) & 0.679 (0.002)          & 0.854 (0.022) \\
 surfboard    & \textbf{0.038 (0.004)} & 0.268 (0.079) & 0.323 (0.065) & \textbf{0.037 (0.010)} & 0.307 (0.004) \\
 tie          & \textbf{0.047 (0.002)} & 0.517 (0.050) & 0.650 (0.008) & 0.193 (0.021)          & 0.395 (0.020) \\
 sports-ball  & \textbf{0.066 (0.003)} & 0.441 (0.073) & 0.484 (0.038) & 0.130 (0.020)          & 0.516 (0.020) \\
 kite         & \textbf{0.015 (0.002)} & 0.128 (0.042) & 0.211 (0.018) & \textbf{0.013 (0.002)} & 0.194 (0.021) \\
\hline
 Average      & \textbf{0.119 (0.005)} & 0.438 (0.016) & 0.476 (0.018) & 0.262 (0.007)          & 0.523 (0.007) \\
\hline
\end{tabular}

==> tables/app_stds_old/results_captions_nll_loss_pos_hard_with_stds.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM           & GDRO                   & IRM                    & CVAR          & Focal                  \\
\hline
 car          & 1.126 (0.045) & \textbf{0.456 (0.039)} & \textbf{0.487 (0.083)} & 0.690 (0.068) & 0.708 (0.011)          \\
 bowl         & 1.486 (0.089) & \textbf{0.533 (0.010)} & 0.675 (0.010)          & 0.705 (0.005) & 0.769 (0.035)          \\
 boat         & 1.386 (0.043) & \textbf{0.416 (0.049)} & 0.616 (0.133)          & 1.004 (0.070) & 0.517 (0.019)          \\
 fire-hydrant & 2.300 (0.060) & \textbf{0.707 (0.034)} & \textbf{0.617 (0.100)} & 1.382 (0.085) & \textbf{0.646 (0.008)} \\
 airplane     & 0.771 (0.038) & 0.247 (0.016)          & 0.269 (0.035)          & 0.628 (0.079) & \textbf{0.210 (0.003)} \\
 cow          & 1.634 (0.037) & \textbf{0.576 (0.071)} & \textbf{0.669 (0.034)} & 1.339 (0.093) & \textbf{0.623 (0.011)} \\
 backpack     & 2.363 (0.060) & \textbf{0.635 (0.006)} & \textbf{0.603 (0.077)} & 0.725 (0.005) & \textbf{0.631 (0.009)} \\
 cup          & 1.898 (0.068) & \textbf{0.522 (0.023)} & 0.633 (0.035)          & 0.702 (0.002) & 0.590 (0.022)          \\
 surfboard    & 2.045 (0.144) & 0.764 (0.112)          & 0.781 (0.028)          & 1.578 (0.184) & \textbf{0.629 (0.010)} \\
 tie          & 2.891 (0.027) & \textbf{0.557 (0.032)} & 0.669 (0.003)          & 1.374 (0.118) & 0.846 (0.028)          \\
 sports-ball  & 2.458 (0.013) & \textbf{0.442 (0.081)} & \textbf{0.507 (0.076)} & 1.282 (0.078) & 0.877 (0.034)          \\
 kite         & 1.672 (0.039) & \textbf{0.614 (0.222)} & \textbf{0.439 (0.083)} & 1.612 (0.165) & \textbf{0.435 (0.047)} \\
\hline
 Average      & 1.836 (0.019) & \textbf{0.539 (0.024)} & \textbf{0.581 (0.020)} & 1.085 (0.028) & 0.623 (0.007)          \\
\hline
\end{tabular}

==> tables/area_aucs_easy.tex <==
% \begin{tabular}{llrrll}
% \hline
%  Task         & ERM            &   GDRO &   IRM & CVAR           & Focal          \\
% \hline
%  car          & \textbf{0.988} &  0.91  & 0.96  & 0.987          & 0.988          \\
%  bowl         & 0.983          &  0.93  & 0.942 & 0.975          & \textbf{0.984} \\
%  boat         & 0.995          &  0.969 & 0.923 & 0.996          & \textbf{0.996} \\
%  fire-hydrant & 0.979          &  0.965 & 0.966 & 0.982          & \textbf{0.985} \\
%  airplane     & 0.997          &  0.985 & 0.998 & \textbf{0.999} & 0.998          \\
%  cow          & 0.995          &  0.959 & 0.99  & 0.995          & \textbf{0.997} \\
%  backpack     & 0.932          &  0.913 & 0.887 & 0.850          & \textbf{0.938} \\
%  cup          & \textbf{0.966} &  0.918 & 0.926 & 0.941          & 0.966          \\
%  surfboard    & 0.998          &  0.974 & 0.951 & 0.998          & \textbf{0.998} \\
%  tie          & 0.987          &  0.982 & 0.976 & 0.983          & \textbf{0.988} \\
%  sports-ball  & 0.993          &  0.956 & 0.935 & \textbf{0.994} & 0.994          \\
%  kite         & 0.999          &  0.997 & 0.997 & \textbf{0.999} & 0.999          \\
% \hline
% \end{tabular}
% \begin{tabular}{llrrll}
% \hline
%  Task         & ERM            &   GDRO &   IRM & CVAR           & Focal          \\
% \hline
%  car          & \textbf{0.988} &  0.918 & 0.959 & 0.987          & 0.988          \\
%  bowl         & 0.983          &  0.922 & 0.943 & 0.975          & \textbf{0.983} \\
%  boat         & 0.995          &  0.969 & 0.945 & 0.996          & \textbf{0.996} \\
%  fire-hydrant & 0.979          &  0.965 & 0.972 & 0.982          & \textbf{0.986} \\
%  airplane     & 0.997          &  0.988 & 0.998 & \textbf{0.999} & 0.998          \\
%  cow          & 0.995          &  0.965 & 0.995 & 0.995          & \textbf{0.997} \\
%  backpack     & 0.932          &  0.907 & 0.903 & 0.850          & \textbf{0.937} \\
%  cup          & \textbf{0.966} &  0.929 & 0.921 & 0.941          & 0.966          \\
%  surfboard    & 0.998          &  0.979 & 0.989 & 0.998          & \textbf{0.998} \\
%  tie          & 0.987          &  0.985 & 0.876 & 0.983          & \textbf{0.989} \\
%  sports-ball  & 0.993          &  0.959 & 0.951 & \textbf{0.994} & 0.994          \\
%  kite         & 0.999          &  0.998 & 0.997 & \textbf{0.999} & 0.999          \\
% \hline
% \end{tabular}
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & \textbf{0.988 (0.000)} & 0.765 (0.044) & 0.959 (0.003)          & \textbf{0.987 (0.002)} & \textbf{0.988 (0.000)} \\
 bowl         & 0.983 (0.000)          & 0.927 (0.017) & 0.943 (0.007)          & 0.975 (0.003)          & \textbf{0.983 (0.000)} \\
 boat         & 0.995 (0.000)          & 0.961 (0.011) & 0.945 (0.022)          & \textbf{0.996 (0.001)} & \textbf{0.996 (0.000)} \\
 fire-hydrant & 0.979 (0.001)          & 0.962 (0.003) & 0.972 (0.005)          & 0.982 (0.003)          & \textbf{0.986 (0.001)} \\
 airplane     & 0.997 (0.001)          & 0.989 (0.003) & \textbf{0.998 (0.002)} & \textbf{0.999 (0.001)} & \textbf{0.998 (0.000)} \\
 cow          & 0.995 (0.001)          & 0.981 (0.007) & 0.995 (0.001)          & 0.995 (0.001)          & \textbf{0.997 (0.000)} \\
 backpack     & 0.932 (0.001)          & 0.898 (0.014) & 0.903 (0.011)          & 0.850 (0.018)          & \textbf{0.937 (0.001)} \\
 cup          & \textbf{0.966 (0.001)} & 0.922 (0.007) & 0.921 (0.007)          & 0.941 (0.006)          & \textbf{0.966 (0.000)} \\
 surfboard    & 0.998 (0.000)          & 0.980 (0.004) & 0.989 (0.003)          & \textbf{0.998 (0.000)} & \textbf{0.998 (0.000)} \\
 tie          & 0.987 (0.001)          & 0.983 (0.003) & 0.876 (0.024)          & \textbf{0.983 (0.006)} & \textbf{0.989 (0.000)} \\
 sports-ball  & \textbf{0.993 (0.000)} & 0.962 (0.004) & 0.951 (0.014)          & \textbf{0.994 (0.000)} & \textbf{0.994 (0.000)} \\
 kite         & 0.999 (0.000)          & 0.996 (0.000) & 0.997 (0.000)          & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
 Average      & 0.984 (0.000)          & 0.944 (0.004) & 0.954 (0.003)          & 0.975 (0.002)          & \textbf{0.986 (0.000)} \\
\hline
\end{tabular}


==> tables/area_aucs_hard_std.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & 0.769 (0.002)          & \textbf{0.923 (0.001)} & 0.868 (0.004)          & 0.780 (0.010)          & 0.773 (0.001)          \\
 bowl         & 0.749 (0.003)          & \textbf{0.846 (0.013)} & \textbf{0.828 (0.023)} & 0.701 (0.009)          & 0.751 (0.005)          \\
 boat         & 0.869 (0.002)          & \textbf{0.945 (0.012)} & 0.909 (0.014)          & 0.894 (0.021)          & 0.854 (0.007)          \\
 fire-hydrant & 0.913 (0.004)          & \textbf{0.942 (0.004)} & 0.902 (0.008)          & 0.933 (0.003)          & 0.925 (0.001)          \\
 airplane     & 0.986 (0.002)          & \textbf{0.995 (0.001)} & 0.986 (0.003)          & 0.984 (0.002)          & 0.983 (0.001)          \\
 cow          & 0.935 (0.003)          & \textbf{0.963 (0.004)} & 0.943 (0.001)          & 0.922 (0.007)          & 0.939 (0.002)          \\
 backpack     & 0.812 (0.004)          & \textbf{0.849 (0.012)} & \textbf{0.811 (0.032)} & 0.755 (0.034)          & 0.816 (0.003)          \\
 cup          & \textbf{0.870 (0.004)} & 0.825 (0.019)          & 0.820 (0.025)          & 0.794 (0.020)          & \textbf{0.868 (0.002)} \\
 surfboard    & 0.939 (0.002)          & \textbf{0.960 (0.004)} & \textbf{0.957 (0.008)} & 0.937 (0.003)          & 0.935 (0.000)          \\
 tie          & 0.742 (0.002)          & \textbf{0.781 (0.036)} & 0.640 (0.029)          & \textbf{0.696 (0.075)} & \textbf{0.743 (0.006)} \\
 sports-ball  & 0.867 (0.002)          & \textbf{0.909 (0.001)} & \textbf{0.859 (0.050)} & 0.856 (0.008)          & 0.865 (0.001)          \\
 kite         & 0.932 (0.001)          & \textbf{0.960 (0.005)} & \textbf{0.953 (0.004)} & 0.931 (0.004)          & 0.940 (0.001)          \\
 Average      & 0.865 (0.001)          & \textbf{0.908 (0.004)} & 0.873 (0.006)          & 0.849 (0.007)          & 0.866 (0.001)          \\
\hline
\end{tabular}

==> tables/calib_failure_modes.tex <==
\begin{tabular}{lrrrrr}
\hline
                   &   ERM &   GDRO &   IRM &   CVAR &   Focal \\
\hline
 Slight Underconf. &     0 &      3 &     4 &      4 &       0 \\
 Very Underconf.   &     0 &      0 &     0 &      1 &       0 \\
 Slight Overconf.  &     0 &      0 &     0 &      0 &       0 \\
 Very Overconf.    &     0 &      4 &     0 &      0 &       0 \\
\hline
\end{tabular}

==> tables/caption_aucs_easy.tex <==
% \begin{tabular}{llrrrl}
% \hline
%  Task         & ERM            &   GDRO &   IRM &   CVAR & Focal          \\
% \hline
%  car          & \textbf{0.988} &  0.935 & 0.968 &  0.952 & 0.987          \\
%  bowl         & 0.993          &  0.946 & 0.955 &  0.985 & \textbf{0.994} \\
%  boat         & 0.993          &  0.968 & 0.938 &  0.993 & \textbf{0.995} \\
%  fire-hydrant & 0.986          &  0.975 & 0.975 &  0.992 & \textbf{0.994} \\
%  airplane     & 0.999          &  0.998 & 0.996 &  0.999 & \textbf{0.999} \\
%  cow          & 0.992          &  0.99  & 0.982 &  0.99  & \textbf{0.996} \\
%  backpack     & 0.959          &  0.942 & 0.927 &  0.909 & \textbf{0.961} \\
%  cup          & \textbf{0.989} &  0.949 & 0.938 &  0.961 & 0.989          \\
%  surfboard    & 0.994          &  0.979 & 0.954 &  0.995 & \textbf{0.997} \\
%  tie          & 0.976          &  0.976 & 0.975 &  0.971 & \textbf{0.980} \\
%  sports-ball  & 0.997          &  0.96  & 0.935 &  0.997 & \textbf{0.998} \\
%  kite         & 0.996          &  0.997 & 0.997 &  0.996 & \textbf{0.998} \\
% \hline
% \end{tabular}
% \begin{tabular}{llrrll}
% \hline
%  Task         & ERM            &   GDRO &   IRM & CVAR           & Focal          \\
% \hline
%  car          & \textbf{0.990} &  0.933 & 0.948 & 0.989          & 0.990          \\
%  bowl         & \textbf{0.991} &  0.957 & 0.856 & 0.984          & 0.990          \\
%  boat         & 0.999          &  0.996 & 0.956 & \textbf{0.999} & 0.999          \\
%  fire-hydrant & 0.999          &  0.998 & 0.996 & 0.998          & \textbf{0.999} \\
%  airplane     & 1.000          &  1     & 1     & \textbf{1.000} & 1.000          \\
%  cow          & 1.000          &  0.994 & 0.997 & 0.999          & \textbf{1.000} \\
%  backpack     & 0.972          &  0.957 & 0.942 & 0.919          & \textbf{0.972} \\
%  cup          & \textbf{0.995} &  0.962 & 0.959 & 0.975          & 0.995          \\
%  surfboard    & 0.999          &  0.991 & 0.983 & 0.999          & \textbf{1.000} \\
%  tie          & 0.978          &  0.979 & 0.863 & 0.972          & \textbf{0.981} \\
%  sports-ball  & 0.999          &  0.966 & 0.956 & 0.998          & \textbf{0.999} \\
%  kite         & 0.998          &  0.998 & 0.997 & 0.999          & \textbf{0.999} \\
% \hline
% \end{tabular}
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO          & IRM           & CVAR                   & Focal                  \\
\hline
 car          & \textbf{0.990 (0.000)} & 0.930 (0.013) & 0.948 (0.014) & 0.989 (0.001)          & 0.990 (0.000)          \\
 bowl         & \textbf{0.991 (0.000)} & 0.959 (0.009) & 0.856 (0.035) & 0.984 (0.002)          & \textbf{0.990 (0.000)} \\
 boat         & \textbf{0.999 (0.000)} & 0.996 (0.001) & 0.956 (0.015) & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
 fire-hydrant & 0.999 (0.000)          & 0.998 (0.000) & 0.996 (0.002) & \textbf{0.998 (0.001)} & \textbf{0.999 (0.000)} \\
 airplane     & \textbf{1.000 (0.000)} & 1.000 (0.000) & 1.000 (0.000) & \textbf{1.000 (0.000)} & \textbf{1.000 (0.000)} \\
 cow          & 1.000 (0.000)          & 0.995 (0.003) & 0.997 (0.001) & 0.999 (0.000)          & \textbf{1.000 (0.000)} \\
 backpack     & \textbf{0.972 (0.001)} & 0.958 (0.002) & 0.942 (0.004) & 0.919 (0.021)          & \textbf{0.972 (0.000)} \\
 cup          & \textbf{0.995 (0.001)} & 0.950 (0.010) & 0.959 (0.014) & 0.975 (0.003)          & \textbf{0.995 (0.000)} \\
 surfboard    & 0.999 (0.000)          & 0.991 (0.003) & 0.983 (0.010) & 0.999 (0.000)          & \textbf{1.000 (0.000)} \\
 tie          & 0.978 (0.001)          & 0.978 (0.001) & 0.863 (0.028) & 0.972 (0.004)          & \textbf{0.981 (0.001)} \\
 sports-ball  & 0.999 (0.000)          & 0.968 (0.004) & 0.956 (0.018) & 0.998 (0.001)          & \textbf{0.999 (0.000)} \\
 kite         & 0.998 (0.000)          & 0.997 (0.000) & 0.997 (0.001) & \textbf{0.999 (0.000)} & \textbf{0.999 (0.000)} \\
 Average      & 0.993 (0.000)          & 0.977 (0.002) & 0.954 (0.005) & 0.986 (0.002)          & \textbf{0.994 (0.000)} \\
\hline
\end{tabular}

==> tables/caption_aucs_hard_std.tex <==
\begin{tabular}{llllll}
\hline
 Task         & ERM                    & GDRO                   & IRM                    & CVAR                   & Focal                  \\
\hline
 car          & 0.766 (0.002)          & \textbf{0.850 (0.014)} & \textbf{0.817 (0.026)} & 0.780 (0.010)          & 0.770 (0.003)          \\
 bowl         & 0.642 (0.004)          & \textbf{0.674 (0.019)} & 0.631 (0.014)          & 0.620 (0.021)          & \textbf{0.655 (0.009)} \\
 boat         & 0.826 (0.002)          & \textbf{0.880 (0.010)} & 0.818 (0.036)          & \textbf{0.855 (0.019)} & 0.806 (0.007)          \\
 fire-hydrant & 0.840 (0.007)          & 0.798 (0.011)          & 0.788 (0.018)          & \textbf{0.865 (0.008)} & 0.847 (0.002)          \\
 airplane     & 0.977 (0.001)          & \textbf{0.981 (0.002)} & 0.961 (0.001)          & 0.979 (0.000)          & 0.975 (0.002)          \\
 cow          & \textbf{0.901 (0.004)} & \textbf{0.906 (0.004)} & 0.845 (0.037)          & \textbf{0.900 (0.003)} & 0.895 (0.003)          \\
 backpack     & \textbf{0.716 (0.004)} & \textbf{0.732 (0.012)} & \textbf{0.729 (0.024)} & 0.604 (0.014)          & \textbf{0.731 (0.003)} \\
 cup          & \textbf{0.733 (0.006)} & \textbf{0.742 (0.015)} & \textbf{0.705 (0.041)} & 0.664 (0.008)          & \textbf{0.729 (0.007)} \\
 surfboard    & \textbf{0.913 (0.002)} & 0.875 (0.005)          & 0.836 (0.030)          & \textbf{0.918 (0.003)} & 0.903 (0.001)          \\
 tie          & \textbf{0.822 (0.003)} & \textbf{0.820 (0.018)} & 0.696 (0.014)          & 0.783 (0.028)          & \textbf{0.821 (0.004)} \\
 sports-ball  & 0.830 (0.003)          & \textbf{0.880 (0.001)} & 0.848 (0.029)          & 0.826 (0.011)          & 0.824 (0.002)          \\
 kite         & \textbf{0.942 (0.001)} & \textbf{0.947 (0.007)} & \textbf{0.943 (0.010)} & \textbf{0.940 (0.004)} & \textbf{0.947 (0.001)} \\
 Average      & 0.826 (0.001)          & \textbf{0.841 (0.003)} & 0.801 (0.008)          & 0.811 (0.004)          & 0.825 (0.001)          \\
\hline
\end{tabular}

==> trash.tex <==

\section{A Bunch of Results Figures}


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_hardpos_beta.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_hardneg_beta.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_maxhphn_beta.pdf}
\end{subfigure}
\caption{
L to R: NLL on hard positives, hard negatives, max(hard positives, hard negatives).
Area method, at $\alpha=0.05$, across a range of $\beta$.
After hyperparameter selection.
} \label{fig:results-avg-nll-3-area}
\end{figure}

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_hardpos_alpha.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_hardneg_alpha.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_maxhphn_alpha.pdf}
\end{subfigure}
\caption{
L to R: NLL on hard positives, hard negatives, max(hard positives, hard negatives).
Area method, at $\alpha=0.05$, across a range of $\beta$.
After hyperparameter selection.
} \label{fig:results-avg-nll-3-area}
\end{figure}


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_nll_hardpos.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_nll_hardneg.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_nll_maxhphn.pdf}
\end{subfigure}
\caption{
L to R: NLL on hard positives, hard negatives, max(hard positives, hard negatives).
Caption method, across a range of $\tau$.
After hyperparameter selection.
} \label{fig:results-avg-nll-3-caption}
\end{figure}



\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_err_hardpos_beta.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_err_hardneg_beta.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_err_maxhphn_beta.pdf}
\end{subfigure}
\caption{
L to R: Error on hard positives, hard negatives, max(hard positives, hard negatives).
Area method, at $\alpha=0.05$, across a range of $\beta$.
After hyperparameter selection.
} \label{fig:results-avg-err-3-area}
\end{figure}


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_err_hardpos.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_err_hardneg.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_err_maxhphn.pdf}
\end{subfigure}
\caption{
L to R: Error on hard positives, hard negatives, max(hard positives, hard negatives).
Caption method, across a range of $\tau$.
After hyperparameter selection.
} \label{fig:results-avg-err-3-caption}
\end{figure}

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_ece_hard_beta.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_ece_easy_beta.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_ece_maxhardeasy_beta.pdf}
\end{subfigure}
\caption{
L to R: ECE on hard examples, easy examples, max(hard easy).
Area method, at $\alpha=0.05$, across a range of $\beta$.
After hyperparameter selection.
} \label{fig:results-avg-ece-3-area}
\end{figure}


\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_ece_hard.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_ece_easy.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.33\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_ece_maxhardeasy.pdf}
\end{subfigure}
\caption{
L to R: ECE on hard examples, easy examples, max(hard easy).
Caption method, across a range of $\tau$.
After hyperparameter selection.
} \label{fig:results-avg-ece-3-caption}
\end{figure}





\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_nll_maxhphn_beta.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_nll_maxhphn.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
The maximum of NLL on hard positives/hard negatives averaged over 12 tasks.
L: area method, at $\alpha=0.05$, across a range of $\beta$.
R: caption method, across a range of $\tau$.
} \label{fig:results-avg-nll}
\end{figure}

\begin{figure}[t!] % "[t!]" placement specifier just for this example
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_area_ece_maxhardeasy_beta.pdf}
% \caption{First subfigure} \label{fig:a}
\end{subfigure}\hspace*{\fill}
\begin{subfigure}{0.48\textwidth}
\includegraphics[width=\linewidth]{figs/results/algo_comp/algo_comp_caption_ece_maxhardeasy.pdf}
% \caption{Second subfigure} \label{fig:b}
\end{subfigure}
\caption{
The maximum of ECE on hard/easy cases averaged over 12 tasks.
L: area method, at $\alpha=0.05$, across a range of $\beta$.
R: caption method, across a range of $\tau$.
} \label{fig:results-avg-ece}
\end{figure}




To ground our exploration of OOC prediction, we use the COCO-Stuff dataset [cite].
This dataset is built on top of the MS-COCO dataset [cite] --- all the images are the same, but COCO-Stuff has extra annotations.
Whereas in COCO, only the ``things'' are labelled, in COCO-Stuff, the ``stuff'' is labelled as well.
The distinction between things and stuff is not so important for the purposes of this paper --- in fact, the taxonomy used by the COCO-Stuff dataset is somewhat irregular (e.g. ``fruit'' is stuff but ``apple'' is a thing).
The most important feature for our purposes is that the COCO-Stuff dataset has every pixel labelled with segmentation information, both foreground objects and background information, and as such yields a coarse but complete description of each image in the dataset.
This is a very rich sandbox for exploring the effects of different types of data on machine learning systems; we focus on one specific avenue here.

In the COCO-Stuff dataset, there are 171 different object categories.
Each image may contain many objects --- some images contain only 1 or 2, some contain > 20.
Most object categories are very imbalanced throughout the dataset (... some statistic here).
We can use the object information to examine co-occurence information





We can train a binary classification model on each of these 171 tasks --- show some result in a figure.

We present the RoCOCO benchmark, which is simply a suite of 12 (10?) binary object detection tasks

\begin{itemize}
    \item We want to look at robust methods in a realistic context
    \item COCOstuff gives us oppurtunity to do that
    \begin{itemize}
        \item describe dataset
    \end{itemize}
    \item Can locate potential confounders + hard positives/negatives
    \begin{itemize}
        \item define
    \end{itemize}
\end{itemize}


\begin{itemize}
    \item Context is important to prediction. What is context? Is it ultimately helpful or harmful for prediction?
    \begin{itemize}
        \item Hard to define
        \item Information theoretic
        \item Contextual cueing effect - it's the cues you can pick up quickly (more efficient), provides information we care about
        \item We care about presence or absence of possible contextual cues
    \end{itemize}
    \item Predicting out of context is hard
    \begin{itemize}
        \item Sometimes context is undersampled, or may not exist at all in the dataset
        \item Context is complicated - often multi-dimensional
        \item In this case, we are almost assured in practice to have OOC prediction problems
    \end{itemize}
    \item Specifically, we care about when this context is more extractible than the label we actually care about
    \begin{itemize}
        \item Then, due to simplicity bias of DNNs, we may learn to predict the context rather than the label
    \end{itemize}
    \item A number of works try to deal with this by using contextual information
    \begin{itemize}
        \item Environments - meaningful partitions of your data (causal interpretation but let's stay away from that)
        \item This often comes in simple forms - eg one hot features (environments), or the background of an image
        \item but context is often more complicated than this - context shifts can be subtle and occur throughout many properties of the image, rather than just the background
        \item Much research does not deal with this - mostly conducted in (semi-)synthetic settings, with manufactured biases/shifts
    \end{itemize}
    \item Investigate in a more realistic setting, where the notions for context is not predefined. Contributions:
    \begin{itemize}
        \item We introduce the Cocostuff robustness benchmark, with naturally occurring distribution shifts over context in object detection
        \item We find that some current methods that rely on environments for robustness fall a little short in some ways
        \begin{itemize}
            \item Define ``hard'' examples: don't do that well on hard examples in general. still much room to improve. Improvment over ERM is smaller than might be indicated in some more synthetic experiments. Some of this is due to less clean shifts; some is due to more confounders than just the 1 (hard examples may have many confounding features)
            \item Poor calibration (let alone multi-calibration) as compared to ERM
            \item Hypothesis: Excessive invariance - through examination of examples where robust underperforms ERM most, we hypothesize that robust algorithms may be excessively invariant to context
        \end{itemize}
        \item We have some ideas to improve?
        \begin{itemize}
            \item Focal loss? CVAR?
            \item Auxiliary tasks?
            \begin{itemize}
                \item Predict all the classes
            \end{itemize}
            \item trying to infer environments?
            \item More complex notions of context
            \item Adapting parameters to context
            \begin{itemize}
                \item Something like FLUTE/FiLM?
            \end{itemize}
        \end{itemize}
    \end{itemize}
    
\end{itemize}

\section{Cocostuff Dataset}

\begin{itemize}
    \item We want to look at robust methods in a realistic context
    \item COCOstuff gives us oppurtunity to do that
    \begin{itemize}
        \item describe dataset
    \end{itemize}
    \item Can locate potential confounders + hard positives/negatives
    \begin{itemize}
        \item define
    \end{itemize}
\end{itemize}

\section{Results}

\begin{itemize}
    \item Methods we are using:
    \begin{itemize}
        \item ERM
        \item Group DRO
        \item IRM
        \item CVAR
        \item Focal loss
        \item Time/compute permitting, other stuff
    \end{itemize}
    \item Results: Hard Positives/Negatives
    \begin{itemize}
        \item Overall: loss, accuracy
        \item Hard, HP, HN: loss accuracy
    \end{itemize}
    \item Results: Calibration
    \begin{itemize}
        \item Calibration plots
        \item Potentially - point out clothes + railroad as outliers??? (if they are still in the benchmark)
    \end{itemize}
    \item Results: Excessive invariance
    \begin{itemize}
        \item Look at best and worst examples of ERM vs Robust
        \item Try to describe using object co-occurence
        \item Contrast with methods that don't do invariance to context
    \end{itemize}
\end{itemize}
